QCSP monsters and the demise of the Chen Conjecture

We give a surprising classification for the computational complexity of the Quantified Constraint Satisfaction Problem over a constraint language $\Gamma$, QCSP$(\Gamma)$, where $\Gamma$ is a finite language over $3$ elements which contains all constants. In particular, such problems are either in P, NP-complete, co-NP-complete or PSpace-complete. Our classification refutes the hitherto widely-believed Chen Conjecture. Additionally, we show that already on a 4-element domain there exists a constraint language $\Gamma$ such that QCSP$(\Gamma)$ is DP-complete (from Boolean Hierarchy), and on a 10-element domain there exists a constraint language giving the complexity class $\Theta_{2}^{P}$. Meanwhile, we prove the Chen Conjecture for finite conservative languages $\Gamma$. If the polymorphism clone of $\Gamma$ has the polynomially generated powers (PGP) property then QCSP$(\Gamma)$ is in NP. Otherwise, the polymorphism clone of $\Gamma$ has the exponentially generated powers (EGP) property and QCSP$(\Gamma)$ is PSpace-complete.

==> MainResults.tex <==
\section{Main Results}\label{MainResults}
In this section we formulate two main results of the paper:
classification of the complexity of $\QCSP(\Gamma)$ 
for all constraint languages $\Gamma$ on a 3-element domain containing 
all constants, 
and a theorem showing how we can combine constraint languages to 
obtain exotic complexity classes.

\subsection{QCSP on a 3-element domain}

Let $a$ and $c$ be constants of our domain $\{0,1,2\}$.

$f_{a,c}(x,y,z) = 
\begin{cases}
x,& \text{if $x=y$ or $y=z=a$}\\
c, &\text{otherwise.}
\end{cases}$

$s_{a,c}(x,y) = \begin{cases}
x, & \text{if $x=y$ or $y=a$}\\
c, & \text{otherwise.}
\end{cases}$

$g_{a,c}(x,y) = \begin{cases}
x, & \text{if $x=a$ or $y\neq c$}\\
c, & \text{otherwise.}
\end{cases}$

$s_{c}(x,y) = \begin{cases}
x, & \text{if $x=y$}\\
c, & \text{otherwise.}
\end{cases}$

\noindent If $\{a,b,c\}=\{0,1,2\}$ then call any idempotent operation $f$, such that 
$f(x,a,b)=x$ and $f(x,c,c) = c$, \emph{$ab$-stable}. Note that $f(x,y,z) = s_{a,c}(x,y)$
is an $ab$-stable operation.
We get the following characterization of the complexity of $\QCSP(\Gamma)$ on a 3-element domain.

\begin{thm}\label{ThreeElementClassification}
Suppose 
$\Gamma$ is a finite constraint language on $\{0,1,2\}$ with constants. Then $\QCSP(\Gamma)$ is 
\begin{enumerate}
\item in P, if $\Pol(\Gamma)$ has the PGP property and has a WNU operation.
\item NP-complete, if $\Pol(\Gamma)$ has the PGP property and has no WNU operation.
\item PSpace-complete, if $\Pol(\Gamma)$ has the EGP property and
has no WNU operation.
%\item PSpace-complete, if $\Pol(\Gamma)$ has the EGP property and $\Pol(\Gamma)$ does not contain $f$ such that 
%$f(x,a)=x$ and $f(x,c) = c$, where $a,c\in\{0,1,2\}$.
\item PSpace-complete, if $\Pol(\Gamma)$ has the EGP property and $\Pol(\Gamma)$ does not contain an $ab$-stable operation.
\item in P, if $\Pol(\Gamma)$ contains $s_{a,c}$ and $g_{a,c}$ for some $a,c\in\{0,1,2\}$, $a\neq c$.
\item in P, if $\Pol(\Gamma)$ contains $f_{a,c}$ for some $a,c\in\{0,1,2\}$, $a\neq c$.
\item co-NP-complete otherwise (in which case $\Pol(\Gamma)$ additionally has an ab-stable operation).
\end{enumerate}
\end{thm}

Note that the semilattice $s_c$ can be derived 
from each of the operations 
$f_{a,c}$, $s_{a,c}$.
%Let $s$ be the semilattice operation on 
%$\{0,1,2\}$ such that 
%$s(a,b)=2$ whenever $a\neq b$. There are two other similar semilattices based on the other two bipartitions of $\{0,1,2\}$. Since they will not play a role in this paper, we resist naming them. 
As we know from \cite{BBCJK}, 
the problem 
$\QCSP(\Inv(s_2))$ is PSpace-complete.
Figure \ref{fig:EGP-WNU}
demonstrates how 
adding new operations 
makes the constraint language weaker and the 
quantified constraint satisfaction problem easier.
Note that all the languages in Figure \ref{fig:EGP-WNU} have the EGP property.
\begin{figure}
\begin{center}
%\begin{scope}[scale = 1,transform canvas={scale=0.8}
\begin{tikzpicture}[scale=0.88]%[sibling distance=20em,
%  every node/.style = {shape=ellipse, rounded corners,
%    draw, align=center,
%    top color=white, bottom color=blue!20}]]
 \node[shape=ellipse, rounded corners,
    draw, align=center,
    top color=white, bottom color=blue!20]  (s) at (-2,6) {$\{s_2\}$};
 \node[shape=ellipse, rounded corners,
    draw, align=center,
    top color=white, bottom color=blue!20]  (s02) at (-8,4) {$\{s_{0,2}\}$};
 \node[shape=ellipse, rounded corners,
    draw, align=center,
    top color=white, bottom color=blue!20]  (g02s) at (-4,4) {$\{g_{0,2},s_2\}$};
 \node[shape=ellipse, rounded corners,
    draw, align=center,
    top color=white, bottom color=blue!20]  (f02) at (-8,2) {$\{f_{0,2}\}$};
  \node[shape=ellipse, rounded corners,
    draw, align=center,
    top color=white, bottom color=blue!20]  (g02s02) at (-4,2) {$\{g_{0,2},s_{0,2}\}$};
%
 \node[shape=ellipse, rounded corners,
    draw, align=center,
    top color=white, bottom color=blue!20]  (g12s) at (0,4) {$\{g_{1,2},s_2\}$};
 \node[shape=ellipse, rounded corners,
    draw, align=center,
    top color=white, bottom color=blue!20]  (s12) at (4,4) {$\{s_{1,2}\}$};
 \node[shape=ellipse, rounded corners,
    draw, align=center,
    top color=white, bottom color=blue!20]  (g12s12) at (0,2) {$\{g_{1,2},s_{1,2}\}$};
  \node[shape=ellipse, rounded corners,
    draw, align=center,
    top color=white, bottom color=blue!20]  (f12) at (4,2) {$\{f_{1,2}\}$};

\node[scale=1.5] at (-2,7) {PSpace};
\node[scale=1.5] at (-8,6) {co-NP};
\node[scale=1.5] at (-8,1) {P};
\node[scale=1.5] at (-4,1) {P};
\node[scale=1.5] at (0,1) {P};
\node[scale=1.5] at (4,1) {P};

\path[->] (s) edge  (s02);
\path[->] (s) edge  (g02s);
\path[->] (s02) edge  (f02);
\path[->] (s02) edge  (g02s02);
\path[->] (g02s) edge  (g02s02);
%
\path[->] (s) edge  (s12);
\path[->] (s) edge  (g12s);
\path[->] (s12) edge  (f12);
\path[->] (s12) edge  (g12s12);
\path[->] (g12s) edge  (g12s12);

\draw (-7,7) .. controls (-7,1.5) and (3,1.5)  .. (3,7);
\draw (-5.7,1) .. controls (-6,3.4) and (-2,3.4)  .. (-2.3,1);
\draw (-9.6,1) .. controls (-9.8,3.4) and (-6.2,3.4)  .. (-6.4,1);
\draw (-1.7,1) .. controls (-2,3.4) and (2,3.4)  .. (1.7,1);
\draw (2.4,1) .. controls (2.2,3.4) and (5.8,3.4)  .. (5.6,1);

\end{tikzpicture}
\end{center}
%\caption{A part of the clone lattice, where clones are given by generating sets, in the case of EGP with a WNU (there may be clones omitted in this drawing).}
\caption{Constraint languages defined as
invariants of sets of operations and their complexity.}
\label{fig:EGP-WNU}
\end{figure}

\input{TheoremExamples}

\subsection{QCSP Monsters}

The following theorem shows how we can combine constraint languages to obtain QCSPs with different complexities.




\begin{thm}\label{QCSPMonsters}
Suppose $\Gamma_{1}$, $\Gamma_{2}$, and $\Gamma_{3}$ are finite constraint languages on sets $A_1$, $A_{2}$, and $A_{3}$, respectively, and $\Gamma_{1}$ contains a constant relation 
$(x=a)$. Then there exist
constraint languages 
$\Delta_{1}$, 
$\Delta_{2}$,
$\Delta_{3}$,
$\Delta_{4}$,
on the domains of size
$|A_{1}|+1$, 
$|A_{2}|\cdot|A_{3}|+|A_{2}|+|A_{3}|$, 
$2\cdot|A_{2}|+|A_{3}|+2$,
and 
$|A_{2}|\cdot|A_{3}|+|A_{2}|+|A_{3}|+2$,
respectively, such that 
$\QCSP(\Delta_{i})$ is polynomially equivalent to the 
following problem:
\begin{enumerate}
\item[i=1] Given an instance of $\QCSP(\Gamma_{1})$
and instance of an NP-complete problem;
decide whether both of them hold,
i.e. $\QCSP(\Gamma_{1})\wedge \mathit{NP}$.
\item[i=2] Given an instance of $\QCSP(\Gamma_{2})$ and 
an instance of $\QCSP(\Gamma_{3})$;
decide whether both of them hold,
i.e. $\QCSP(\Gamma_2)\wedge \QCSP(\Gamma_3)$.
\item[i=3] Given $n>0$, 
instances $I_{1},\ldots,I_{n}$ of $\QCSP(\Gamma_{2})$,
and
instances $J_{1},\ldots,J_{n}$ of $\CSP(\Gamma_{3})$;
decide whether
$(I_{1}\vee J_{1})\wedge \dots\wedge (I_{n}\vee J_{n})$
holds,
i.e.
$(\QCSP(\Gamma_{2})\vee \CSP(\Gamma_{3}))
\wedge
\dots
\wedge
(\QCSP(\Gamma_{2})\vee \CSP(\Gamma_{3}))$.

\item[i=4] Given $n>0$, instances  
$I_{1},\ldots,I_{n}$ of $\QCSP(\Gamma_{2})$,
and
instances $J_{1},\ldots,J_{n}$ of $\QCSP(\Gamma_{3})$;
decide whether
$(I_{1}\vee J_{1})\wedge \dots\wedge (I_{n}\vee J_{n})$
holds,
i.e.
$(\QCSP(\Gamma_{2})\vee \QCSP(\Gamma_{3}))
\wedge
\dots
\wedge
(\QCSP(\Gamma_{2})\vee \QCSP(\Gamma_{3}))$.
\end{enumerate}
\end{thm}

\begin{proof}
The proof for $i=1$, $i=2$, $i=3$, and $i=4$ 
follows from Lemmas~\ref{ConstraintConjunctionOne},
\ref{ConstraintConjunctionTwo}, \ref{ConstraintDisjunctionFirst}, and \ref{ConstraintDisjunction},
respectively.
\end{proof}


\begin{cor}\label{DPon4elements}
There exists a finite constraint language 
$\Gamma$ on a 4-element domain such that 
$\QCSP(\Gamma)$ is DP-complete (where 
$\mathit{DP} = \mathit{NP}
\wedge \mathit{co}\mbox{-}\mathit{NP}$ from the Boolean hierarchy).
\end{cor}

\begin{proof}
By Theorem~\ref{ThreeElementClassification},
there exists a constraint language $\Gamma_{1}$ on a 3-element domain with constants such that $\QCSP(\Gamma_{1})$ is co-NP-complete.
Applying Theorem~\ref{QCSPMonsters} with $i=1$
to $\Gamma_{1}$ we obtain a constraint language 
$\Gamma$ on a 4-element domain such that $\QCSP(\Gamma)$ is polynomially equivalent 
to DP.
\end{proof}

The complexity class $\Theta^{\mathrm{P}}_2$ (see \cite{LukasiewiczM17} and references therein) admits various definitions, one of which is that it allows a Turing machine polynomial time with a logarithmic number of calls to an NP\,oracle. A condition proved equivalent to this, through Theorems 4 and 7 of \cite{BussH91}, is as follows. 
In this theorem $i \le p(|x|)$ indicates $i$ is a  positive integer smaller than $p(|x|)$, where $x$ is a string of length $|x|$.
\begin{thm}[\cite{BussH91}]
Every predicate in $\Theta^{\mathrm{P}}_2$ can be defined by a formula of the form
$\exists i \le p(|x|) \ A(i,x) \wedge \neg B(i,x)$ as well as by a formula of the form $\forall i \le p'(|x|) \ A'(i,x) \vee \neg B'(i,x)$, where $A, B, A'$ and $B'$ are NP-predicates and $p$ and $p'$ are polynomials.
\label{thm:BH}
\end{thm}
\noindent The second (universal) characterization will play the key role in the following observation.
\begin{cor}
There exists a finite constraint language 
$\Gamma$ on a 10-element domain such that 
$\QCSP(\Gamma)$ is $\Theta^{\mathrm{P}}_2$-complete.
\label{cor:emil}
\end{cor}
\begin{proof}
By Theorem~\ref{ThreeElementClassification},
there exists a constraint language $\Gamma_{1}$ on a 3-element domain with constants such that $\QCSP(\Gamma_{1})$ is co-NP-complete.
Choose a constraint language $\Gamma_{2}$ on a 2-element domain such that 
$\CSP(\Gamma_{2})$ is NP-complete.
Using item 3 of Theorem~\ref{QCSPMonsters},
we construct a constraint language $\Gamma$ so that $\QCSP(\Gamma)$ is equivalent to the truth of $(I_{1}\vee J_{1})\wedge \dots\wedge (I_{n}\vee J_{n})$, where $I_1,\ldots,I_n$ are instances of $\QCSP(\Gamma_{1})$ and $J_1,\ldots,J_n$ are instances of $\CSP(\Gamma_{2})$. 

To prove membership of $\QCSP(\Gamma)$ in $\Theta^{\mathrm{P}}_2$, we use the second characterization of Theorem \ref{thm:BH} together with $A'(i,x)$ indicating that $J_i$ is a yes-instance of $\CSP(\Gamma_{2})$ and $\neg B'(i,x)$ indicating that $I_i$ is a yes-instance (or $B'(i,x)$ indicating $I_i$ is a no-instance) of $\QCSP(\Gamma_{1})$. Thus, we want $i$ to range over numbers from $1$ to $n$, so in the predicates $A'(i,x)$ and $\neg B'(i,x)$ we should in particular set these to be true if $i$ is not a number from $1$ to $n$.

To prove that $\QCSP(\Gamma)$ is $\Theta^{\mathrm{P}}_2$-complete, we use again the second formulation of characterization of Theorem \ref{thm:BH}, but this time break the universal quantification into a conjunction of length $p'(|x|)$.
\end{proof}



%\subsection{Conservative QCSP}



==> old/Reductions.tex <==
\section{Reductions and hardness results for the 3-element domain}\label{HardnessSection}

In this section we consider the domain $A= \{0,1,2\}$
and prove all the hardness results we need for the 3-element domain.
An operation $f$ is called \emph{$0$-stable}
if $f(x,0) = x$ and $f(x,2) = 2$.
An operation $f$ is called \emph{$1$-stable}
if $f(x,1) = x$ and $f(x,2) = 2$.
Recall that 
$s_2$ is the semilattice operation such that
$s_2(a,b) = 2$ whenever $a\neq b$.

We will show how 
$\QCSP(\Gamma)$ can be reduced to a $\Pi_{2}$ formula 
if $\Gamma$ is preserved 
by a 0-stable or a 1-stable operation.

Let us define the following relations:
\[
\begin{array}{c}
\sigma = \{0,2\}^2 \cup \{1,2\}^2 \\
\sigma_0 = \{ (a,b,c) : a \in A, b,c \in \{1,2\}, (a \in \{0,2\} \vee b=c) \} \\
\sigma'_0 = \{ (a,b,c) : a \in A, b,c \in \{0,2\}, (a \in \{0,2\} \vee b=c) \} \\
\sigma_1 = \{ (a,b,c) : a \in A, b,c \in \{0,2\}, (a \in \{1,2\} \vee b=c) \} \\
\sigma'_1 = \{ (a,b,c) : a \in A, b,c \in \{1,2\}, (a \in \{1,2\} \vee b=c) \}
\end{array}
\]
\begin{lem}
The problems $\QCSP(\{\sigma,\sigma_0,\sigma_1\})$, $\QCSP(\{\sigma'_0,\sigma_1\})$ and $\QCSP(\{\sigma_0,\sigma'_1\})$ are PSpace-hard.
\label{PSpaceHardness}
\end{lem}

\begin{proof}
Let us begin with QCSP$(\{\sigma,\sigma_0,\sigma_1\})$. The reduction will be from the complement of (monotone) \emph{Quantified Not-All-Equal 3-Satisfiability} (co-QNAE3SAT) which is co-PSpace-hard (see \cite{papa}) and consequently also PSpace-hard (as PSpace is closed under complement). Consider an instance $I$ of co-QNAE3SAT of the form $(x_{a_1},x_{b_1},x_{c_1}), \ldots, (x_{a_s},x_{b_s},x_{c_s})$ which is a yes-instance precisely when, for all truth assignments to the variables, one among these triples $(x_{a_i},x_{b_i},x_{c_i})$ is either $(0,0,0)$ or $(1,1,1)$. We will use two variables $x^0_i$ and $x^1_i$ to encode each variable $x_{i}$ from the original problem (among the $x_{a_i},x_{b_i},x_{c_i}$). $x_i=0$ will be encoded as $(x^0_i,x^1_i)=(1,0)$ and $x_i=1$ will be encoded as $(x^0_i,x^1_i)=(0,1)$. We start with the formula
\[
\begin{array}{ll}
\Phi= & \bigwedge_{1 \le i \le s} (\sigma_1(x_{a_i}^0,y_{i-1},y_i) \wedge \sigma_1(x_{b_i}^0,y_{i-1},y_i) \wedge \sigma_1(x_{c_i}^0,y_{i-1},y_i)) \wedge \\
& \bigwedge_{s+1 \le i \le 2s} (\sigma_1(x_{a_i}^1,y_{i-1},y_i) \wedge \sigma_1(x_{b_i}^1,y_{i-1},y_i) \wedge \sigma_1(x_{c_i}^1,y_{i-1},y_i))
\end{array}
\]
with the quantifier prefix $\exists y_1 \ldots \exists y_{2s-1}$.  Suppose we imagine our $x$ variables restricted to $\{0,1\}$, then $\Phi$ captures the quantifier-free part of $I$ when either $y_0=0$ and $y_{2s}=2$; or $y_0=2$ and $y_{2s}=0$.

Let the quantifier prefix of $I$ be $Q_nx_n\ldots Q_1x_1$. Starting with $Q_1x_1$, we modify $\Phi$ iteratively in the following way. Let $k$ and $l$ be the minimal and maximal indices appearing in the $y$ variables of $\Phi$, respectively. Note that $k \le 0$ and $l>0$, and that typically $k$ decreases and $l$ increases during our construction. 

If $Q_i$ is a universal quantifier then we add outermost quantification to $\Phi$ of $\forall x^0_i \forall x^1_i$ and do not modify the quantifier-free part.

If $Q_i$ is an existential quantifier then we add outermost quantification to $\Phi$ of $\exists y_k \forall x^0_i \forall x^1_i \exists y_l$ and conjoin $\sigma_1(x^0_i,y_{k-1},y_l) \wedge \sigma_1(x^1_i,y_{l},y_{l+1})$ to the quantifier-free part. The idea is that $y_k$ ``chooses'' $(x^0_i,x^1_i)=(0,1)$ or $(x^0_i,x^1_i)=(1,0)$ in the following fashion.
%
Let us assume that $y_{k-1},y_k,y_l,y_{l+1} \in \{0,2\}$, $y_{k-1} \neq y_{l+1}$, $x^0_i,x^1_i \in \{0,1\}$, $x^0_i \neq x^1_i$, which we shall subsequently see will be the case. At the point Existential plays $y_k$, she knows the values of $y_{k-1}$ and $y_{l+1}$. Let us start with the case $(y_{k-1},y_{l+1})=(0,2)$. If $y_k=0$, then Universal must play $(x^0_i,x^1_i)=(1,0)$ in order to force $y_k \neq y_{l} = 2$. If Universal played $(x^0_i,x^1_i)=(0,1)$, then Existential could get away with $y_k = y_{l} = 0$. If $y_k=2$, then it is the other way around, with Universal having to play $(x^0_i,x^1_i)=(0,1)$ in order to force $y_k \neq y_{l} = 0$. Thus, $y_k=0$ chooses $(x^0_i,x^1_i)=(1,0)$ and $y_k=2$ chooses $(x^0_i,x^1_i)=(0,1)$. The second case of $(y_{k-1},y_{l+1})=(0,2)$ similarly splits into two subcases.

We call the quantifiers of $\Phi$ associated with those from the instance $I$ the \emph{simulation} quantifiers. Let us now ensure that Universal never tries to play some $(x^0_i,x^1_i)$ with $x^0_i=x^1_i$. We will conjoin the following.
\[
\begin{array}{c}
\Delta_0 = \bigwedge_{1 \le i \le n} \left( \sigma_0(x^0_i,z_{i-1},z_i) \wedge \sigma_0(x^1_i,z_{i-1},z_i) \right) \\
\Delta_1 = \bigwedge_{1 \le i \le n} \left( \sigma_1(x^0_i,t_{i-1},t_i) \wedge \sigma_1(x^1_i,t_{i-1},t_i) \right) \\
\end{array}
\]
The idea here is that, if (for any $i$) $x^0_i=x^1_i=0$, then $\Delta_0$ holds on a tuple with $(z_0,z_n)=(1,2)$; while if  (for any $i$) $x^0_i=x^1_i=1$, then $\Delta_1$ holds on a tuple with $(t_0,t_n)=(0,2)$.

Let $k$ and $l$ be, respectively, minimal and maximal indices appearing in the final formula $\Phi$. We claim that the original instance $I$ is equivalent to the following instance $\Psi$ of $\QCSP(\{\sigma,\sigma_0,\sigma_1\})$.
\[ y_k=0 \wedge \Phi \wedge y_l=t_0 \wedge \Delta_1 \wedge \sigma(t_n,z_n) \wedge \Delta_0 \wedge z_0=1 \]
where we make this prenex and add quantifiers $\exists t_0 \ldots \exists t_n \exists z_0 \ldots \exists z_n \exists y_k \exists y_l$ innermost. For pedagogical reasons we prefer to imagine the quantifiers $\exists y_1 \ldots \exists y_{2s-1}$ to be truly innermost, but since existential quantifiers commute with one another, this is no problem.


%## BARNY Below, it is probably not clear that by 
% x_{i}^{0},x_{i}^{1}=2 you mean that just one of them is equal to 2.
% fixed
($I\in \mathrm{co\mbox{-}QNAE3SAT}$ implies $\Psi \in \QCSP(\{\sigma,\sigma_0,\sigma_1\})$.) Let us begin by arguing that if Universal at any point plays some $x^0_i=x^1_i$ or $x^0_i,x^1_i =2$ then Existential will surely win. Suppose some $x^0_i=x^1_i=0$, then we know $\Delta_0$ holds on a tuple with $(z_0,z_n)=(1,2)$. It doesn't matter how the simulation quantifiers have been evaluated, we just set $t_n,\ldots,t_0=0$ and $y_k,\ldots,y_l=0$ (and evaluate the $z_i$ in between $z_0$ and $z_n$ as in the tuples that satisfies $\Delta_0$). Suppose some $x^0_i=x^1_i=1$, then we know $\Delta_1$ holds on a tuple with $(t_0,t_n)=(0,2)$. Set $z_n,\ldots,z_0=1$ and $y_k,\ldots,y_l=0$. Suppose now some $x^0_j=2$ or $x^1_j=2$, we find  again that $\Delta_0$ holds on a tuple with $(z_0,z_n)=(1,2)$
or 
$\Delta_1$ holds on a tuple with $(t_0,t_n)=(0,2)$.
%## BARNY. The case below was already considered.
% fixed
%while if  (for any $i$) $x^0_i=x^1_i=1$, then $\Delta_1$ holds on a tuple with $(t_0,t_n)=(0,2)$
Thus, we reduce to previous cases.

We now know that Universal must play each $(x^0_j,x^1_j)$ as either $(0,1)$ or $(1,0)$ if he is to have any chance of winning on $\Psi$. We have assumed Existential has a winning strategy in $I$ and this can be copied in $\Psi$ according to how we described the rules for how each $\exists y_k \forall x^0_i \forall x^1_i \exists y_l$ selects either  $(x^0_i,x^1_i)=(0,1)$ or $(x^0_i,x^1_i)=(1,0)$.  After the quantifiers are played in $I$, we will have in $\Psi$ that either $(y_0,y_{2s})=(0,2)$ or $(y_0,y_{2s})=(2,0)$. 
%## Barny. It is not really symmetric since we send y_k to 0.
% Thus it should be always (0,2)
% fixed
Recall $(y_0,y_{2s})=(0,2)$. After Existential has played a winning strategy in $I$, suppose that it is the triple $(x_{a_j},x_{b_j},x_{c_j})$ that is either $(0,0,0)$ or $(1,1,1)$. 
%## BARNY. The sentence below should be different for 
% (0,0,0) and (1,1,1).
% fixed
If it is $(0,0,0)$, then we evaluate $y_i$ as $0$ for $0 \le i \le j$ and $2$ for $j < i \le 2s$. If it is $(1,1,1)$, then we evaluate $y_{i}$ as $0$ for $0 \le i \le s+j$ and $2$ for $s+j < i \le 2s$ 
Then set $t_n,\ldots,t_0=2$ and $z_n,\ldots,z_0=1$. Finally, $y_k=0$ and $y_l=2$.

($\Psi \in \QCSP(\{\sigma,\sigma_0,\sigma_1\})$ implies $I\in \mathrm{co\mbox{-}QNAE3SAT}$.) Let us consider only evaluations of $\Psi$ in which each $(x^0_i,x^1_i)$ is either $(0,1)$ or $(1,0)$.  We play through the simulation quantifiers of $\Psi$ copying what is chosen in $I$.  We must have $z_n,\ldots,z_0=1$, $t_n,\ldots,t_0=2$, $y_l=2$ due to the constraints $y_k=0\wedge y_l=t_0 \wedge \sigma(t_n,z_n) \wedge z_0=1$. Furthermore, let us assume Universal plays $(x^0_i,x^1_i)$ that came from existential variables of $I$ according to their selecting $y_k$. It follows that $y_0\neq y_{2s}$ and there must be a $0 \le i \le 2s$ so that $y_i\neq y_{i+1}$. This then selects some triple of $I$ that is either $(0,0,0)$ (if $i<s$) or $(1,1,1)$ (if $i\ge s$).

Now let us show what adjustments need to be made for the problem $\QCSP(\{\sigma'_0,\sigma_1\})$ (the case $\QCSP(\{\sigma_0,\sigma'_1\})$ is symmetric). We replace $\Delta_0$ with 
\[ \Delta'_0 = \bigwedge_{1 \le i \le n} \left( \sigma'_0(x^0_i,z_{i-1},z_i) \wedge \sigma'_0(x^1_i,z_{i-1},z_i) \right) \]
and build the final instance of $\Psi$ according to
\[ y_k=0 \wedge \Phi \wedge y_l=t_0 \wedge \Delta_1 \wedge t_n=z_n \wedge \Delta'_0 \wedge z_0=2 \]
where we make this prenex and add quantifiers $\exists t_0 \ldots \exists t_n \exists z_0 \ldots \exists z_n \exists y_k \exists y_l$ innermost. 

($I\in \mathrm{co\mbox{-}QNAE3SAT}$ implies $\Psi \in \QCSP(\{\sigma'_0,\sigma_1\})$.) Let us begin by arguing that if Universal at any point plays some $x^0_i=x^1_i$ or $x^0_i,x^1_i =2$ then Existential will surely win. Suppose some $x^0_i=x^1_i=0$, then we know $\Delta'_0$ holds on a tuple with $(z_0,z_n)=(0,2)$. It doesn't matter how the simulation quantifiers have been evaluated, we just set $t_n,\ldots,t_0=0$ and $y_k,\ldots,y_l=0$ (and evaluate the $z_i$ in between $z_0$ and $z_n$ as in the tuples that satisfies $\Delta'_0$). Suppose some $x^0_i=x^1_i=1$, then we know $\Delta_1$ holds on a tuple with $(t_0,t_n)=(0,2)$. Set $z_n,\ldots,z_0=2$ and $y_k,\ldots,y_l=0$. 
%## BARNY Below, it is probably not clear that by 
% x_{j}^{0},x_{j}^{1}=2 you mean that just one of them is equal to 2.
% fixed
Suppose now some $x^0_j=2$ or $x^1_j=2$, we find  again that $\Delta'_0$ holds on a tuple with $(z_0,z_n)=(0,2)$
or $\Delta_1$ holds on a tuple with $(t_0,t_n)=(0,2)$.
%## BARNY. The case below was already considered.
% fixed
%while if  (for any $i$) $x^0_i=x^1_i=1$, then $\Delta_1$ holds on a tuple with $(t_0,t_n)=(0,2)$. 
Thus, we reduce to previous cases.

We now know that Universal must play each $(x^0_j,x^1_j)$ as either $(0,1)$ or $(1,0)$ if he is to have any chance of winning on $\Psi$. We have assumed Existential has a winning strategy in $I$ and this can be copied in $\Psi$ according to how we described the rules for how each $\exists y_k \forall x^0_i \forall x^1_i \exists y_l$ selects either  $(x^0_i,x^1_i)=(0,1)$ or $(x^0_i,x^1_i)=(1,0)$.  After the quantifiers are played in $I$, we will have in $\Psi$ that either $(y_0,y_{2s})=(0,2)$ or $(y_0,y_{2s})=(2,0)$. 
%## Barny. It is not really symmetric since we send y_k to 0.
% Thus it should be always (0,2)
Recall $(y_0,y_{2s})=(0,2)$. After Existential has played a winning strategy in $I$, suppose that it is the triple $(x_{a_j},x_{b_j},x_{c_j})$ that is either $(0,0,0)$ or $(1,1,1)$. 
%## BARNY. The sentence below should be different for 
% (0,0,0) and (1,1,1).
% fixed
If it is $(0,0,0)$, then we evaluate $y_i$ as $0$ for $0 \le i \le j$ and $2$ for $j < i \le 2s$. If it is $(1,1,1)$, then we evaluate $y_{i}$ as $0$ for $0 \le i \le s+j$ and $2$ for $s+j < i \le 2s$ 
Then set $t_n,\ldots,t_0=2$ and $z_n,\ldots,z_0=2$. Finally, $y_k=0$ and $y_l=2$.

($\Psi \in \QCSP(\{\sigma'_0,\sigma_1\})$ implies $I\in \mathrm{co\mbox{-}QNAE3SAT}$.) Let us consider only evaluations of $\Psi$ in which each $(x^0_i,x^1_i)$ is either $(0,1)$ or $(1,0)$.  We play through the simulation quantifiers of $\Psi$ copying what is chosen in $I$.  We must have $z_n,\ldots,z_0=2$, $t_n,\ldots,t_0=2$, $y_l=2$ due to the constraints $y_k=0\wedge y_l=t_0 \wedge t_n=z_0 \wedge z_n=2$. Furthermore, let us assume Universal plays $(x^0_i,x^1_i)$ that came from existential variables of $I$ according to their selecting $y_k$. It follows that $y_0\neq y_{2s}$ and there must be a $0 \le i \le 2s$ so that $y_i\neq y_{i+1}$. This then selects some triple of $I$ that is either $(0,0,0)$ (if $i<s$) or $(1,1,1)$ (if $i\ge s$).
\end{proof}

By $\QCSP^{2}(\Gamma)$ recall we denote the decision problem 
where the input in a $\QCSP(\Gamma)$ instance
is a $\Pi_{2}$ formula, that is a formula of the form $\forall x_1 \dots\forall x_{n} \exists y_1\dots\exists y_s \Phi.$


%By $h_{0}$ we denote the operation such that $h_{0}(0,1) %= 0$, $h_{0}(a,a) = a$ and it returns 2 otherwise.
%Similarly, by $h_{1}$ we denote the operation such that %$h_{1}(1,0) = 1$, $h_{1}(a,a) = a$ and it returns 2 %otherwise.




The following lemma shows that using 
0-stable and 1-stable operations we can reduce 
$\QCSP(\Gamma)$ to $\QCSP^{2}(\Gamma)$.


\begin{lem}\label{ReductionToQCSP2}
Suppose $\Gamma$ is preserved by $s_2$ and a 0-stable operation $h_{0}$.
Then an instance 
$$\forall x_1\exists y_1 \forall x_2 \exists y_2 \dots \forall x_{n} \exists y_{n} \Phi$$
of $\QCSP(\Gamma)$ is equivalent to 
$$\forall x_1\forall x_2 \dots \forall x_{n}
\exists \exists  
((\exists' \exists '\Phi_{1})\wedge 
(\exists' \exists' \Phi_2) \wedge \dots \wedge (\exists' \exists' \Phi_n)),$$
where $$\Phi_{i} = \Phi^{x_{i+1},\ldots,x_{n}, y_{i+1},\ldots,y_{n}}_{x_{i+1}',\ldots,x_{n}',y_{i+1}',\ldots,y_{n}'} \wedge x_{i+1}' = 0 \wedge \dots\wedge x_{n}' = 0,$$
(note that $\Phi_{n} = \Phi$) and by 
$\exists \exists$ and $\exists' \exists'$ we mean that we add all necessary existential quantifiers for variables without primes and with primes, respectively.
\end{lem}

\begin{proof}
(Forwards/ downwards.)
If we have a solution $(f_1,\ldots,f_{n})$ of the original instance then it is 
also a solution of the new instance with the additional assignments $x_{j}' = 0$ and $y_{j}' = 
f_{j}(x_{1},\ldots,x_{i},0,\ldots,0)$ 
in the definition of $\Phi_{i}$ for every $j$.
%To get $\Phi_{i}$ form the original instance 
%we just assign $x_{j} = 0$ for every $j>i$, 
%which is obviously weaker than the original instance.


(Backwards/ upwards.)
Consider solutions of the new instance
such that 
$y_{i} = f_{i}(x_{1},\ldots,x_{n})$
for every $i$.
Let $N$ be the minimal number such that 
$f_{N}$ depends on $x_{j}$ for some $j>N$. In fact, we would like that there is some solution such that this number does not exist as then this is also a solution of the original instance. But for now assume for contradiction that such an $N$ does exist and we choose it to be minimal among all the solutions.
Since 
$(f_{1},\ldots,f_{n})$ is also a solution of $\Phi_{N}$, 
the following tuple is a solution of $\Phi$
$$(x_{1},\ldots,x_{N},0,\ldots,0,
f_{1}(x_{1},\ldots,x_{n}),\ldots,
f_{N}(x_{1},\ldots,x_{n}),h_{N+1}(x_{1},\ldots,x_{n}),
\ldots,h_{n}(x_{1},\ldots,x_{n}))$$
for every $x_{1},\ldots,x_{n}$ and some functions $h_{N+1},\ldots, h_{n}$. Note that we could see this tuple (with an additional term written and another omitted) rather as
$$(x_{1},\ldots,x_{N},0,\ldots,0,
f_{1}(x_{1}),\ldots,f_{N-1}(x_{1},\ldots,x_{N-1}),
f_{N}(x_{1},\ldots,x_{n}),h_{N+1}(x_{1},\ldots,x_{n}),
\ldots)$$
as we assume $f_i$ depends only on $x_1,\ldots,x_i$ for $i\le N$.
Consider all the evaluations of the variables 
$x_{N+1},\ldots,x_{n}$ to obtain $3^{n-N}$ solutions of $\Phi$, 
then apply the semilattice operation to them to obtain 
one solution $\alpha(x_{1},\ldots,x_{N})$ of the form
$$(x_{1},\ldots,x_{N},0,\ldots,0,
f_{1}(x_{1},\ldots,x_{n}),\ldots,
f_{N-1}(x_{1},\ldots,x_{n}),
e_{N}(x_{1},\ldots,x_{N}),
%g_{N+1}(x_{1},\ldots,x_{N}),
\ldots,e_{n}(x_{1},\ldots,x_{N})).$$
Note that $e_{N}(x_{1},\ldots,x_{N})$ is equal to $c$ if 
$f_{N}(x_{1},\ldots,x_{N},a_{N+1},\ldots,a_{n})=c$ for every $a_{N+1},\ldots,a_{n}$, 
and 
$e_{N}(x_{1},\ldots,x_{N})=2$ otherwise.

It remains to 
apply $h_{0}$ to
$(x_{1},\ldots,x_{n},f_{1}(x_{1},\ldots,x_{n}),\ldots,f_{n}(x_{1},\ldots,x_{n}))$
and 
$\alpha(x_{1},\ldots,x_{N})$ 
to obtain a solution of the instance 
such that $f_{N}$ doesn't depend on $x_{N+1},\ldots,x_{n}$, which gives us a contradiction to the minimality of $N$ over all solutions.
\end{proof}

The next lemma follows from Lemma~\ref{ReductionToQCSP2} and the fact 
that if $\Gamma$ is preserved by a semilattice then $\CSP(\Gamma)$ can be solved in polynomial time.
Nevertheless, to explain how a $0$-stable operation can be used 
in an algorithm we give an alternative proof.

\begin{lem}\label{InCONPForStable}
Suppose $\Gamma$ is preserved by $s_2$ and a 0-stable operation $h_{0}$.
Then 
$\QCSP(\Gamma)$ is in co-NP.
\end{lem}

\begin{proof}
Suppose we have an instance 
$\forall x_1\exists y_1 \forall x_2 \exists y_2 \dots \forall x_{n} \exists y_{n} \Phi$.
We can use an oracle to choose an appropriate value for $x_{1}$ (let this value be $a_{1}$).
Then we need to find an appropriate value for $y_{1}$, such that we can use an oracle for $x_2$ and continue.
We want to be sure that if the instance holds then it holds after fixing $y_{1}$. 

To find out how to fix $y_{1}$ we solve the instance 
$$\exists y_1 \exists x_2 \exists y_2 \dots \exists x_{n} \exists y_{n} \Phi\wedge x_{1} = a_{1} \wedge x_{2} = x_{3}=\dots=x_{n} = 0.$$
This is a CSP instance, which can be solved in polynomial time 
because the semilattice preserves $\Gamma$.
We check whether we have a solution with $y_{1}=0$, $y_{1} =1$, $y_{1}=2$ (we solve three instances).
Let $Y$ be the set of possible values for $y_{1}$.
If $|Y|=1$, then we fix $y_{1}$ with the only value in $Y$. Obviously, 
the fixing of $y_{1}$ cannot transform  
the QCSP instance that holds into an instance that does not hold.
If $|Y|>1$ then $2\in Y$ due to the semilattice polymorphism. 
Let the solution of the CSP instance with $y_{1} = 2$ be 
$(x_{1},y_{1},x_{2},y_{2},\dots,x_{n},y_{n}) = 
(a_{1},2, 0, c_{2},\dots,0, c_{n})$.
Assume that the QCSP instance has a solution 
$(a_{1},f_{1} (a_{1}), x_{2},f_{2}(x_{1},x_{2}), \ldots,x_{n},f_{n}(
x_{1},\ldots,x_n))$.
Then by applying the operation $h_{0}$ to this solution and 
$(a_{1},2, 0, c_{2},\dots,0, c_{n})$,
we get a (partial) solution of the $\QCSP(\Gamma)$
with $y_{1}=2$.

We proceed this way through the quantifier prefix, using an oracle to choose values for  $x_{2}, \ldots,x_{n}$,
while we solve CSP instances to 
choose appropriate values for 
$y_{2},y_{3},\ldots,y_{n}$.
\end{proof}


We say that a ternary relation $R$ is \emph{an AND-type} relation if 
$R\cap (\{0,1\}\times\{0,1\}\times\{0,1,2\})
=\begin{pmatrix}
0&0&1&1\\
0&1&0&1\\
0&0&0&1
\end{pmatrix}$, that is, it is row-wise the truth table of AND.
If $s_2$ preserves $R$, 
then it also contains $(2,2,0)$ and $(2,2,2)$.
We say that a ternary relation $R$ is \emph{an OR-type} relation if 
$R\cap (\{0,1\}\times\{0,1\}\times\{0,1,2\})
=\begin{pmatrix}
0&0&1&1\\
0&1&0&1\\
0&1&1&1
\end{pmatrix}$, that is, it is row-wise the truth table of OR.
Again, if $s_2$ preserves $R$, 
then it also contains $(2,2,1)$ and $(2,2,2)$. One can readily imagine AND/OR-type relations of arity $k+1$ higher than three built from AND/OR operations of arity $k$. 

\begin{lem}\label{ANDORHardness}
Suppose $\Gamma$ contains an AND-type relation and an OR-type relation,
and $\Gamma$ is preserved by $s_2$.
Then $\QCSP(\Gamma)$ is co-NP-hard.
\end{lem}
\begin{proof}

By $R_{and,2}$ and 
$R_{or,2}$ we 
denote an AND-type and an OR-type relation, respectively.
For $n=2,3,4,\dots$ put 
$$R_{and,n+1}(x_{1},\ldots,x_{n},x_{n+1},y) = 
\exists z \;R_{and,n}(x_{1},\ldots,x_{n},z)
\wedge R_{and,2}(x_{n+1},z,y),$$
$$R_{or,n+1}(x_{1},\ldots,x_{n},x_{n+1},y) = 
\exists z \; R_{or,n}(x_{1},\ldots,x_{n},z)
\wedge R_{or,2}(x_{n+1},z,y).$$

Let us define a relation $\xi_{n}$ for every $n$ by
\begin{align*}
\xi_{n}(x_{1},y_{1},z_{1},\dots,
x_{n},y_{n},z_{n})&=
\exists u\exists u_{1}\dots\exists u_{n}
\exists v\exists v_{1}\dots\exists v_{n}\;
R_{and,2}(u,v,v) \wedge \\
R_{and,3}(x_{1},y_{1},z_{1},u_{1})&\wedge
\dots\wedge
R_{and,3}(x_{n},y_{n},z_{n},u_{n})\wedge
R_{or,n}(u_1,\dots,u_{n},u)\wedge\\
R_{or,3}(x_{1},y_{1},z_{1},v_{1})&\wedge
\dots\wedge
R_{or,3}(x_{n},y_{n},z_{n},v_{n})\wedge
R_{and,n}(v_1,\dots,v_{n},v).
\end{align*}

It follows from the definition 
that 
$\xi_{n}\cap \{0,1\}^{3n}$ is defined by
$\mathrm{AE}_3(x_{1},y_{1},z_{1})\vee
\mathrm{AE}_3(x_{2},y_{2},z_{2})\vee
\dots
\vee
\mathrm{AE}_3(x_{n},y_{n},z_{n})$,
where 
$\mathrm{AE}_3 = \{(0,0,0),(1,1,1)\}$.

Suppose 
$R(y_1,\dots,y_{t}) = 
\xi_{n}(y_{i_1},y_{i_{2}},\dots,y_{i_{3n}})$, 
where 
$i_{1},\dots,i_{3n}\in\{1,2,\dots,t\}$.
Let us show that 
$\forall y_{1}\dots\forall y_{t}\;
\xi_{n}(y_{i_1},y_{i_{2}},\dots,y_{i_3n})$
holds if 
$\xi_{n}(y_{i_1},y_{i_{2}},\dots,y_{i_3n})$
holds for all $y_{1},\ldots,y_{t}\in\{0,1\}$.
%Suppose $\xi_{n}(y_{i_1},y_{i_{2}},\dots,y_{i_3n})$
%defines a relation $R$.
We need to prove that if $\{0,1\}^{t}\subseteq R$ then 
$A^{t}\subseteq R$, which follows from the fact that the semilattice $s_2$ preserves $R$.

Now we may encode the complement of \emph{Not-All-Equal 3-Satisfiability} using $\Gamma$.
This complement can be expressed by
a formula of the following form:
$$\forall y_{1}\dots\forall y_{t} \ 
\mathrm{AE}_3(y_{i_1},y_{i_{2}},y_{i_3})\vee
\dots
\vee
\mathrm{AE}_3(y_{i_{3n-2}},y_{i_{3n-1}},y_{i_{3n}}),$$
which is equivalent to 
$$\forall y_{1}\dots\forall y_{t}\;
\xi_{n}(y_{i_1},y_{i_{2}},\dots,y_{i_{3n}}).$$
Thus, we reduced a co-NP-complete problem to $\QCSP(\Gamma)$, which completes the proof.
\end{proof}


\begin{lem}\label{NoStrange2Hardness}
Suppose $\Gamma\subseteq\Inv(s_2)$, 
$\Gamma$
contains 
$\delta(x,y,z) = (x\neq 0)\vee (y=z)$ 
and an AND-type relation $R_{2}$. 
Then $\QCSP(\Gamma)$ is co-NP-hard.
\end{lem}
\begin{proof}
Here we will define a reduction from the complement of 
$\CSP(\{1\mathrm{IN}3\})$, which is known  to be NP-complete \cite{Schaefer},
where 
$1\mathrm{IN}3 = \begin{pmatrix}
1&0&0\\
0&1&0\\
0&0&1
\end{pmatrix}$.
First, 
put 
$$\delta_1(x_1,x_2,x_3,x_4) = \exists t\;\delta(x_1,x_{3},t) \wedge \delta(x_{2},t,x_4).$$
It is not hard to see that 
$\delta_1(x_1,x_2,x_3,x_{4}) = 
(x_{1}\neq 0)\vee 
(x_{2}\neq 0)\vee
(x_{3}=x_{4}).$
Put 
$$\delta_{2}(x_{1},x_{2},x_{3},x_{4}) = 
\delta_{1}(x_{1},x_{2},x_{3},x_{4})
\wedge 
\delta_{1}(x_{1},x_{3},x_{2},x_{4})
\wedge 
\delta_{1}(x_{2},x_{3},x_{1},x_{4}).
$$
By the definition, the first three variables of
$\delta_{2}$ are symmetric.
Suppose $(a,b,c,d)\in\delta_{2}$. 
It is not hard to see that
$a=b=c=0$ implies $d=0$.
Also 
$a=1, b=c=0$ implies $d=1$.
If there are at least two 1s in $(a,b,c)$ then 
$d$ can be arbitrary.
Put $R'(x,y) = R_{2}(x,x,y)$.
By the definition of an AND-type relation, 
$R'$ contains $(0,0),(1,1),(2,2),(2,0)$
but doesn't contain $(0,1),(0,2),(1,0),(1,2)$.
Put
$$\delta_{3}(x_{1},x_{2},x_{3},x_{4}) = 
\exists x_{1}'\exists x_{2}'\exists x_{3}'\;
\delta_{2}(x_{1}',x_{2}',x_{3}',x_{4})
\wedge 
R'(x_{1},x_1')
\wedge 
R'(x_{2},x_2')
\wedge 
R'(x_{3},x_3').$$
Then 
$(a,b,c,0)\in\delta_{3}$
for all tuples $(a,b,c)$ but the tuples from $1\mathrm{IN}3$.

%Let $R_2$ be the AND-type relation.
Again, we apply the recursive 
formula to build an $n$-ary ``and''
$$R_{n+1}(x_{1},\ldots,x_{n+1},z) = 
\exists t\; R_{n}(x_{1},\ldots,x_{n},t)\wedge
R_{2}(t,x_{n+1},z).$$


Define 
$\zeta_{n}(x_{1},\ldots,x_{3n})$ by
$$\exists z_{1}\dots\exists z_{n}\exists t\;
R_{n}(z_{1},\ldots,z_{n},t)
\wedge 
\delta_{3}(x_{1},x_{2},x_{3},z_{1})\wedge
\dots\wedge \delta_{3}(x_{3n-2},x_{3n-1},x_{3n},z_{n})
\wedge (t=0).
$$

Now we may encode the complement of $\CSP(\{1\mathrm{IN}3\})$ using $\Gamma$. If $\overline{1\mathrm{IN}3}$ is the complement of $1\mathrm{IN}3$ with respect to $\{0,1\}^3$, then we use
a formula of the following form:
$$\forall y_{1}\dots\forall y_{t} \ 
\overline
{1\mathrm{IN}3}(y_{i_1},y_{i_{2}},y_{i_3})\vee
\dots
\vee
\overline{1\mathrm{IN}3}(y_{i_{3n-2}},y_{i_{3n-1}},y_{i_{3n}}),$$
which is equivalent to 
$$\forall y_{1}\dots\forall y_{t}\;
\xi_{n}(y_{i_1},y_{i_{2}},\dots,y_{i_{3n}}).$$
Thus, we reduced a co-NP-complete problem to $\QCSP(\Gamma)$, which completes the proof.
\end{proof}

==> old/ThreeElementCorrection.tex <==
\subsection{Finiteness of the language 2}


Put $N = k+1$.
First, we define a matrix $M$ whose columns are all different tuples from $\{0,1\}^{N}$.

Put $N = 2^{k+1}-2$.
For $i=0,1,\dots,N$ by 
$\beta_{i}$ we denote binary representation of the number $i$
of length $k+1$.
Thus, $\beta_{i}(j)$ is the $j$-th bit of the number $i$.
By $M$ we denote the matrix, whose columns are
$\beta_{0},\dots,\beta_{N}$.
Note that there is no column
$11\dots 11$ in the matrix.

By $f_{1}$ we denote the operation of arity $N+1$ that 
returns 1 on rows of the matrix $M$, and returns $2$ otherwise.

\begin{lem}
Suppose $f_{1}$ is not $\{0,2\}\{1,2\}$-projective. 
\end{lem}

\begin{proof}
If $f_{1}$ is $\{0,2\}\{1,2\}$-projective then there should be $i$ such that 
$f_{1}$ always returns the $i$-th variable or 2.
Since the column $11\dots 11$ is not in the matrix
and $f_{1}$ applied to $M$ gives $11\dots 11$, 
we get a contradiction.
\end{proof}

\begin{lem}
There exists an AND-type, OR-type, $\oplus$-type relation, or NOT-type relation in 
$\Gamma$.
\end{lem}
\begin{proof}
Since $f_{1}$ is not $\{0,2\}\{1,2\}$-projective, there should be a relation in $\Gamma$ that is not preserved by $f_{1}$.
Let $\rho$ be a relation of the minimal arity that is not preserved by $f_{1}$.
Let $l$ be the arity of $\rho$,
$\alpha_{0},\ldots,\alpha_{N}\in\rho$ and 
$f_{1}(\alpha_{0},\ldots,\alpha_{N})=\beta\notin\rho$.

We consider the matrix $M'$ 
whose columns are $\alpha_{0},\dots,\alpha_{N}$. 
Since $\rho$ is a relation of the minimal arity, every row should contain different elements and 
all rows of the matrix should be different. 
Also (see the proof of Lemma~\ref{almostNU} for the detailed explanation), 
for every $i$ there should be a tuple $\beta_{i}\in\rho$ such that 
$\beta_{i}$ differs from $\beta$ only in the $i$-th coordinate.

Assume that $\beta$ has at least two elements equal to $2$ and they appear at the $i$-th and $j$-th positions.
Then $s(\beta_{i},\beta_{j}) = \beta$, which contradicts the fact that 
$s$ preserves $\rho$.
Assume that $\beta$ has no $2$. 
Then every row of the matrix $M'$ should be 
a row of the matrix $M$. 
We know that $M'$ has less rows than $M$, therefore
$M'$ should contain all tuples (as columns) of length $l$ including $\beta$, 
which gives a contradiction.

Then each consists of $2k$ pairs $(1,0)$ and $(0,1)$, where one of these pairs may appear at most once in every row.
Therefore, since we have $N\le k$ rows and $2k$ pairs, there should be a column among $\alpha_{1},\ldots,\alpha_{2k}$ equal to $\beta$, which contradicts our assumptions.
W.l.o.g., we assume that $\beta(N) = 2$.

Put $\alpha_{i}' = \proj_{1,\ldots,N-1}(\alpha_{i})$ 
for every $i$, $\beta' = \proj_{1,\ldots,N-1}(\beta)$.
For every $i\in\{1,\dots,N-1\}$ the $i$-th row contains at most one pair different from the others.
Since $N\le k$, at least $k+1$ of the tuples 
$\alpha_{1}',\ldots,\alpha_{2k}'$ are equal to $\beta'$.
W.l.o.g., we assume that 
$\alpha_{s+1}' = \dots = \alpha_{2k}' = \beta'$, $\alpha_{i}'\neq\beta'$ 
for every $i\in\{1,\ldots,s\}$, where $s< N$.  
Since $\beta(N)=2$ and $s$ preserves $\rho$, we also obtain 
$\alpha_{s+1} = \dots = \alpha_{2k}$.



\end{proof}



Below we define two operations similar to 
$nu_{B,C}^{n}$, which will be used to derive 
AND-type and OR-type relations.

By $nu_{10}^{n}$
we denote 
the operation of arity $2n$ defined on a tuple 
$(a_1,b_{1},a_2,b_2,\ldots,a_n,b_{n})$ as follows. 
If $a_{1} = \dots = a_n=b_{1}=\dots=b_n$ then return $a_1$.
If 
$(a_{1},b_{1})=\dots=(a_{i-1},b_{i-1}=
a_{i+1},b_{i+1})=\dots=(a_{n},b_{n}) = (1,0)$,
$(a_{i},b_{i})\in\{(0,1),(1,0)\}$ for some $i$, then return 
$1$. Otherwise, it return $2$.

By $nu_{0110}^{n}$
we denote 
the operation of arity $2n$ defined on a tuple 
$(a_1,b_{1},a_2,b_2,\ldots,a_n,b_{n})$ as follows. 
If $a_{1} = \dots = a_n=b_{1}=\dots=b_n$ then return $a_1$.
If 
$(a_{1},b_{1})=\dots=(a_{i-1},b_{i-1}=
a_{i+1},b_{i+1})=\dots=(a_{n},b_{n})\in\{(0,1),(1,0)\}$,
$(a_{i},b_{i})\in\{(0,1),(1,0)\}$ for some $i$, then return 
$a_{j}$ for $j\neq i$. Otherwise, it return $2$.

Similar to Lemma~\ref{almostNU} we will prove the following lemma.

\begin{lem}\label{almostf}
Suppose $\Gamma$ is not preserved by 
$f\in\{nu_{10}^{2k},nu_{0110}^{2k}\}$.
Then there exists a relation $\rho\in \Gamma\setminus \Inv(f)$ of arity $N$ 
such that 
one of the following conditions holds:
\begin{enumerate}
    \item There exist 
    $\alpha_{1},\gamma_{1},\alpha_{2},\gamma_{2},\alpha_{3},\gamma_{3}\in\rho$ 
    such that 
    $f(\alpha_{1},\gamma_{1},\alpha_{2},\gamma_{2},\alpha_{3},\gamma_{3},\ldots,\alpha_{3},\gamma_{3}) = \beta\notin\rho$, 
    $\beta(i) = \alpha_{3}(i)\neq 2$ for $i\in\{1,\ldots,N-1\}$, 
    $\beta(N) = 2$,
    $\alpha_{1}(N) = \alpha_{2}(N) =
    \gamma_{3}(N)\neq 
        \gamma_{1}(N) = \gamma_{2}(N) =
    \alpha_{3}(N)$.
    Moreover, if $f=nu_{10}^{2k}$ then 
    $\alpha_{1}(N)=0$.    
    \item 
    There exist $\alpha_{1},\gamma_{1},\alpha_{2},\gamma_{2}\in\rho$ 
    such that 
    $f(\alpha_{1},\gamma_{1},\alpha_{2},\gamma_{2},\dots,\alpha_{2},\gamma_{2}) = \beta\notin\rho$,
    $\beta(i) = \alpha_{2}(i)\neq 2$ for every $i\in\{1,\ldots,N-1\}$, 
    $\beta(N) = 2$. 
\end{enumerate}
Additionally, $\rho$ is a relation of the minimal arity in $\Gamma$ that is not preserved by $f$.
\end{lem}

\begin{proof}
We assume that $\rho$ is a relation of the minimal arity that is not preserved by $f$.
Let $N$ be the arity of $\rho$. 
Consider tuples 
$\alpha_{1},\gamma_{1},\ldots,\alpha_{2k},\gamma_{2k}\in\rho$ such that 
$f(\alpha_{1},\gamma_{1},\ldots,\alpha_{2k},\gamma_{2k})=\beta\notin \rho$.
Arguing as in Lemma~\ref{almostNU} we can show that 
for every $i$
there exists a tuple $\beta_{i}\in\rho$ that differs from $\beta$ only in the $i$-th coordinate. 

We consider the matrix $M$ 
whose columns are $\alpha_{1},\gamma_{1},\ldots,\alpha_{2k},\gamma_{2k}$. 
Since $\rho$ is a relation of the minimal arity, every row should contain different elements and 
all rows of the matrix should be different.

Assume that $\beta$ has at least two elements equal to $2$ and they appear at the $i$-th and $j$-th positions.
Then $s(\beta_{i},\beta_{j}) = \beta$, which contradicts the fact that 
$s$ preserves $\rho$.
Assume that $\beta$ has no $2$. 
Then each consists of $2k$ pairs $(1,0)$ and $(0,1)$, where one of these pairs may appear at most once in every row.
Therefore, since we have $N\le k$ rows and $2k$ pairs, there should be a column among $\alpha_{1},\ldots,\alpha_{2k}$ equal to $\beta$, which contradicts our assumptions.
W.l.o.g., we assume that $\beta(N) = 2$.

Put $\alpha_{i}' = \proj_{1,\ldots,N-1}(\alpha_{i})$ 
for every $i$, $\beta' = \proj_{1,\ldots,N-1}(\beta)$.
For every $i\in\{1,\dots,N-1\}$ the $i$-th row contains at most one pair different from the others.
Since $N\le k$, at least $k+1$ of the tuples 
$\alpha_{1}',\ldots,\alpha_{2k}'$ are equal to $\beta'$.
W.l.o.g., we assume that 
$\alpha_{s+1}' = \dots = \alpha_{2k}' = \beta'$, $\alpha_{i}'\neq\beta'$ 
for every $i\in\{1,\ldots,s\}$, where $s< N$.  
Since $\beta(N)=2$ and $s$ preserves $\rho$, we also obtain 
$\alpha_{s+1} = \dots = \alpha_{2k}$.

If $s=0$, then the second condition of this lemma holds.

Suppose $s\ge 1$.
In the same way as in the proof of Lemma~\ref{almostNU} 
we substitute $\alpha_{j}$ instead of $\alpha_{i}$ 
for any $i\in\{1,\dots,s\}$ and $j\in\{s+1,\dots,2k\}$.
We assume 
$f_{B,C}^{n}(\alpha_{0},\dots,\alpha_{i-1},\alpha_{j},\alpha_{i+1},\dots,\alpha_{2k})\in\rho$, since otherwise we may replace $\alpha_{i}$ by $\alpha_{j}$ 
and reduce $s$.
We therefore conclude that 
$2k-2$ elements among the elements 
$\alpha_{1}(N),\dots,\alpha_{i-1}(N),\alpha_{i+1}(N),\dots,\alpha_{2k}(N)$ 
are equal to $\alpha_{j}(N)$.
Since $\beta(N) = 2$, we also have
$\alpha_{i}(N)\neq\alpha_{j}(N)$.
This implies that 
$\alpha_{s+1}(N) = \dots = \alpha_{2k}(N)\in B$, 
and one of the following cases holds, which completes the proof:
\begin{enumerate}
    \item $s = 1$, $\alpha_{2} = \dots = \alpha_{2k}$;
    \item $s = 2$, $\alpha_{1}(N),\alpha_{2}(N)\in C$,
    $\alpha_{3} = \dots = \alpha_{2k}$.
\end{enumerate}
\end{proof}

\subsection{Connection with Boolean functions}

A mapping $f:\{0,1\}^{n}\to\{0,1\}$ is called \emph{a Boolean function}.
We say that 
a Boolean function $f$ of arity $n$ is represented by $\Gamma$
if there exists a relation $R$ of arity $n+1$ pp-definable using $\Gamma$
such that for 
all $a_{1},\ldots,a_{n}\in\{0,1\}$
$$(a_{1},\ldots,a_{n},b)\in R\Rightarrow b = f(a_{1},\ldots,a_{n}).$$
Thus, an AND-type relation is a representation of conjunction, 
an OR-type relation is a representation of disjunction.


\subsection{Remove}

\begin{lem}\label{ANDAlmostAlways}
Suppose $\Gamma$ is preserved by a 0-stable operation.
Then $\Gamma$ contains an 
AND-type relation or 
the relation $\begin{pmatrix}
0& 1& 2\\
1& 0& 2
\end{pmatrix}$.
\end{lem}

\begin{proof}
%Let us define a $(2k+1)$-ary operation $f$.
%It returns $1$ on the tuples 
%$01^i01^{2k-i-1}$,  for $i=0,1,\dots,2k-1,$
%and $0 1^{2k}$. It returns $2$ otherwise.
%This operation is not $\{0,2\}\{1,2\}$-projective, 
%therefore there should be a relation $\rho$ in $\Gamma$ that is not preserved by $f$.

Since $f_{\{1\},\{0\}}^{2k}$ is not $\{0,2\}\{1,2\}$-projective,
$\Gamma$ is not preserved by $f_{\{1\},\{0\}}^{2k}$.
By Lemma \ref{almostf} there exists a relation $\rho\in\Gamma$
satisfying one of the two cases (see notations in Lemma~\ref{almostf}).

%We are going to argue in the same way as in the proof of Lemma~\ref{almostNU}.
%We assume that $\rho$ is a relation of the minimal arity that is not preserved by $f$.
%Let $N$ be the arity of $\rho$. 
Consider tuples 
$\alpha_{0},\alpha_{1},\ldots,\alpha_{2k}\in\rho$ such that 
$f(\alpha_{0},\alpha_{1},\ldots,\alpha_{2k})=\beta\notin \rho$.
Put $\alpha_{i}' = \proj_{1,\ldots,N-1}(\alpha_{i})$ 
for every $i$, $\beta' = \proj_{1,\ldots,N-1}(\beta)$.
Since $\rho$ is a relation of the minimal arity 
for every $i$ there exists $\beta_{i}\in\rho$ that differs 
from $\rho$ only in the $i$-th coordinate.

We consider a matrix $M$ whose columns 
are $\alpha_{0},\dots,\alpha_{2k}$.
As in the proof of Lemma~\ref{almostNU} we
can show that 
every row of this matrix contains different elements, and 
all rows should be different.

Assume that $\beta$ has at least two elements equal to $2$ and they appear at the $i$-th and $j$-th positions.
Then $s(\beta_{i},\beta_{j}) = \beta$, which contradicts the fact that 
$s$ preserves $\rho$.
Assume that $\beta$ has no $2$. 
Every row of the matrix must have exactly one element different from all other elements,
and the result of applying $f$ to every row is the popular element of the row. Since we have $N\le k$ rows and $2k$ columns, there should be a column among $\alpha_{1},\ldots,\alpha_{2k}$ equal to $\beta$, which contradicts our assumptions.
W.l.o.g., we assume that $\beta(N) = 2$ 
(otherwise we just permute variables of $\rho$).


Put $\alpha_{i}' = \proj_{1,\ldots,N-1}(\alpha_{i})$ 
for every $i$, $\beta' = \proj_{1,\ldots,N-1}(\beta)$.
We know that for every $i\in\{1,\dots,N-1\}$ the $i$-th row contains exactly one element different from the others.
Since $N\le k$, at least $k+1$ of the tuples 
$\alpha_{1}',\ldots,\alpha_{2k}'$ are equal to $\beta'$.
W.l.o.g., we assume that 
$\alpha_{s+1}' = \ldots = \alpha_{2k}' = \beta'$, $\alpha_{i}'\neq\beta'$ 
for every $i\in\{1,\ldots,s\}$, where $s< N$.  
Since not all elements of the first row of the matrix are equal, 
we have $s\ge 1$.

Replace the first column of the matrix $M$ by $\alpha_{2k}$
and consider 
$nu_{B,C}^{2k}(\alpha_{2k},\alpha_{2},\alpha_{3},\ldots,\alpha_{2k}) 
= \gamma_{1}$.
Since $\alpha_{1}'\neq \beta'$, there should be a row
in the new matrix whose elements are equal.
Therefore, $\gamma_{1}\in\rho$, otherwise 
we consider $\alpha_{2k},\alpha_{2},\alpha_{3},\ldots,\alpha_{2k}$
instead of the original sequence, and get a contradiction 
with the fact that every row should contain at least two different elements.
By the definition $\proj_{1,\ldots,N-1}(\gamma_{1}) = \beta'$, 
therefore $\gamma_{1}(N)\neq 2$.
This means that 
at least $2k-2$ among the elements
$\alpha_{2}(N),\ldots,\alpha_{2k}(N)$ are equal 
to $\alpha_{2k}(N)$.
In the same way we can substitute $\alpha_{j}$ instead of $\alpha_{i}$ 
for any $i\in\{1,\dots,s\}$ and $j\in\{s+1,\dots,2k\}$ to conclude that 
$2k-2$ elements among the elements 
$\alpha_{1}(N),\dots,\alpha_{i-1}(N),\alpha_{i+1}(N),\dots,\alpha_{2k}(N)$ 
are equal to $\alpha_{j}(N)$.
Since $\beta(N) = 2$, we also have
$\alpha_{i}(N)\neq\alpha_{j}(N)$.
This implies that 
$\alpha_{s+1}(N) = \dots = \alpha_{2k}(N)\in B$, 
and one of the following cases holds:
\begin{enumerate}
    \item $s = 1$, $\alpha_{2} = \dots = \alpha_{2k}$;
    \item $s = 2$, $\alpha_{1}(N),\alpha_{2}(N)\in C$,
    $\alpha_{3} = \dots = \alpha_{2k}$.
\end{enumerate}
If $s=1$ then $\alpha_{1}(i)\neq \alpha_{2}(i)$ since there should be different elements in every row.


From the proof of Lemma~\ref{almostNU} we know that 
\begin{enumerate}
    \item $\beta$ is an essential tuple and $\rho$ is an essential relation.
    \item In any row of the matrix there should be elements that are not equal.
    \item $\beta(N) = 2$, $\beta_{i}\neq 2$ for $i\neq N$.
    \item $\alpha_{s+1}' = \ldots = \alpha_{2k}' = \beta'$, 
    $\alpha_{i}'\neq\beta'$ for every $i\in\{1,\ldots,s\}$.      
    \item $s=1$ and $N=2$ and $\beta = 12$, or 
    $s=2$, $N=3$ and $\alpha_{0}(3)=0$, $\alpha_{1}(3) =\alpha_{2}(3) = 0$, $\alpha_{3}(3) = \dots=\alpha_{2k}(3)=1$
    and $\beta = 112$.
\end{enumerate}
(I believe we need to make Lemma~\ref{almostNU} stronger to be able to apply it here).

We consider two cases from the last item.
Suppose the relation $\rho$ is binary.
Then it has tuples
$(0,c),(1,d)$ for some $c$ and $d$ but it doesn't have a tuple 
$(1,2)$. 
Since a $0$-stable operation applied to 
$(1,d)$ and $(0,2)$ gives $(1,2)$, we have $(0,2)\notin\rho$.
Since the semilattice preserves $\rho$ 
We cannot have both $(0,1)$ and $(0,0)$ in $\rho$.
Also we cannot have both $(1,1)$ and $(1,0)$ in $\rho$.

Assume that $c=d$. Then $\beta(2) = c$, which contradicts our assumptions.
Assume that $c=0$ and $d=1$, then $\beta(2) = d$, which also contradicts our assumptions.
Therefore, $c=1$ and $d=0$.
Put $\rho'(x,y) = \rho(x,y)\wedge \rho(y,x)$. 
It is not hard to see that 
$\rho'=\begin{pmatrix}
0& 1& 2\\
1& 0& 2
\end{pmatrix}$, which completes this case.

Suppose the relation $\rho$ is ternary.
Then $\rho$ contains the following tuples
$(0,0,0),(1,1,1),(0,1,0),(1,0,0)$, but doesn't contain the tuple
$(1,1,2)$.
Since $\rho$ is preserved by a 0-stable operation, 
$(c,d,2)\notin\rho$ for all $c,d\in\{0,1\}$ (otherwise we apply the 0-stable operation to 
$(1,1,1)$ and $(c,d,2)$ to get a contradiction).
Thus $\rho$ is an AND-type relation.
\end{proof}

\begin{lem}\label{ANDInTheRemaining}
Suppose 
$\delta=\begin{pmatrix}
0& 1& 2\\
1& 0& 2
\end{pmatrix}\in\Gamma$,
then there exists an AND-type relation and an OR-type relation 
in $\Gamma$.
\end{lem}

\begin{proof}
Let us consider an operation 
$f$ of arity $2k+1$ such that 
$f(01^{i}01^{2k-i-1}) = 1$,
$f(10^{i}10^{2k-i-1}) = 0$,
$f(01^{2k}) = 1$,
$f(10^{2k}) = 0$,
and $f$ returns 2 on all other tuples.

Since $f$ is not $\{0,2\}\{1,2\}$- projective, there should be a relation in $\Gamma$ 
that is not preserved by $f$.
Then we do the same as in Lemma~\ref{almostNU}.
%As a result we get a relation $\rho$ which is either binary or ternary.
To consider less cases, we may assume that $\beta$ consists of $1$ and $2$.
If $\beta(i) =0$ then instead of $\rho$ 
we consider the relation
$$\rho'(x_{1},\ldots,x_{N}) = \exists z
\rho(x_{1},\ldots,x_{i-1},z,x_{i+1},\ldots,x_{N})
\wedge \delta(z,x_{i}).$$
It is not hard to see that $\rho'$ satisfies all the properties we required from $\rho$.

Arguing as in Lemma~\ref{almostNU} we can show that 
$\rho$ is either binary or ternary.

Assume that $\rho$ is binary. Then it contains 
$(0,c)$, $(1,d)$ for some $c$ and $d$, but it 
doesn't contain $(1,2)$. 
Arguing as in the previous lemma we obtain $c=1$ and $d=0$. 
But then we get a contradiction with the fact that 
$\beta(2) = 2$ (since $f$ preserves the permutation $\delta$).

Thus $\rho$ should be a ternary relation containing 
$(0,0,0),(1,1,1),(0,1,0),(1,0,0)$. 
Arguing as in the previous lemma we show that 
$\rho$ is an AND-type relation.
\end{proof}

==> old/ThreeElements.tex <==
\section{EGP and WNU on 3-element domain}

In this section we consider constraint languages for which
$\Pol(\Gamma)$ has the EGP property and contains a WNU operation.
It can be shown (see the proof of Theorem~\ref{ThreeElementClassification})
that in this case $\Pol(\Gamma)$ contains a semilattice operation.
Thus, in this section we have the following assumptions:
\begin{enumerate}
    \item $\Gamma$ is a finite constraint language on $A = \{0,1,2\}$
    \item $\Gamma$ contains the relations $\{0\},\{1\},\{2\},\{0,2\},\{1,2\}$ 
    and the equality relation.
    \item $\Gamma$ is preserved by the semilattice operation $s_2$
    \item $\Pol(\Gamma)$ is $\{0,2\}\{1,2\}$-projective
    
    \item all relations in $\Gamma$ are of arity at most $k\ge 4$
    \item $\Gamma$ contains all relations of arity at most $k$
    that can be pp-defined from $\Gamma$
\end{enumerate}




\subsection{Finiteness of the language}
In this subsection we will derive some properties of 
$\Gamma$ based on the facts that 
$\Gamma$ is finite and 
$\Pol(\Gamma)$ is $\{0,2\}\{1,2\}$-projective.

For $B,C\subseteq A$ and $n\ge 3$ by $nu_{B,C}^{n}$ we denote 
the operation of arity $n$ defined on a tuple 
$(a_1,\ldots,a_n)$ as follows. 
If $a_{1} = \dots = a_n$ then it returns $a_1$.
If $a_{1} = \dots = a_{i-1} = a_{i+1} =\dots = a_n\in B$
and 
$a_{i}\in C$ for some $i$, then it returns $a_{j}$ for $j\neq i$.
Otherwise, it returns $2$.

\begin{lem}\label{almostNU}
Suppose $\rho$ is a relation of the minimal arity $N$ in $\Gamma$ 
that is not preserved by $nu_{B,C}^{2k}$.
%there exists a relation $\rho\in \Gamma\setminus \Inv(nu_{B,C}^{2k})$ of arity $N$ 
%such that 
Then, after some permutation of variables, $\rho$ satisfies one of the following conditions:
\begin{enumerate}
    \item There exist $\alpha_{1},\alpha_{2},\alpha_{3}\in\rho$ 
    such that 
    $nu_{B,C}^{2k}(\alpha_{1},\alpha_{2},\alpha_{3},\alpha_{3},\ldots,\alpha_{3}) = \beta\notin\rho$, 
    $\beta(i) = \alpha_{3}(i)\neq 2$ for $i\in\{1,\ldots,N-1\}$, 
    $\beta(N) = 2$, $\alpha_{1}(N),\alpha_{2}(N)\in C$, 
    $\alpha_{3}(N) \in B$, 
    $\alpha_{1}(i)\neq \alpha_{3}(i)$ or $\alpha_{2}(i)\neq \alpha_{3}(i)$ for every $i$.
    Moreover, if $2\in C$, then $\alpha_{1}(i),\alpha_{2}(i)\in\{\alpha_{3}(i),2\}$ for every $i$, 
    $\alpha_{1}(N) = \alpha_{2}(N) = 2$, $N=3$.
    \item 
    There exist $\alpha_{1},\alpha_{2}\in\rho$ 
    such that 
    $nu_{B,C}^{2k}(\alpha_{1},\alpha_{2},\alpha_{2},\ldots,\alpha_{2}) = \beta\notin\rho$, 
    $\beta(i) = \alpha_{2}(i)\neq 2$ for $i\in\{1,\ldots,N-1\}$, 
    $\beta(N) = 2$, %$\alpha_{1}(N)\notin C$, 
    %$\alpha_{3}(N) \in B$,
    $\alpha_{1}(i)\neq \alpha_{2}(i)$ for every $i$.
\end{enumerate}
%Additionally, $\rho$ is a relation of the minimal arity in $\Gamma$ that is not preserved by $nu_{B,C}^{2k}$.
\end{lem}

\begin{proof}
%Let $\rho$ be a relation of the minimal arity in $\Gamma$ that is not preserved by $nu_{B,C}^{2k}$.
%Let $N$ be the arity of $\rho$. 
Consider tuples 
$\alpha_{1},\ldots,\alpha_{2k}\in\rho$ such that 
$nu_{B,C}^{2k}(\alpha_{1},\ldots,\alpha_{2k})=\beta\notin \rho$.
Since $\rho$ is of the minimal arity, 
$nu_{B,C}^{2k}$ preserves any proper projection of $\rho$.
For example, $nu_{B,C}^{2k}$ preserves $\proj_{1,\ldots,N-1}(\rho)$, 
therefore 
$$nu_{B,C}^{2k}(\proj_{1,\ldots,N-1}(\alpha_1),\ldots,\proj_{1,\ldots,N-1}(\alpha_{2k}))\in \proj_{1,\ldots,N-1}(\rho).$$
Hence, there exists a tuple $\beta_{N}\in\rho$ that differs from $\beta$ only in the $N$-th element. 
Similarly, for every $i$
there exists a tuple $\beta_{i}\in\rho$ that differs from $\beta$ only in the $i$-th element. 
%This means that $\beta$ is an essential tuple and %$\rho$ is an essential relation.

Let us consider the matrix $M$ 
whose columns are $\alpha_{1},\ldots,\alpha_{2k}$. 
Assume that 
for some $j$ we have 
$\alpha_{1}(j) = \dots = \alpha_{2k}(j)$.
Then if we substitute constant 
$\alpha_{1}(j)$ for the $j$-th variable of $\rho$ we get a relation of smaller arity that is not preserved by $nu_{B,C}^{2k}$, which contradicts our assumptions.
Therefore in any row of the matrix there should be elements that are not equal.
Also, all rows of the matrix should be different, since otherwise we
can identify the corresponding variables of $\rho$ to obtain 
a relation of smaller arity that is not preserved by 
$nu_{B,C}^{2k}$.

Assume that $\beta$ has at least two elements equal to $2$ and they appear at the $i$-th and $j$-th positions.
Then $s_2(\beta_{i},\beta_{j}) = \beta$, which contradicts the fact that 
$s_2$ preserves $\rho$.
Assume that $\beta$ has no $2$. 
Every row of the matrix must have exactly one element different from all other elements,
and the result of applying $nu_{B,C}^{2k}$ to every row is the most popular element of the row. Since we have $N\le k$ rows and $2k$ columns, there should be a column among $\alpha_{1},\ldots,\alpha_{2k}$ equal to $\beta$, which contradicts our assumptions.
W.l.o.g., we assume that $\beta(N) = 2$ 
(otherwise we just permute variables of $\rho$).


Put $\alpha_{i}' = \proj_{1,\ldots,N-1}(\alpha_{i})$ 
for every $i$, $\beta' = \proj_{1,\ldots,N-1}(\beta)$.
We know that for every $i\in\{1,\dots,N-1\}$ the $i$-th row contains exactly one element different from the others.
Since $N\le k$, at least $k+1$ of the tuples 
$\alpha_{1}',\ldots,\alpha_{2k}'$ are equal to $\beta'$.
W.l.o.g., we assume that 
$\alpha_{s+1}' = \ldots = \alpha_{2k}' = \beta'$, $\alpha_{i}'\neq\beta'$ 
for every $i\in\{1,\ldots,s\}$, where $s< N$.  
Since not all elements of the first row of the matrix are equal, 
we have $s\ge 1$.

Replace the first column of the matrix $M$ by $\alpha_{2k}$
and consider 
$nu_{B,C}^{2k}(\alpha_{2k},\alpha_{2},\alpha_{3},\ldots,\alpha_{2k}) 
= \gamma_{1}$.
Since $\alpha_{1}'\neq \beta'$, there should be a row
in the new matrix whose elements are equal.
Therefore, $\gamma_{1}\in\rho$, otherwise 
we consider $\alpha_{2k},\alpha_{2},\alpha_{3},\ldots,\alpha_{2k}$
instead of the original sequence, and get a contradiction 
with the fact that every row should contain at least two different elements.
By the definition $\proj_{1,\ldots,N-1}(\gamma_{1}) = \beta'$, 
therefore $\gamma_{1}(N)\neq 2$.
This means that 
at least $2k-2$ among the elements
$\alpha_{2}(N),\ldots,\alpha_{2k}(N)$ are equal 
to $\alpha_{2k}(N)$.
In the same way we can substitute $\alpha_{j}$ instead of $\alpha_{i}$ 
for any $i\in\{1,\dots,s\}$ and $j\in\{s+1,\dots,2k\}$ to conclude that 
$2k-2$ elements among the elements 
$\alpha_{1}(N),\dots,\alpha_{i-1}(N),\alpha_{i+1}(N),\dots,\alpha_{2k}(N)$ 
are equal to $\alpha_{j}(N)$.
Since $\beta(N) = 2$, we also have
$\alpha_{i}(N)\neq\alpha_{j}(N)$.
This implies that 
$\alpha_{s+1}(N) = \dots = \alpha_{2k}(N)\in B$, 
and one of the following cases holds:
\begin{enumerate}
    \item $s = 1$, $\alpha_{2} = \dots = \alpha_{2k}$;
    \item $s = 2$, $\alpha_{1}(N),\alpha_{2}(N)\in C$,
    $\alpha_{3} = \dots = \alpha_{2k}$.
\end{enumerate}
If $s=1$ then $\alpha_{1}(i)\neq \alpha_{2}(i)$ for every $i$ since there should be different elements in every row.

It remains to get an extra condition for the case when $2\in C$
and $s=2$.
In this case we replace 
$\alpha_{1}$ by $\delta_{1} = s_2(\beta_{1},\beta_{N})$ (see the definition of $\beta_{1}$ and $\beta_{N}$ above),
and $\alpha_{2}$ by $\delta_{2} = s_2(\beta_{2},\beta_{N})$. 
%$\delta_{1} = nu_{B,C}^{2k}(\alpha_{1},\alpha_{1},\alpha_{3},\alpha_{3},\ldots,\alpha_{3})$
%and 
%$\alpha_{2}$ by 
%$\delta_{2} = nu_{B,C}^{2k}(\alpha_{2},\alpha_{2},\alpha_{3},\alpha_{3},\ldots,\alpha_{3})$.
%Both of these tuples should be in $\rho$, otherwise 
%we get a new matrix with just one element in a row, which contradicts our assumptions.
Then 
$\delta_{1}(i),\delta_{2}(i)\in\{\alpha_{3}(i),2\}$ for every $i$, 
and 
$nu_{B,C}^{2k}(\delta_1,\delta_2,\alpha_{3},\ldots,\alpha_{3})= \beta$.
Note that $\delta_{1}$ can differ from $\alpha_{3}$ in at most 2 coordinates and one of them is the $N$-th coordinate.
The same is true for $\delta_{2}$.
Therefore, since $\delta_{1},\delta_{2},\alpha_{3}$ (viewed as a matrix with 3 columns)
cannot have equal rows,
$N$ should be equal to 3.
\end{proof}

Our plan is to apply the above lemma to define relations that will be used to prove hardness results.

\begin{lem}\label{ArityThreeRelations}
One of the following cases holds.
\begin{enumerate}
\item $(\{0,2\}\times\{0,2\}\times\{0,2\})\setminus\{(0,0,2)\}\in\Gamma$,
\item $(\{1,2\}\times\{1,2\}\times\{1,2\})\setminus\{(1,1,2)\}\in\Gamma$,
\item $(\{0,2\}\times\{0,2\}\times\{1,2\})\setminus\{(0,0,2)\}\in\Gamma$,
\item $(\{1,2\}\times\{1,2\}\times\{0,2\})\setminus\{(0,0,2)\}\in\Gamma$.
\end{enumerate}
\end{lem}

\begin{proof}
Since $nu_{A,A}^{2k}$ is not $\{0,2\}\{1,2\}$-projective,
$\Gamma$ is not preserved by $nu_{A,A}^{2k}$.
By Lemma \ref{almostNU} there exists a relation $\rho\in\Gamma$
satisfying one of the two cases. The second case is not possible because $nu_{A,A}^{2k}(\alpha_{1},\alpha_{2},\alpha_{2},\ldots,\alpha_{2}) = \alpha_{2}$ for every $\alpha_{1},\alpha_{2}$.
Thus, $\rho$ is of arity 3 and there exist $\alpha_{1},\alpha_{2},\alpha_{3}\in\rho$ 
    such that 
    $nu_{B,C}^{2k}(\alpha_{1},\alpha_{2},\alpha_{3},\alpha_{3},\ldots,\alpha_{3}) = \beta\notin\rho$, 
    $\beta(i) = \alpha_{3}(i)\neq 2$ for $i\in\{1,2\}$, 
    $\beta(3) = 2$,  
    $\alpha_{1}(i)\neq \alpha_{3}(i)$ or $\alpha_{2}(i)\neq \alpha_{3}(i)$,
    $\alpha_{1}(i),\alpha_{2}(i)\in\{\alpha_{3}(i),2\}$ for every $i$, 
    $\alpha_{1}(3) = \alpha_{2}(3) = 2$.
    Suppose $\alpha_{3} = (a_1,a_2,a_3)$. 
    We know that $(a_{1},a_{2},a_{3}), (2,a_{2},2),(a_1,2,2)\in \rho$ (as $\alpha_{3},\alpha_{1},\alpha_{2}$) 
    and $(a_{1},a_{2},2)\notin\rho$ (as $\beta$).
    Since the semilattice $s_2$ applied to $(a_{1},a_{2},0)$ and 
    $(a_{1},a_{2},1)$ gives $(a_{1},a_{2},2)\notin\rho$, 
    $(a_{1},a_{2},c)\in\rho$ implies $c=a_{3}$.
    
    Since $a_{1},a_{2},a_{3}\in\{0,1\}$, 
    at least two of them are equal.
    We consider three cases:
    
    Case 1. $a_{2} = a_{3}$.
    Put $\delta(x,y,z) = \exists t\;\rho(x,a_{2},t)\wedge \rho (y, t,z)$. 
    It is not hard to see that 
    $(a_{1},a_{1}, 2)\notin \delta$ (we need to put $t = a_{2} = a_{3}$ and, therefore, $z = a_{3}$), 
    $(a_{1},2,2),(a_{1},a_{1},a_{3})\in\delta$ (put $t = a_{2} = a_{3} $),
    $(2,2,2),(2,a_{1},2)\in\delta$ (put $t = 2$).

    Case 2. $a_{1} = a_{3}$.
    Put $\delta(x,y,z) = \exists t\;\rho(a_{1},x,t)\wedge \rho (t, y,z)$. 
    It is not hard to see that 
    $(a_{2},a_{2}, 2)\notin \delta$ (we need to put $t = a_{1} = a_{3}$ and, therefore, $z = a_{3}$), 
    $(a_{2},2,2),(a_{2},a_{2},a_{3})\in\delta$ (put $t = a_{1} = a_{3} $),
    $(2,2,2),(2,a_{2},2)\in\delta$ (put $t = 2$).    
    
    Case 3. $a_{1} = a_{2}$. In this case we put $\delta = \rho$.
    
    Thus, we have a relation $\delta\in\Gamma$ 
    satisfying the following properties:
    for some $a,b\in\{0,1\}$ we have 
    $(a,a,b),(2,a,2),(a,2,2),(2,2,2)\in \delta$, 
    $(a,a,2)\notin\delta$.
    Since $s_2$ preserves $\delta$, 
    $(a,a,c)\in\delta$ implies $c=b$.
    
    Put $\delta_{1} = \delta\cap (\{a,2\}\times\{a,2\}\times\{b,2\})$,
$\delta_{2}(x,y,z) = 
\exists t \;
\delta_{1}(x,y,t)\wedge \delta_{1}(x,z,t)
\wedge \delta_{1}(z,x,t).$

Assume that 
$(a,a,2)\in\delta_{2}$.
Since we need to set $t=b$, we have
$(a,2,b),(2,a,b)\in\delta_{1}$.
Since $s_2$ preserves $\delta_{1}$ we obtain 
$(2,2,b)\in\delta_{1}$, 
which means that $\delta_{1}=
(\{a,2\}\times\{a,2\}\times\{b,2\})\setminus\{(a,a,2)\}$
and completes this case.

Assume that 
$(a,a,2)\notin\delta_{2}$.
We know that $(a,a,a)\in\delta_{2}$ (put $t=b$), 
$(a,2,2)$, $(2,a,2)$, $(2,2,a)$, $(2,2,2)\in\delta_{2}$ (put $t = 2$).
Put
$$\delta_{3}(x,y,z) = 
\exists x'\exists y'\exists z' \;
\delta_{2}(x,x,x')\wedge
\delta_{2}(y,y,y')\wedge
\delta_{2}(z',z',z)\wedge
\delta_{2}(x',y',z').$$
Let us show that $\delta_{3} = (\{a,2\}\times\{a,2\}\times\{a,2\})\setminus\{(a,a,2)\}$.
If $x = 2$, then we put $x'=z'=2$ and $y'=y$.
If $y=2$ then we put $y'=z'=2$ and $x'=x$.
If $x=y=z=a$, then we put $y'=z'=y' = a$.
It remains to show that $(a,a,2)\notin\delta_{3}$, which follows from the fact that 
$x'$ should be equal to $a$, 
$y'$ should be equal to $a$, 
$z'$ should be equal to $2$, 
$(a,a,2)\notin\delta_{2}$.
Thus, $\delta_{3} = (\{a,2\}\times\{a,2\}\times\{a,2\})\setminus\{(a,a,2)\}$,
which completes the proof.
\end{proof}

\begin{lem}\label{ArityThreeOrTransZero}
One of the following conditions holds.
\begin{enumerate}
\item $(\{0,2\}\times\{0,2\}\times\{0,2\})\setminus\{(0,0,2)\}\in\Gamma$;
\item there exists a relation $\delta\in\Gamma$ such that 
$(0,1),(2,2)\in\delta$, 
$(0,2)\notin\delta$;
\end{enumerate}
\end{lem}
\begin{proof}
Since $nu_{\{0\},A}^{2k}$ is not $\{0,2\}\{1,2\}$-projective,
$\Gamma$ is not preserved by $nu_{\{0\},A}^{2k}$.
By Lemma \ref{almostNU} there exists a relation $\rho\in\Gamma$
satisfying one of the two cases of Lemma \ref{almostNU}.
Suppose we have the first case of Lemma \ref{almostNU}, where we import that lemma's notation.
Then $\alpha_{3} = (0,0,0), \alpha_{1} = (2,0,2), \alpha_{2}=(0,2,2)$,
$\beta = (0,0,2)$
(or $\alpha_{1}$ and $\alpha_{2}$ can be switched).
Since $s_2$ preserves $\rho$, we have $(2,2,2)\in\rho$.

Let 
$\delta_{0} = \rho\cap\{0,2\}^{3}$.
Consider two cases:

Case 1. $(2,2,0)\in\delta_{0}$. 
For $\epsilon(x,y)=\delta_{0}(y,y,x)$ 
we have $\epsilon=
\begin{pmatrix}
0 & 0& 2\\
0 & 2 & 2
\end{pmatrix}$.

Case 2. $(2,2,0)\notin\delta_{0}$. 
Put $\epsilon(x,y)=\exists t \; \delta_{0}(t,x,y)
\wedge \delta_{0}(x,t,y)$.
If $(2,0)\in\epsilon$, then $(0,2,0),(2,0,0)\in\delta_{0}$,
which, using the semilattice $s_2$, implies 
$(2,2,0)\in\delta_{0}$. This contradiction
shows that $(2,0)\notin\epsilon$ and $\epsilon=
\begin{pmatrix}
0 & 0& 2\\
0 & 2 & 2
\end{pmatrix}$.

Then the required relation $(\{0,2\}\times\{0,2\}\times\{0,2\})\setminus\{(0,0,2)\}$
can be pp-defined by
$$\delta_{1}(x,y,z) = \exists x'\exists y' \exists z'\;
\epsilon(x',x)\wedge \epsilon(y',y)\wedge 
\epsilon(z,z')\wedge \delta_{0}(x',y',z').$$

Suppose we have the second case in Lemma \ref{almostNU}.
Then $\beta = (0,2), \alpha_{1} = (c,d), \alpha_{2} = (0,1)$, 
$s_2(\alpha_{1},\alpha_{2}) = (2,2)\in \rho$.
%If $(0,0)\in\rho$, then %$s\left(\begin{pmatrix}0\\0\end{pmatrix},\begin{pmatrix}0\\1\end{pmatrix}\%right) = \begin{pmatrix}0\\2\end{pmatrix}\in \rho$, which contradicts the %fact that $\beta\notin\rho$. 
Thus, $\rho$ satisfies the conditions of item 2.
\end{proof}

Similarly, if we switch 0 and 1 we get the following lemma.
\begin{lem}\label{ArityThreeOrTransOne}
One of the following cases holds.
\begin{enumerate}
\item $(\{1,2\}\times\{1,2\}\times\{1,2\})\setminus\{(1,1,2)\}\in\Gamma$
\item there exists $\delta\in\Gamma$ such that 
$(1,0),(2,2)\in\delta$, 
$(1,2)\notin\delta$
\end{enumerate}
\end{lem}

\begin{lem}\label{ArityThreeRelationsStrong}
One of the following cases holds:
\begin{enumerate}
\item $(\{0,2\}\times\{0,2\}\times\{0,2\})\setminus\{(0,0,2)\},(\{1,2\}\times\{1,2\}\times\{1,2\})\setminus\{(1,1,2)\}\in\Gamma$
\item $(\{1,2\}\times\{0,2\}\times\{0,2\})\setminus\{(1,0,2)\}, (\{0,2\}\times\{0,2\}\times\{0,2\})\setminus\{(0,0,2)\}\in\Gamma$
\item $(\{0,2\}\times\{1,2\}\times\{1,2\})\setminus\{(0,1,2)\}, (\{1,2\}\times\{1,2\}\times\{1,2\})\setminus\{(1,1,2)\}\in\Gamma$
\end{enumerate}
\end{lem}
\begin{proof}
We apply Lemmas \ref{ArityThreeOrTransZero} and
\ref{ArityThreeOrTransOne}.
If we have the first case in both of them, then the first condition holds and we are done.

Assume that we have the second case in both of them and the corresponding relations are $\delta_{0}$ and $\delta_{1}$, respectively.
Put $$\delta(x,y) = \delta_{0}(x,y)\wedge \delta_{1}(y,x)\wedge (x\in\{0,2\})
\wedge (y\in\{1,2\}).$$
It is not hard to see that 
$\delta = \begin{pmatrix} 0 & 2\\ 1& 2\end{pmatrix}$.
Using this relation we can easily switch $0$ and $1$ in relations.
By Lemma~\ref{ArityThreeRelations}
we have $\rho = (\{a,2\}\times\{a,2\}\times\{b,2\})\setminus\{(a,a,2)\}\in\Gamma$
for some $a,b\in\{0,1\}$.
If $a=b$, then we use the relation $\rho$ and the relation defined by the following 
pp-definition to satisfy condition 1:
$$\rho_{1}(x,y,z) = \exists x'\exists y'\exists z'\;
\rho(x',y',z') \wedge \delta(x,x')\wedge \delta(y,y')\wedge \delta(z,z'),$$
If $a\neq b$, then the relations we need to satisfy condition 1 can be defined by:
$$\rho_{2}(x,y,z) = \exists z'\;
\rho(x,y,z') \wedge \delta(z,z'),$$
$$\rho_{3}(x,y,z) = \exists x'\exists y'\;
\rho(x',y',z) \wedge \delta(x,x')\wedge \delta(y,y').$$

Assume that we have 
the first case in Lemma \ref{ArityThreeOrTransZero}
and 
the second case in Lemma \ref{ArityThreeOrTransOne}.
Thus, $\rho_{4} = (\{0,2\}\times\{0,2\}\times\{0,2\})\setminus\{(0,0,2)\}\in\Gamma$
and 
there exists $\delta\in\Gamma$ such that 
$(1,0),(2,2)\in\delta$, 
$(1,2)\notin\delta$.
Put
$$\rho_{5}(x,y,z)= \exists x' \;\rho_{4}(x',y,z) \wedge \delta(x,x')
\wedge x\in\{1,2\}\wedge x'\in\{0,2\}.$$
Then $\rho_{4}$ and $\rho_{5}$ satisfy the second condition of this lemma.

Assume that we have 
the second case in Lemma \ref{ArityThreeOrTransZero}
and 
the first case in Lemma \ref{ArityThreeOrTransOne}.
Thus, $\rho_{6} = (\{1,2\}\times\{1,2\}\times\{1,2\})\setminus\{(1,1,2)\}\in\Gamma$
and 
there exists $\delta\in\Gamma$ such that 
$(0,1),(2,2)\in\delta$, 
$(0,2)\notin\delta$.
Put
$$\rho_{7}(x,y,z)= \exists x' \; \rho_{6}(x',y,z) \wedge \delta(x,x')
\wedge x\in\{0,2\}\wedge x'\in\{1,2\}.$$
Then $\rho_{6}$ and $\rho_{7}$ satisfy the third condition of this lemma.
\end{proof}

\subsection{Connection with Boolean functions}

A mapping $f:\{0,1\}^{n}\to\{0,1\}$ is called \emph{a Boolean function}.
We say that 
a Boolean function $f$ of arity $n$ is represented by $\Gamma$
if there exists a relation $R$ of arity $n+1$ pp-definable using $\Gamma$
such that for 
all $a_{1},\ldots,a_{n}\in\{0,1\}$, $b\in\{0,1,2\}$
$$(a_{1},\ldots,a_{n},b)\in R\Leftrightarrow  f(a_{1},\ldots,a_{n}) = b.$$
For example, an AND-type relation is a representation of conjunction, 
an OR-type relation is a representation of disjunction.
A $k$-ary Boolean function $f$ is \emph{monotonic} if $f(x_1,\ldots,x_k)\leq f(y_1,\ldots,y_k)$ whenever 
$x_{i}\le y_{i}$ for every 
$i\in\{1,2,\dots,k\}$.
A $k$-ary Boolean function is \emph{linear} if it is of the form $c_{1}x_1+\ldots+c_{k}x_k+c_{0}$ for 
$c_{0},c_{1},\dots,c_{k}\in\{0,1\}$.

\begin{lem}\label{IsClone}
%Let $\Gamma$ be any constraint language containing $0$ %and $1$. The set of all Boolean functions represented by
%$\Gamma$ is a clone containing constants 0 and 1.
The set of all Boolean functions represented by $\Gamma$ is a clone containing constants
0 and 1.
\end{lem}
\noindent Note that this is true for 
arbitrary constraint language containing 
$0$ and $1$.

\begin{proof}
Notice that 
constants 0 and 1 are represented by 
the singleton relations $\{0\}$ and $\{1\}$, which are in $\Gamma$, and 
a projection can be represented 
by the equality relation, which is assumed to be in $\Gamma$.

Suppose we have
Boolean functions 
$g_{1},\dots,g_{n}$ 
of arity $m$ represented by 
relations 
$R_{1},\ldots,R_{n}$, respectively.
Suppose 
$f$ is Boolean function of arity $n$
represented by a relation $R$.
Then the composition 
$h= f(g_1,\dots,g_n)$ can be represented by
the relation defined by 
\begin{align*}
R'(x_{1},\ldots,x_{m},z)
=
\exists y_1\dots\exists y_n
R_{1}(x_{1},\dots,x_{m},y_{1})\wedge
\dots
\wedge
R_{n}(x_{1},\dots,x_{m},y_{n})
\wedge 
R(y_1,\dots,y_n,z).
\end{align*}
\end{proof}

By $\BoolClo(\Gamma)$ we denote the set of all 
Boolean functions represented by $\Gamma$, which is a clone 
by Lemma~\ref{IsClone}.

Let 
$\alpha_{1},\ldots,\alpha_{N}$, where $N = 2^{k+1}-1$,
be the set of all tuples from $\{0,1\}^{k+1}$
except for the tuple $(1,1,\dots,1)$.
Thus, $\alpha_{i}$ can be viewed as a binary representation of 
the number $(i-1)$.

Let us define an operation $f_{\Gamma}$ of arity $N$.
If there exists a unique Boolean function $h\in\BoolClo(\Gamma)$ 
of arity $k+1$ such that 
$h(\alpha_{i}) = a_{i}$ for every $i$, then 
put $f(a_{1},\ldots,a_{N}) = h(1,1,\ldots,1)$.
Otherwise, put $f(a_{1},\ldots,a_{N}) = 2$.

\begin{lem}
Suppose Boolean functions $h_{1}$ and $h_{2}$ of arity $n\ge 2$
differ only on the tuple $(1,1,\dots,1)$.
Then conjunction can be generated from $h_{1},h_{2}$ and constants $0,1$.
\end{lem}
\begin{proof}
Since the functions $h_1$ and $h_2$ differ just on one tuple,
they cannot be both linear.
Assume that they are monotonic.
Since $h_1(1,1,\dots,1) \neq h_2(1,1,\dots,1)$, 
we have $h_1(x_1,\dots,x_n) = 0$ 
and $h_2(x_1,\dots,x_n) = x_1\wedge\dots\wedge x_n$
(or we should switch $h_1$ and $h_2$).
Thus, we generated conjunction in this case.

Assume that one of the functions $h_1$ and $h_2$ is not monotonic.
Then 
%By \cite{Post},
%it is sufficient 
%to check that 
$h_{1},h_{2},0,1$ are not contained in any maximal clone 
of Boolean functions.
Hence, by \cite{Post}, any function, including conjunction, 
can be generated from $h_1$, $h_2$, $0$, and $1$.
\end{proof}

Therefore, 
if $\BoolClo(\Gamma)$ does not contain conjunction, 
then the word ``unique'' can be removed from the definition of $f_{\Gamma}$.
Also, since constants 0 and 1 are in $\BoolClo(\Gamma)$, 
the operation 
$f_{\Gamma}$ is idempotent in this case.

\begin{lem}\label{fGammaIsNotProjective}
Suppose $\BoolClo(\Gamma)$ does not contain conjunction, 
then $f_{\Gamma}$ is not 
$\{0,2\}\{1,2\}$-projective.
\end{lem}

\begin{proof}
Assume that 
$f_{\Gamma}$ is a $\{0,2\}\{1,2\}$-projection onto the $i$-th coordinate.
Let $\alpha_{i}$ have $0$ at the $j$-th coordinate, 
and $h$ is the $(k+1)$-ary Boolean projection onto the $j$-th coordinate.
Then 
$f_{\Gamma}(h(\alpha_{1}),h(\alpha_{2}),\dots,h(\alpha_{N}))=h(1,1,\dots,1) = 1$
and $h(\alpha_{i})=0$. Contradiction.
\end{proof}

\begin{lem}\label{0StableNegationImplies1Stable}
Suppose the negation Boolean function is represented by $\Gamma$, 
and $\Gamma$ is preserved by a 0-stable operation $v_{0}$.
Then $v_{0}$ is 1-stable.
\end{lem}

\begin{proof}
Since $v_{0}$ preserves the relation representing the negation and
$v_{0}(1,0) = 1$, we have 
$v_{0}(0,1)=0$. 
Combining this with the fact that 
$v_{0}$ is idempotent and
$v_{0}$ is a $\{0,2\}\{1,2\}$-projection onto the first coordinate, we obtain that $v_{0}$ is 1-stable.
\end{proof}

\begin{thm}\label{ANDTypeForStable}
Suppose $\Gamma$ is preserved by a 0-stable operation $v_{0}$, 
then $\Gamma$ contains an AND-type relation 
(equivalently $\BoolClo(\Gamma)$ contains conjunction).
\end{thm}

\begin{proof}
Assume that $\BoolClo(\Gamma)$ does not contain conjunction.

By Lemma~\ref{fGammaIsNotProjective}, 
$f_{\Gamma}$ is not $\{0,2\}\{1,2\}$-projective, 
hence there should be a relation in $\Gamma$ that is not preserved by 
$f_{\Gamma}$.
Let $\rho$ be a relation of the minimal arity in $\Gamma$ that is not preserved by $f_{\Gamma}$.
Thus, 
there exists a matrix $M$ whose columns are tuples from $\rho$ 
such that 
$f_{\Gamma}$ applied to the rows of $M$ gives $\beta\notin\rho$.
Let $L$ be the arity of $\rho$.

Note that each row of the matrix should contain different elements, 
since otherwise we could substitute a constant into $\rho$ and reduce the arity of $\rho$ (recall that $f_{\Gamma}$ is idempotent).
Since $\rho$ is a relation of the minimal arity, for every $i$ there should be a tuple $\beta_{i}\in\rho$ such that 
$\beta_{i}$ differs from $\beta$ only in the $i$-th coordinate (otherwise, we consider the projection of $\rho$ onto all coordinates but $i$-th, which has the same properties as $\rho$ but smaller arity).
%(see the proof of Lemma~\ref{almostNU} for the detailed explanation).

Assume that $\beta$ has at least two elements equal to $2$ and they appear at the $i$-th and $j$-th coordinates.
Then $s_2(\beta_{i},\beta_{j}) = \beta$, which contradicts the fact that 
$s_2$ preserves $\rho$.

Assume that $\beta$ contains exactly one $2$.
W.l.o.g., we assume that $\beta(L) = 2$.
By the definition of 
$f_{\Gamma}$ 
for every $i\in[L-1]$
there exists a Boolean function 
$h_{i}\in\BoolClo(\Gamma)$ (not a constant function)
such that 
the $i$-th row of $M$ 
is 
$(h_{i}(\alpha_{1}),\dots,h_{i}(\alpha_{N}))$.

Assume that there exists a tuple $\gamma\in\rho$ such that $\gamma(L) = 2$ and $\gamma(i) \in\{0,1\}$
for $i\in[L-1]$.
By Lemma~\ref{0StableNegationImplies1Stable}, 
we have two cases:

Case 1. $\BoolClo(\Gamma)$ does not contain negation.
It follows from Post's lattice (see \cite{Post}) that all functions in $\BoolClo(\Gamma)$ are monotonic.
Thus, $h_{i}$ is a monotonic function that is not a constant, 
therefore 
$\beta(i) = h_{i}(1,1,\ldots,1) = 1$ for every $i\in[L-1]$.
Applying the 0-stable operation $v_{0}$ to $\beta_{L}$ and $\gamma$
we obtain $(1,1,\dots,1,2) = \beta$, which contradicts the fact that 
$v_{0}$ preserves $\rho$.

Case 2. $v_{0}$ is 1-stable.
Applying $v_{0}$ to $\beta_{L}$ and $\gamma$
we obtain $\beta$, which contradicts the fact that
$v_{0}$ preserves $\rho$.

Thus, we proved that 
$\rho$ does not contain a tuple whose last element is 2 and the remaining elements are from $\{0,1\}$. For instance, this means that the matrix $M$ contains only 0 and 1.
Let $R_{i}$ be a relation pp-definable from $\Gamma$ 
representing $h_{i}$.
Define a new relation by 
\begin{align*}
R(x_{1},\ldots,x_{k+1},z)
=&\\
\exists y_1\dots\exists y_{L-1}\;&
R_{1}(x_{1},\dots,x_{k+1},y_{1})\wedge
\dots
\wedge
R_{L-1}(x_{1},\dots,x_{k+1},y_{L-1})
\wedge 
\rho(y_1,\dots,y_{L-1},z).
\end{align*}
We can check that for each 
$\alpha_{i}$ 
there exists a unique $b_{i}\in\{0,1\}$ 
such that 
$\alpha_{i}b_{i}\in R$.
Note that $b_{i}$ is the $i$-th element of the last 
row of the matrix.
Since
$(1,1,\ldots,1,h_i(1,1,\dots,1)) \in R_{i}$ 
and $\beta(i) = \beta_{L}(i) = h_i(1,1,\dots,1)$
for every $i\in[L-1]$, we have
$(1,1,\dots,1,\beta_{L}(L))\in R$,
which means that $R$ represents the 
corresponding Boolean function 
and $f_{\Gamma}(b_{1},\dots,b_{N})=\beta_{L}(L)$.
This contradicts the fact that 
$\beta(L) = 2$.


It remains to consider the case when $\beta$ has no $2$. 
Therefore,
for every $i\in[L]$
there exists a Boolean function 
$h_{i}\in\BoolClo(\Gamma)$ (not a constant function)
such that 
the $i$-th row of $M$ 
is 
$(h_{i}(\alpha_{1}),\dots,h_{i}(\alpha_{N}))$.
It follows from Post's Lattice (see \cite{Post}) that we have only the following two cases.

Case 1. $\BoolClo(\Gamma)$ contains only linear functions.
Consider a system of linear equations 
$$
\begin{cases}
h_{1}(x_{1},\ldots,x_{k+1}) = h_{1}(1,\dots,1)\\
h_{2}(x_{1},\ldots,x_{k+1}) = h_{2}(1,\dots,1)\\
\dots\\
h_{L}(x_{1},\ldots,x_{k+1}) = h_{L}(1,\dots,1)
\end{cases}
$$
Since $L\le k$, there should be a solution of this system of equations
different from 
$(1,1,\dots,1)$.
Let this solution be equal to $\alpha_{i}$ for $i\in[N]$.
Therefore, the $i$-th column of the matrix $M$ 
is equal to 
$(h_{1}(1,\dots,1),h_{2}(1,\dots,1),\dots,h_{L}(1,1,\dots,1))$, 
which is equal to $\beta$. 
This contradicts the fact that $\beta\notin\rho$.

Case 2. $\BoolClo(\Gamma)$ is the clone generated by disjunction and constants.
Since every operation $h_{j}$ is monotonic and not constant, 
$\beta = (1,1,\dots,1)$.
Since $h_{j}$ is not a constant for every $j\in[L]$, 
we can choose $n_{j}$ such that 
$h_{j}(x_{1},\dots,x_{k+1})\ge x_{n_{j}}$.
Let $\alpha_{i}$ be the tuple having 1 only on 
coordinates $n_{1},\dots,n_{L}$ (such $\alpha_{i}$ exists because $L<k+1$).
Then 
the $i$-th column of the matrix $M$ 
is equal to $(1,1,\dots,1)$, which contradicts the fact that $\beta\notin\rho$.
\end{proof}

In the same way we can prove the following theorem.
\begin{thm}\label{ORTypeForStable}
Suppose $\Gamma$ is preserved by a 1-stable operation, 
then $\Gamma$ contains an OR-type relation 
(equivalently $\BoolClo(\Gamma)$ contains disjunction).
\end{thm}


\subsection{The proof of the EGP classification}




\begin{lem}\label{NoStableOperation}
Suppose $\Pol(\Gamma)$ does not have a $0$-stable operation.
Then $\Gamma$ contains one of the two relations
$\begin{pmatrix}
0 & 1 & 2 & 0 & 2\\
0 & 0 & 0 & 2 & 2 
\end{pmatrix}$,
$\begin{pmatrix}
0 & 1 & 2 & 0 & 2\\
1 & 1 & 1 & 2 & 2 
\end{pmatrix}$.
\end{lem}
\begin{proof}
Let $\delta_{1}$ and $\delta_2$ be the 
relations generated from 
%\left\langle
$\begin{pmatrix}
1 & 0\\
0 & 2 
\end{pmatrix}$
%\right\rangle_{\Pol(\Gamma)}$,
%$\delta_{2} = \left\langle
and 
$\begin{pmatrix}
1 & 0\\
1 & 2 
\end{pmatrix}$
%\right\rangle_{\Pol(\Gamma)}$.
using $\Pol(\Gamma)$, respectively.
Note that since 
$s_2\in\Pol(\Gamma)$ we have $(2,2)\in \delta_{1}$ and $(2,2)\in \delta_2$.
Assume that 
$(1,2)\in \delta_{1}$ and $(1,2)\in\delta_{2}$.
Then there exist operations 
$f_{1}, f_{2}\in\Pol(\Gamma)$ 
such that 
$f_{1}(1,0) = f_{2}(1,0) = 1$, 
$f_{1}(0,2) = f_{2}(1,2) = 2$.
Since $f_{1}$ and $f_{2}$ are $\{0,2\}\{1,2\}$-projective, 
they should be $\{0,2\}\{1,2\}$-projections onto the first coordinate and $f_{1}(2,x) =f_{2}(2,x) = 2$.
Put $f(x,y) = f_{1}(f_{2}(x,y),y)$,
then
$f(1,0) = 1$, $f(0,2) = f(1,2) = f(2,0) = 2$.
%Since $f$ is $\{0,2\}\{1,2\}$-projective, we obtain that 
%$f(2,0) = 2$. 
Therefore, $f$ is a $0$-stable operation. Contradiction.

Assume that 
$(1,2)\notin \delta_{1}$.
Then by Lemma~\ref{ArityThreeRelationsStrong}, 
$\psi_{1} = (\{0,2\}\times\{a,2\}\times\{a,2\})\setminus\{(0,a,2)\}\in\Gamma$
for some $a\in\{0,1\}$.
Then one of the two necessary relations is defined 
by the formula 
$\delta_{1}'(x,y) = \exists z \;\delta_{1}(x,z) \wedge \psi_{1}(z,a,y)$.

It remains to consider the case when
$(1,2)\notin \delta_{2}$.
Then by Lemma~\ref{ArityThreeRelationsStrong}, 
$\psi_{2} = (\{1,2\}\times\{a,2\}\times\{a,2\})\setminus\{(1,a,2)\}\in\Gamma$ for some $a\in\{0,1\}$.
Then one of the two necessary relations is defined 
by the formula 
$\delta_{2}'(x,y) = \exists z \;\delta_{2}(x,z) \wedge \psi_{2}(z,a,y)$.

\end{proof}

In the same way we can prove the following lemma.
\begin{lem}\label{NoStableOperationOne}
Suppose $\Pol(\Gamma)$ does not have a $1$-stable operation.
Then $\Gamma$ contains one of the two relations
$\begin{pmatrix}
0 & 1 & 2 & 1 & 2\\
0 & 0 & 0 & 2 & 2 
\end{pmatrix}$,
$\begin{pmatrix}
0 & 1 & 2 & 1 & 2\\
1 & 1 & 1 & 2 & 2 
\end{pmatrix}$.
\end{lem}


Recall the following relations from 
Section~\ref{HardnessSection}:
$$\sigma_{0} = \{(a,b,c)\mid a\in A, b,c\in\{1,2\}, a\in \{0,2\}\vee(b=c)\}$$
$$\sigma_{0}' = \{(a,b,c)\mid a\in A, b,c\in\{0,2\}, a\in \{0,2\}\vee(b=c)\}$$
$$\sigma_{1} = \{(a,b,c)\mid a\in A, b,c\in\{0,2\}, a\in \{1,2\}\vee(b=c)\}$$
$$\sigma_{1}' = \{(a,b,c)\mid a\in A, b,c\in\{1,2\}, a\in \{1,2\}\vee(b=c)\}$$

\begin{lem}
Suppose $\Pol(\Gamma)$ does not have a $0$-stable 
or $1$-stable operation, then 
one of the following conditions holds:
\begin{enumerate}
\item $\sigma_{0},\sigma_{1}\in \Gamma$,
\item $\sigma_{0}',\sigma_{1}\in \Gamma$,
\item $\sigma_{0},\sigma_{1}'\in \Gamma$.
\end{enumerate}
\label{lem:Pspace-definitions}
\end{lem}


\begin{proof}
By Lemmas~\ref{NoStableOperation}
and \ref{NoStableOperationOne},
we have the relations $\delta_{1} = \begin{pmatrix}
0 & 1 & 2 & 0 & 2\\
a_{1} & a_{1} & a_{1} & 2 & 2 
\end{pmatrix}$ and 
$\delta_{2}=\begin{pmatrix}
0 & 1 & 2 & 1 & 2\\
a_{2} & a_{2} & a_{2} & 2 & 2 
\end{pmatrix}$
in $\Gamma$
for some $a_{1},a_{2}\in\{0,1\}$.
By Lemma~\ref{ArityThreeRelationsStrong}, 
for some $b_{1},b_{2}\in\{0,1\}$ the relations $\psi_{1}=(\{a_{1},2\}\times\{b_{1},2\}\times\{b_{1},2\})\setminus\{(a_{1},b_{1},2)\}$,
$\psi_{2}= (\{a_{2},2\}\times\{b_{2},2\}\times\{b_{2},2\})\setminus\{(a_{2},b_{2},2)\}$ are in $\Gamma$.
We define 
$$\psi_{1}'(x,y,z) = \exists t \;\delta_{1}(x,t)\wedge \psi_{1}(t,y,z)\wedge \psi_{1}(t,z,y),$$
$$\psi_{2}'(x,y,z) = \exists t \;\delta_{2}(x,t)\wedge \psi_{2}(t,y,z)
\wedge \psi_{2}(t,z,y).$$
If $b_{1}=1$ then $\psi_{1}'= \sigma_{0}$.
If $b_{1}=0$ then $\psi_{1}'= \sigma_{0}'$.
If $b_{2}=0$ then $\psi_{2}'= \sigma_{1}$.
If $b_{2}=1$ then $\psi_{2}'= \sigma_{1}'$.
Thus, if $b_{1}=b_{2}=0$ then
$\sigma_{0}',\sigma_{1}\in \Gamma$, which is the second case.
If $b_{1}=b_{2}=1$ then
$\psi_{1} = \sigma_{0},\sigma_{1}'\in \Gamma$, 
which is the third case.
If $b_{1} = 1$ and $b_{2}=0$ then 
$\sigma_{0},\sigma_{1}\in\Gamma$, 
which is the first case.

If remains to consider the case when 
$b_{1} = 0$ and $b_{2}=1$.
In this case the relations 
$\sigma_{0}$ and $\sigma_1$
can be pp-defined from 
$\sigma_{0}'$ and $\sigma_{1}'$ as follows:
$$\sigma_{1}(x,y,z) = \exists z'\;
\sigma_{1}'(x,1,z')\wedge \sigma_{0}'(z',y,z),$$
$$\sigma_{0}(x,y,z) = \exists z'\;
\sigma_{0}'(x,0,z')\wedge \sigma_{1}'(z',y,z).$$
\end{proof}

Combining the above lemma with Lemma~\ref{PSpaceHardness} 
we obtain the following corollary.

\begin{cor}\label{PSpaceCompleteness}
Suppose $\Pol(\Gamma)$ does not have a $0$-stable 
or $1$-stable operation, then 
$\QCSP(\Gamma)$ is PSpace-complete.
\end{cor}

%\begin{lem}\label{OnePPDefinition}
%Suppose 
%$R_{1}$ is an AND-type relation, 
%$\begin{pmatrix}
%0&1&2\\
%0&2&2
%\end{pmatrix}\subseteq R_{2}\subseteq 
%\begin{pmatrix}
%0&1&2&1&2\\
%0&0&0&2&2
%\end{pmatrix}$,
%$\begin{pmatrix}
%0&2\\
%1&2
%\end{pmatrix}\subseteq R_{3}\subseteq 
%\begin{pmatrix}
%0&2&2\\
%1&1&2
%\end{pmatrix}$.
%Then 
%$\begin{pmatrix}
%0&1&1&1&2&2&2\\
%1&0&1&2&0&1&2
%\end{pmatrix}$ can be pp-defined from $\{R_{1},R_{2},R_{3}\}$.
%\end{lem}
%\begin{proof}
%Since $(2,2,0),(2,2,2)\in R_{1}$, the required relation can be pp-defined as follows.
%$$\rho(x,y) = \exists 
%z_{1}\exists z_{2}\exists z_{3}\;
%R_{2}(x,z_{1})\wedge R_{1}(z_{1},z_{1},z_{2})
%\wedge 
%R_{3}(z_{2},z_{3})\wedge R_{1}(z_{3},z_{3},y).$$
%\end{proof}

\begin{lem}\label{SecondPPDefinition}
Suppose $\Gamma$ is not preserved by $f_{0,2}$, 
$\Gamma$ is preserved by $s_{0,2}$,
$$\begin{pmatrix}
0&1&1&1&2&2&2\\
1&0&1&2&0&1&2
\end{pmatrix},
\begin{pmatrix}
0&1&1&1&2&2&2\\
0&0&1&2&0&1&2
\end{pmatrix},\begin{pmatrix}
0&1&2&2&2\\
0&1&0&1&2
\end{pmatrix}\in\Gamma,$$
then the relation 
$\delta(x,y,z) = (x\neq 0)\vee (y=z)$ can be pp-defined from $\Gamma$.
\end{lem}
\begin{proof}
First, denote 
the relations from the statement by $R_1$, $R_2$ and 
$R_3$, respectively.
Let $\rho_{1}$ be the relation generated from
%=\left\langle
$\begin{pmatrix}
0 & 0 & 2\\
1 & 0 & 0\\
1 & 0 & 1
\end{pmatrix}$ using $\Pol(\Gamma)$.
%\right\rangle_{\Pol(\Gamma)}$.
Assume that 
$(0,1,2)\in\rho_{1}$, 
then there exists 
a function $f\in\Pol(\Gamma)$ such that 
$f(0,0,2) = 0$, $f(1,0,0)=1$, and $f(1,0,1) =2$.
Since $f$ is $\{0,2\}\{1,2\}$-projective, 
$f$ always returns the first variable or 2.
Since $f$ preserves $R_1$
%$\begin{pmatrix}
%0&1&1&1&2&2&2\\
%1&0&1&2&0&1&2
%\end{pmatrix}$ 
and $f(0,0,2) = 0$, we have $f(1,1,a) = 1$ for every $a$.
Since 
$f$ preserves $R_2$
%$\begin{pmatrix}
%0&1&1&1&2&2&2\\
%0&0&1&2&0&1&2
%\end{pmatrix}$
and $f(0,0,2) = 0$, 
we have $f(0,0,a) = 0$ for every $a$.

Let us show that 
$f_{0,2}(x,y,z) = f(s_{0,2}(x,y),y,z)$.
If $x=y$ then 
by the above property we have
$f(s_{0,2}(x,y),y,z) = f(x,y,z) = x$.
Also, if $y=z=0$ then
since 
$f(1,0,0)=1$ and $f(0,0,0)=0$, 
we obtain
$f(s_{0,2}(x,y),y,z) = f(x,y,z) = x$.
If $x=2$ or $y=2$ then 
$f(s_{0,2}(x,y),y,z)$ returns 2.
If 
$x=0$ and $y=1$ then $s_{0,2}(x,y)=2$
and $f(s_{0,2}(x,y),y,z)=2$.
If $x=z=1$ and $y=0$, then 
$f(s_{0,2}(x,y),y,z)=f(x,y,z)=f(1,0,1)=2.$
Thus, we considered all cases and showed that 
$f_{0,2}(x,y,z) = f(s_{0,2}(x,y),y,z)$, 
which contradicts the fact that $f_{0,2}\notin\Pol(\Gamma)$.
Therefore 
$(0,1,2)\notin\rho_{1}$.
%Denote $\rho_{2}= \begin{pmatrix}
%0&1&1&1&2&2&2\\
%0&0&1&2&0&1&2
%\end{pmatrix}$,
%$\rho_{3}= \begin{pmatrix}
%0&1&2&2&2\\
%0&1&0&1&2
%\end{pmatrix}$.
Put
$$\rho_{2}(x,y,z) = 
\exists x'\exists y' \exists z'\;
\rho_{1}(x',y',z')
\wedge 
R_{2}(x,x')
\wedge 
R_{3}(y,y')
\wedge 
R_{3}(z',z).$$

Note that $\rho_{1}\subseteq \rho_{2}$, 
and $(0,1,2)\notin\rho_{2}$.
Since $\rho_{1}$ is preserved by $s_2$ 
and $s_{0,2}$, we have 
$s_2
\begin{pmatrix}
0&2\\
0&0\\
0&1
\end{pmatrix}
=
\begin{pmatrix}
2\\
0\\
2
\end{pmatrix}\in\rho_{1}$,
$s_{0,2}
\begin{pmatrix}
0&2\\
1&0\\
1&2
\end{pmatrix}
=
\begin{pmatrix}
2\\
1\\
2
\end{pmatrix}\in\rho_{1}$,
$s_2
\begin{pmatrix}
2&2\\
0&1\\
2&2
\end{pmatrix}
=
\begin{pmatrix}
2\\
2\\
2
\end{pmatrix}\in\rho_{1}$.
Therefore $\rho_{2}$ contains all the tuples $(1,a,b),(2,a,b)$ for every 
$a,b\in A$ 
(we just put $x'=z'=2$ in the definition of $\rho_{2}$).

Define $\delta'(x,y,z) = \rho_{2}(x,y,z)\wedge \rho_{2}(x,z,y)$.
By the previous fact, 
$\delta'$ contains all the tuples with the first element different from 
$0$.
If $\rho_{2}$ contains $(0,1,0)$ then 
we may apply $s_2$ to 
$(0,1,0)$ and $(0,1,1)$ to obtain $(0,1,2)$, which is not from $\rho_{2}$. 
Thus $(0,1,0)\notin\rho_{2}$.
Therefore, $(0,1,0),(0,0,1),(0,1,2),(0,2,1)\notin\delta'$.

Assume that $\delta'$ contains the tuple 
$(0,0,2)$.
Then applying $s_{0,2}$ to 
$(0,1,1)$ and $(0,0,2)$ we get a tuple $(0,1,2)$ which contradicts our assumptions.
Therefore $\delta'=\delta$, which completes the proof.
\end{proof}




\begin{lem}\label{StrangeOneImplies}
Suppose $\Gamma$ is preserved by a 0-stable operation but not preserved by $g_{0,2}$, and 
$R= \begin{pmatrix}
0&1&2&2&2\\
0&1&0&1&2
\end{pmatrix}\in\Gamma$.
Then $\Gamma$ contains a relation
$\delta\in\left\{
\begin{pmatrix}
0&2\\
1&2
\end{pmatrix},
\begin{pmatrix}
0&2&2\\
1&1&2
\end{pmatrix}\right\}$.
\end{lem}

\begin{proof}
Let
$\rho$ 
be the relation generated from 
$\begin{pmatrix}
0&2\\
1&0\\
1&2
\end{pmatrix}$
using $\Pol(\Gamma)$.
Assume that 
$(0,1,2)\in\rho$, then there exists an operation $f$ such that $f(0,2)= 0$, $f(1,0) = 0$, 
$f(1,2) =2$.
Let us check that $f=g_{0,2}$.
Since $f$ preserves $R$ and $f(0,2) = 0$,
we have $f(0,a) = 0$ for any $a$.
We also know that 
$f(1,0) = 1$, $f(1,1) =1$, $f(1,2) = 2$.
It remains to check that $f$ returns 2 if the first variable equals 2. 
This follows from the fact that $f$ is $\{0,2\}\{1,2\}$-projective.

Assume that 
$(0,1,2)\notin\rho$.
Since $\rho$ is preserved by a 0-stable operation
and $(0,1,1),(2,0,2)\in\rho$, we have $(2,1,2)\in\rho$.
%Since $\Pol(\Gamma)$ is $\{0,2\}\{1,2\}$-projective, 
%$\{0,2\}$ and $\{1,2\}$ are from $\Gamma$.
Put 
$\delta(x,y) = \rho(x,1,y)\wedge x\in\{0,2\}\wedge y\in\{1,2\}$. 
We know that 
$(0,1),(2,2)\in\delta$, $(0,2)\notin\delta$, which completes the proof.
\end{proof}


Now we are ready to prove the classification of the complexity for 
constraint languages we consider in this section.



\begin{thm}\label{SpecialClassification}
Suppose $\Gamma$ is a finite constraint language on $\{0,1,2\}$   
with constants,
%containing $\{0\},\{1\},\{2\}$, $\Gamma$ is preserved by $s_2$, 
$\Pol(\Gamma)$ is $\{0,2\}\{1,2\}$-projective. Then $\QCSP(\Gamma)$ is 
\begin{enumerate}
\item PSpace-complete, if $\Pol(\Gamma)$ does not contain a 0-stable or 1-stable operation.
\item in P, if 
$\Gamma$ is preserved by $s_{a,2}$ and $g_{a,2}$ for some $a\in\{0,1\}$.
\item in P, if
$\Gamma$ is preserved by $f_{a,2}$ for some $a\in\{0,1\}$.
\item co-NP-complete, otherwise.
\end{enumerate}
\end{thm}

\begin{proof}
Let $r$ be the maximal arity of relations in $\Gamma$, 
let $k=max(4,r)$. 
Note that if we add to $\Gamma$ all the relations of arity at most $k$
that can be pp-defined from $\Gamma$ then  we do not change the complexity of $\QCSP(\Gamma)$.
Also, adding the equality relation to $\Gamma$ does not change the complexity since 
the equalities can be propagated out.
Another important fact is that adding pp-definable relations and the equality relation to a constraint language does not affect the set of polymorphisms $\Pol(\Gamma)$.
Thus, it is sufficient to prove the claim only for constraint languages $\Gamma$ containing all such relations.
Additionally, 
since $\Pol(\Gamma)$ is $\{0,2\}\{1,2\}$-projective, 
$\{0,2\}$ and $\{1,2\}$ are from $\Gamma$.
Therefore, $\Gamma$ satisfies all the assumptions 
we formulated in the beginning of this section.

Case 1 follows from Corollary~\ref{PSpaceCompleteness}.
Then we may assume that 
$\Gamma$ is preserved by a 0-stable operation (the 1-stable case can be considered in the same way).
If $\Gamma$ is preserved by $f_{0,2}$ 
then 
by Corollary~\ref{CorComplexityStrange2} $\QCSP(\Gamma)$ is in P.
Similarly, 
if $\Gamma$ is preserved by $s_{0,2}$ and $g_{0,2}$ 
then by Corollary~\ref{CorComplexityStrange1} 
$\QCSP(\Gamma)$ is in P.
Thus we assume that $f_{0,2}$ does not preserve $\Gamma$, 
and $s_{0,2}$ or $g_{0,2}$ does not preserve $\Gamma$.

By Lemma~\ref{InCONPForStable} the problem 
$\QCSP(\Gamma)$ is in co-NP.
By Theorem~\ref{ANDTypeForStable},
$\Gamma$ contains an 
AND-type relation $\delta$.
We can check that $\delta_{1}(x,y) = \delta(x,x,y)$ is equal to $\begin{pmatrix}
0&1&2&2&2\\
0&1&0&1&2
\end{pmatrix}$
 (to derive $(2,1)$ we apply a 0-stable operation to $(1,1)$ and $(2,0)$).

If $\Gamma$ is also preserved by a 1-stable operation, 
then by Theorem~\ref{ORTypeForStable}, 
$\Gamma$ contains an OR-type relation,
and 
by Lemma~\ref{ANDORHardness}, $\QCSP(\Gamma)$ is co-NP-complete.

Thus, we assume that $\Gamma$ is not preserved by a 1-stable operation.
By Lemma~\ref{NoStableOperationOne},
$\Gamma$ contains a relation
$\delta_{2}\in\left\{\begin{pmatrix}
0 & 1 & 2 & 1 & 2\\
0 & 0 & 0 & 2 & 2 
\end{pmatrix},
\begin{pmatrix}
0 & 1 & 2 & 1 & 2\\
1 & 1 & 1 & 2 & 2 
\end{pmatrix}\right\}$.
Define 
$$\delta_{3}(x,y)= \exists x'\exists y'\;\delta_{2}(x,x')\wedge
\delta(x,x',y')\wedge \delta_{1}(y',y).$$
We can check that $(0,a)\in\delta_{3}$ implies $a=0$.
Applying $s_2$ to the tuples 
$(1,1,1)$,$(1,0,0)$, 
and to the tuples 
$(1,1,1)$,$(0,0,0)$, 
we obtain that 
$(1,2,2),(2,2,2)\in\delta$.
Then 
$(1,a),(2,a)\in\delta_{3}$ for every $a$
(put $x'=y' = 2$ in the definition of $\delta_{3}$),
which means that
$\delta_{3}=\begin{pmatrix}
0 & 1 & 1 & 1 & 2 & 2 & 2\\
0 & 0 & 1 & 2 & 0 & 1 & 2 
\end{pmatrix}$.

Assume that a 0-stable operation we have is 
$h_{0}$.
Since $h_{0}$ is $\{0,2\}\{1,2\}$-projective, 
it returns the first variable or 2.
If $h_{0}(0,1) = 0$, then $h_{0}$ is also 1-stable operation, which contradicts our assumptions.
Thus $h_{0}(0,1) = 2$.
If $h_{0}(0,2) =0$ then we get a contradiction 
with the fact that $h_{0}$ preserves $\delta_{3}$.
Thus $h_{0} = s_{0,2}$, which means that $\Gamma$ is not preserved by $g_{0,2}$.
By Lemma~\ref{StrangeOneImplies}, 
$\Gamma$ contains 
a relation 
$\delta_{4}\in \left\{\begin{pmatrix}
0&2\\
1&2
\end{pmatrix},
\begin{pmatrix}
0&2&2\\
1&1&2
\end{pmatrix}\right\}$.
Define 
$$\delta_{5}(x,y) = \exists 
z_{1}\exists z_{2}\;
\delta_{3}(x,z_{1})\wedge \delta_{4}(z_{1},z_{2})\wedge \delta_1(z_{2},y).$$
%By Lemma~\ref{OnePPDefinition},
%
We can check that 
$\delta_{5}=\begin{pmatrix}
0&1&1&1&2&2&2\\
1&0&1&2&0&1&2
\end{pmatrix}\in\Gamma$.
Applying Lemma~\ref{SecondPPDefinition} to $\delta_{5}$, $\delta_{3}$, and $\delta_{1}$, 
we derive that the required relation $(x\neq 0)\vee (y=z)$ can be pp-defined from $\Gamma$.
Then by Lemma~\ref{NoStrange2Hardness},
$\QCSP(\Gamma)$ is co-NP-complete.
\end{proof}

==> old/comments.tex <==
1) I don't think it is good that we repeat the whole proof in Lemma 17.

==> old/crap.tex <==
Let us show (1) for $\delta_{k-1}$. 
Suppose $p_{k-1}(x_1,\dots,x_{k-1})$ holds, 
then there exists $x_{k}\in\{0,1\}$
such that $p_{k}(x_1,\dots,x_{k})$ holds. 
If $x_{k}=0$ then the EP chooses $u = y$
in the definition of $\delta_{k-1}$, 
otherwise if $x_{k}=1$ he chooses $u = y'$.
If the UP plays $x_{k} = 0$
they the EP chooses 
$u'= y'$, if the UP plays $x_{k} = 1$
they the EP chooses $u'= y$. 
By the property (3) it does not make sense for the UP to play $x_{k}=2$.
Thus, in all the cases the 
part $\sigma_0(x_{k},y,u') \wedge \sigma_1(x_{k},y',u')$
is satisfied. 
Notice that if 
the choice of $x_{k}$ in 
$p_{k}(x_1,\dots,x_{k})$ is different from the 
choice of $x_{k}$ in $\delta_{k-1}$
then $u=u'$ and
the part $\delta_{k}(x_1,\dots,x_{k},u,u')$ holds by 
(2).

If the universal player plays $x_{k} = 0$
they the existential player can safely choose 
$u'= y'$.
If the universal player plays $x_{k} = 1$
they the existential player can safely choose 
$u'= y$. By the property (3) it does not make sense for the universal play $x_{k}=2$.


\begin{proof}
{\color{red}
 The reduction will be from the complement of (monotone) \emph{Quantified Not-All-Equal 3-Satisfiability} (co-QNAE3SAT) which is co-PSpace-hard (see \cite{papa}) and consequently also PSpace-hard (as PSpace is closed under complement). Consider an instance $I$ of co-QNAE3SAT of the form $(x_{a_1},x_{b_1},x_{c_1}), \ldots, (x_{a_s},x_{b_s},x_{c_s})$ which is a yes-instance precisely when, for all truth assignments to the variables, one among these triples $(x_{a_i},x_{b_i},x_{c_i})$ is either $(0,0,0)$ or $(1,1,1)$.

Let
\begin{align*}
    \Phi= & \bigwedge_{1 \le i \le s}
    \begin{array}{c}
    (\sigma_0(x_{a_i},y_{i-1},y_i)\wedge
    \sigma_0(x_{b_i},y_{i-1},y_i) \wedge \sigma_0(x_{c_i},y_{i-1},y_i)) \\
    (\sigma_1(x_{s+a_i},y_{s+i-1},y_i)\wedge
    \sigma_1(x_{s+b_i},y_{s+i-1},y_i) \wedge \sigma_1(x_{s+c_i},y_{s+i-1},y_i))
    \end{array}
    \\
    \Phi'(y_1,y_{2s})= & \; \exists y_2 \dots\exists y_{2s-1}
\;
 \Phi
\end{align*}
Plainly, $\Phi'(y_1,y_{2s})$ has additionally more free $x$-variables but we will have special need to refer to the two extreme $y$-variables, $y_1$ and $y_{2s}$, which will be substituted by other variables. In our construction the $x$-variables in instances of $\Psi$ will never change.

 It remains to show how to add quantifiers to $\Psi$. Let us begin with an instance $\Psi(y_1,y_{2s})=\Phi'(y_1,y_{2s})$ and deal with the quantifiers of $I$ from the innermost to the outermost. Universal quantification is trivial, we just add the quantifiers $\forall x_i$. It is more complicated with the existential quantifier because we need $x_{i}$ to be from $\{0,1\}$
    and we cannot just write $\exists x_i$ because Existential can cheat by choosing $x_i=2$.
    Nevertheless, the following trick suggested by Miroslav Ol\u{s}\'ak solves the problem.
    To express $\exists x_{i}$ we substitute our formula $\Psi(v,v')$ by $\Psi'(v,v')$ defined as
    $$\exists z \forall x_{i} \exists z' \Psi(z,z') \wedge \sigma_0(x_{i},v,z') \wedge \sigma_1(x_{i},v',z').$$
    Thus, instead of adding the existential quantifier to $x_{i}$ 
    we add the universal quantifier to $x_{i}$,
    two existential quantifiers, and two additional constraints. Note that we also renamed some variables. Finally, we set $\Psi(v,v')$ to $\Psi'(v,v')$ defined as $\Psi(v,v') \wedge v=b \wedge v'=2$. The new existential variables we have added (labelled either as $z$ or $v$) we will call $z$-variables. Note that $y_0$ and $y_{2s}$ are both $y$-variables that become $z$-variables under renaming.
    %Note that in the new formula  
    %the variables $y_{-1}$ and $y_{k+1}$ play the role of 
    %$y_{0}$ and $y_{k}$ in $\Phi$.

($\Psi \in \QCSP(\{\sigma_0,\sigma_1\})$ implies $I\in \mathrm{co\mbox{-}QNAE3SAT}$)

Let us duplicate the inward play of the quantifiers of $I$ in $\Psi$ with the proviso that existentially quantified variables $x_i$ in $I$ are played by Universal in $\Psi$ according to the following rule (whose variable names make sense in line with the iterative creation of the formula). If $z$ was chosen to be equal to $v$ then set $x_{i}=0$, else set $x_i=1$. Let us designate this (partial) strategy of Universal as \emph{well-behaved}, and note that this strategy yields $z=z'$ implies $v=v'$. Let us see why. If $v=z$, then $x_i=0$ means $\sigma_1(x_i,v',z')$ means $v'=z'$ and the assumption $z=z'$ yields $v=v'$. If $v \neq z$, then $x_i=1$ means $\sigma_0(x_i,v,z')$ means $v=z'$ implies  $z\neq z'$ immediately. 

Thus, after unwinding the quantifiers, we have something remaining that satisfies $\exists y_2 \dots \exists y_{2s-1} \wedge \Phi \wedge y_1 \neq y_{2s}$. It follows that at some point $j$ in $\Phi$ we have $y_j \neq y_{j-1}$. If $j\leq s$, then $(x_{a_j},x_{b_j},x_{c_j})$ is $(0,0,0)$, if $j>s$, then $(x_{a_{s-j}},x_{b_{s-j}},x_{c_{s-j}})$ is $(1,1,1)$.

($I\in \mathrm{co\mbox{-}QNAE3SAT}$ implies $\Psi \in \QCSP(\{\sigma_0,\sigma_1\})$.)

Let us duplicate the inward play of the universal variables of $I$ appearing in $\Psi$ by the rule that $0$ remains $0$; and $1$ and $2$ become $1$. Let us duplicate the play of existential variables in $I$ according to the following rule (whose variable names make sense in line with the iterative creation of the formula). If $x_i=0$ (in $I$), then choose $z=v$ (in $\Psi$); and if $x_i=1$, then choose $z=v'$. Suppose, in $\Psi$, that Existential plays $z=v$, then assuming Universal plays $x_i=0$, Existential plays $z'=v'$. Suppose that Existential plays $z=v'$, then assuming Universal plays $x_i=1$, Existential plays $z'=v$.

Let us first argue this strategy is complete for Existential, by arguing that if Universal deviates from his well-behaved strategy in playing of the universal variables of $\Psi$ that came from existential variables in $I$, then he always loses. Suppose Existential plays $z=v$ and Universal plays differently from $x_i=0$. Then Existential may play $z'=z$. Then all the existential $z$-variables and $y$-variables further in the formula may be played by existential to $z=z'$ and she will win. Suppose Existential plays $z\neq v$ and Universal plays differently from $x_i=1$. Then Existential may play $z'=z$. Then all the existential $z$-variables and $y$-variables further in the formula may be played by existential to $z=z'$ and she will win.

Now let us assume that Universal (well-)behaves himself with his response to Existential on the universal variables of $\Psi$ coming from existential variables in $I$. Eventually, we will have played all the $z$-variables and be left needing to satisfy  $\exists y_2 \dots \exists y_{2s-1} \Phi$ with some assignment already existing to $y_1$ and $y_{2s}$. Since we already proved that well-behaviour yields $v\neq v'$ implies $z \neq z'$, it follows that $y_1,y_{2s} \in \{b,2\}$ and $y_1\neq y_{2s}$ .

We may assume that the resulting instance of  $\mathrm{co\mbox{-}QNAE3SAT}$ in $I$ has a clause $j$ that is either $(0,0,0)$ or $(1,1,1)$. Suppose first it is $(1,1,1)$, which arises from a setting in $\Phi$ of $(x_{a_j},x_{b_j},x_{c_j})\in \{1,2\}^3$.  Existential plays in $\Phi$ as follows. She plays $y_2,\ldots,y_{s+j-1}=y_1$ and $y_{s+j},\ldots,y_{2s-1}=y_{2s}$. Let us look at the interesting conjunction in $\Phi$, which is $\sigma_1(x_{a_j},y_{s+j-1},y_{s+j})\wedge
    \sigma_1(x_{b_j},y_{s+j-1},y_{s+j}) \wedge \sigma_1(x_{c_j},y_{s+j-1},y_{s+j})$, and note that this is satisfied trivially as $(x_{a_j},x_{b_j},x_{c_j})\in \{1,2\}^3$. The fact that the other parts are satisfied is straightforward since $y_{i}=y_{i-1}$.


Suppose now it is $(0,0,0)$, which arises from a setting in $\Phi$ of $(x_{a_j},x_{b_j},x_{c_j})=(0,0,0)$.  Existential plays in $\Phi$ as follows. She plays $y_2,\ldots,y_{j-1}=y_1$ and $y_j,\ldots,y_{2s-1}=y_{2s}$. Let us look at the interesting conjunction in $\Phi$, which is $\sigma_0(x_{a_j},y_{j-1},y_{j})\wedge
    \sigma_0(x_{b_j},y_{j-1},y_{j}) \wedge \sigma_0(x_{c_j},y_{j-1},y_{j})$, and note that this is satisfied trivially as $(x_{a_j},x_{b_j},x_{c_j})=(0,0,0)$. The fact that the other parts are satisfied is straightforward since $y_{i}=y_{i-1}$.
}
\end{proof}


{\color{red}A binary operation $f$ is called \emph{$0$-stable}
if $f(x,0) = x$ and $f(x,2) = 2$.
A binary operation $f$ is called \emph{$1$-stable}
if $f(x,1) = x$ and $f(x,2) = 2$.
A ternary operation $f$ is called \emph{$01$-stable}
if $f(x,0,1) = x$ and $f(x,2,2) = 2$.
Notice that by adding a dummy variable we can make 
a $01$-stable operation from a 0-stable or 1-stable operation.
Recall that 
$s_2$ is the semilattice operation such that
$s_2(a,b) = 2$ whenever $a\neq b$.

By $\QCSP^{2}(\Gamma)$ recall we denote the decision problem 
where the input in a $\QCSP(\Gamma)$ instance
is a $\Pi_{2}$ formula, that is a formula of the form $\forall x_1 \dots\forall x_{n} \exists y_1\dots\exists y_s \Phi.$
The following lemma shows that using 
a 01-stable operation we can reduce 
$\QCSP(\Gamma)$ to $\QCSP^{2}(\Gamma)$.
}

\begin{proof}
{\color{blue!20!black!50!green}
 The reduction will be from the complement of (monotone) \emph{Quantified Not-All-Equal 3-Satisfiability} (co-QNAE3SAT) which is co-PSpace-hard (see \cite{papa}) and consequently also PSpace-hard (as PSpace is closed under complement). Consider an instance $I$ of co-QNAE3SAT of the form
 $$\exists x_{2n}\forall x_{2n-1}\dots\exists x_{2}\forall x_{1}
 \mathrm{AE}_{3}(x_{a_1},x_{b_1},x_{c_1})\vee\dots\vee\mathrm{AE}_{3}(x_{a_s},x_{b_s},x_{c_s}),$$
 where 
$\mathrm{AE}_3 = \{(0,0,0),(1,1,1)\}$.
Let us define the equivalent instance of 
$\QCSP(\{\sigma_0,\sigma_1,\{b\},\{2\}\})$.
Let
\begin{align*}
    \Phi= & \bigwedge_{1 \le i \le s}
    \begin{array}{c}
    (\sigma_0(x_{a_i},y_{i-1},y_i)\wedge
    \sigma_0(x_{b_i},y_{i-1},y_i) \wedge \sigma_0(x_{c_i},y_{i-1},y_i)) \\
    (\sigma_1(x_{s+a_i},y_{s+i-1},y_{s+i})\wedge
    \sigma_1(x_{s+b_i},y_{s+i-1},y_{s+i}) \wedge \sigma_1(x_{s+c_i},y_{s+i-1},y_{s+i}))
    \end{array}
    \\
    \Phi_{0}(y_1,y_{2s})= & \; \exists y_2 \dots\exists y_{2s-1}
\;
 \Phi
\end{align*}
It can be checked that $\Phi$ encodes the quantifier-free part of the instance 
$I$.
In fact, if $y_{0}\neq y_{2s}$ 
and $x_{1},\dots,x_{2n}\in\{0,1\}$, then they are equivalent. 
It remains to explain how to add quantifiers to $\Phi_{2n}$.

Let us define $\Phi_{1},\Phi_{2},\dots,\Phi_{2n}$ inductively.
For $k=0,1,2,\dots,n-1$ put
\begin{align*}
\Phi_{2k+1}&:= \forall x_{2k} \Phi_{2k},\\
\Phi_{2k+2}&:= \exists y_{2s+k}\forall x_{2k-1} \exists y_{-k}  \;\;\Phi_{2k}
\wedge \sigma_0(x_{2k+1},y_{2s+k+1},y_{-k}) \wedge \sigma_1(x_{2k-1},y_{-k-1},y_{-k})
\end{align*}
Note that the only free variables of $\Phi_{2k+1}$
are $x_{2k+2},\dots,x_{2n},y_{-k}, y_{2s+k}$, and 
the only free variables of $\Phi_{2k}$
are $x_{2k+1},\dots,x_{2n},y_{-k}, y_{2s+k}$.

\begin{sublem}
Suppose $k\in\{0,1,\dots,n\}$, $y_{-k},y_{2s+k}\in\{b,2\}$, 
$y_{-k}\neq y_{2s+k}$. 
Then 
\begin{enumerate}
    \item $\Phi_{2k}$ holds on 
    $x_{2k+1},\dots,x_{2n}\in\{0,1\}$ IFF
    $\exists x_{2k}\forall x_{2k-1}\dots\exists x_{2}\forall x_{1}
 \mathrm{AE}_{3}(x_{a_1},x_{b_1},x_{c_1})\vee\dots\vee\mathrm{AE}_{3}(x_{a_s},x_{b_s},x_{c_s}),$ holds;
    \item $\Phi_{2k+1}$ holds on 
    $x_{2k+2},\dots,x_{2n}\in\{0,1\}$ IFF
        $\forall x_{2k+1}\exists x_{2k}\dots\exists x_{2}\forall x_{1}
 \mathrm{AE}_{3}(x_{a_1},x_{b_1},x_{c_1})\vee\dots\vee\mathrm{AE}_{3}(x_{a_s},x_{b_s},x_{c_s}),$ holds; 
     \item If the variable $x_{i}$ appears in $I$
    and $i\in \{2k+1,2k+2,\dots,2n\}$, 
    then $\Phi_{2k}$ holds whenever $x_{i}=2$;
    \item If the variable $x_{i}$ appears in $I$
    and $i\in \{2k+2,2k+2,\dots,2n\}$, 
    then $\Phi_{2k+1}$ holds whenever $x_{i}=2$.
\end{enumerate}
\end{sublem}
\begin{proof}
We prove by induction on $k$.
(1) and (3) for $k=0$ follows from the definition of $\Phi_{0}$.
Let us prove ....

\end{proof}

The above claim implies that 
$\Phi_{2n}$ is equivalent to $I$ if we send $y_{-n}$ to $b$ and 
$y_{2s+n}$ to $2$.
Thus, the equivalent instance of $\QCSP(\{\sigma_0,\sigma_1,\{b\},\{2\}\})$ 
is 
$$\exists y_{-n} \exists y_{2s+n} \Phi_{2n} \wedge 
(y_{-n}=b) \wedge  (y_{2s+n}=2).$$
}
\end{proof}




Consider solutions of the new instance
such that 
$y_{i} = f_{i}(x_{1},\ldots,x_{n})$
for every $i$. \textcolor{red}{A solution for the new instance will also have Skolem functions for each of $y^0_i$ and $y^1_i$ making it of size $4n$ including the $x_i$. However we will repress the additional $2n$ terms in our tuple representation for reasons of space. For a certain such solution,} let $N$ be the minimal number such that 
$f_{N}$ depends on $x_{j}$ for some $j>N$. In fact, we would like that there is some solution such that this number does not exist as then this is also a solution of the old instance. But for now assume for contradiction that such an $N$ does exist and we choose it to be \textcolor{red}{maximal} among all the solutions.
{\color{blue}Since 
$(f_{1},\ldots,f_{n})$ gives us a solution of $\Phi_{N}^0$, 
the following tuple is a solution of $\Phi$
%\begin{align*}
$$(x_{1},\ldots,x_{N},0,\ldots,0,
f_{1}(x_{1},\ldots,x_{n}),\ldots,
f_{N}(x_{1},\ldots,x_{n}),f_{N+1}^0(x_{1},\ldots,x_{n}),
\ldots,f_{n}^0(x_{1},\ldots,x_{n}))$$
%(x_{1},\ldots,x_{N},1,\ldots,1&,
%f_{1}(x_{1},\ldots,x_{n}),\ldots,
%f_{N}(x_{1},\ldots,x_{n}),f_{N+1}^1(x_{1},\ldots,x_{n}),
%\ldots,f_{n}^1(x_{1},\ldots,x_{n}))
%\end{align*}
for every $x_{1},\ldots,x_{n}$ and some functions $f_{N+1}^0,\ldots, f_{n}^0$.
%\textcolor{red}{This solution to $\Phi$ has a canonical extension to an enlarged tuple which was the assumed solution to the whole quantifier-free part of the new instance, however we will not write this extra part of the enlarged tuple for reasons of space.} 
Note that we could see this tuple (with an additional term written and another omitted) rather as
$$(x_{1},\ldots,x_{N},0,\ldots,0,
f_{1}(x_{1}),\ldots,f_{N-1}(x_{1},\ldots,x_{N-1}),
f_{N}(x_{1},\ldots{n}),f_{N+1}^0(x_{1},\ldots,x_{n})
\ldots)$$
as we assume $f_i$ depends only on $x_1,\ldots,x_i$ for $i< N$.
Consider all the evaluations of the variables 
$x_{N+1},\ldots,x_{n}$ to obtain $3^{n-N}$ solutions of $\Phi$, 
then apply the semilattice operation to them to obtain
one solution $\alpha^0(x_{1},\ldots,x_{N})$ of the form
$$(x_{1},\ldots,x_{N},0,\ldots,0,
f_{1}(x_{1}),\ldots,
f_{N-1}(x_{1},\ldots,x_{N-1}),
e_{N}^0(x_{1},\ldots,x_{N}),
%g_{N+1}(x_{1},\ldots,x_{N}),
\ldots,e_{n}^0(x_{1},\ldots,x_{N})).$$
Note that $e_{N}^0(x_{1},\ldots,x_{N})$ is equal to $c$ if 
$f_{N}(x_{1},\ldots,x_{N},a_{N+1},\ldots,a_{n})=c$ for every $a_{N+1},\ldots,a_{n}$, 
and 
$e_{N}^0(x_{1},\ldots,x_{N})=2$ otherwise.
}

{\color{blue}
Doing the same with the solution of $\Phi_{N}^1$ we get 
a solution $\alpha^1(x_{1},\ldots,x_{N})$ of $\Phi$ of the form
$$(x_{1},\ldots,x_{N},1,\ldots,1,
f_{1}(x_{1}),\ldots,
f_{N-1}(x_{1},\ldots,x_{N-1}),
e_{N}^1(x_{1},\ldots,x_{N}),
%g_{N+1}(x_{1},\ldots,x_{N}),
\ldots,e_{n}^1(x_{1},\ldots,x_{N})).$$
Note that $e_{N}^0=e_{N}^1$.
}

%Let us build a solution of the new instance.
%Denote the quantifier free part of the new instance by $\Psi$.
%We need to find an assignment to all the $y$-variables 
%Put 
%$y_{i} = f_{i}(x_1,\dots,x_{n})$ for $i<n$, 
%$y_{i} = 
{\color{blue}
It remains to 
apply the 01-stable operation $g$ to
$(x_{1},\ldots,x_{n},f_{1}(x_{1},\ldots,x_{n}),\ldots,f_{n}(x_{1},\ldots,x_{n}))$, 
$\alpha^0(x_{1},\ldots,x_{N})$, and 
$\alpha^1(x_{1},\ldots,x_{N})$ 
to obtain a solution of the instance 
such that $f_{N}$ doesn't depend on $x_{N+1},\ldots,x_{n}$. \textcolor{red}{Recalling that we should have been applying always our polymorphisms to the $4n$-tuples involving Skolem functions for each of the $y^0_i$ and $y^1_i$, this gives also a new solution to the new instance,
%Also, applying $g$ to a solution of $\Phi_{j}^{c}$ and 
which gives us a contradiction to the maximality} of $N$ over all solutions.
}

Now let us define the evaluations $f'_1,\ldots,f'_n$ for the existential variables in the original instance by $f'_i(x_1,\ldots,x_i)=f_i(x_1,\ldots,x_i, x_{i+1},\ldots,x_n)$ where $x_{i+1},\ldots,x_n$ are chosen arbitrarily (as we proved $f$ does not depend on them).
%WE NEED TO DEFINE THE EVALUATIONS TO $y_{i}^{0}$ in each $\Phi_{i}$.



\subsection{Examples of Constraint Languages}

In this section we will show an example of a constraint language 
on $\{0,1,2\}$ for every case of Theorem~\ref{ThreeElementClassification} and explain  informally why it gives the respective complexity class.

Case (1). $\Pol(\Gamma)$ has the PGP property and has a WNU operation, 
and $\QCSP(\Gamma)$ is in P.
We can build a constraint language $\Gamma$ with a single ternary relation $x-y+z=1 \mod 3$.

Case (2). 
$\Pol(\Gamma)$ has the PGP property but has no WNU operation, 
and $\QCSP(\Gamma)$ is NP-complete.
We can  take a single ternary relation $\{(1,0,0),(0,1,0),(0,0,1)\}$ that does not involve $2$. As a result universal quantifiers do not play any role and can be ommited, therefore 
the problem is equivalent to the CSP over the relation $\{(1,0,0),(0,1,0),(0,0,1)\}$ 
which is known to be NP-complete \cite{Schaefer}.

Case (3). 
$\Pol(\Gamma)$ has the EGP property and
has no WNU operation, 
and $\QCSP(\Gamma)$ is PSpace-complete.
We can take the closely related single ternary relation $$\{(x,0,0),(0,x,0),(0,0,x) : x \in \{1,2\} \}.$$ The QCSP over this language is equivalent to the QCSP over 
the relation $\{(1,0,0),(0,1,0),(0,0,1)\}$ on the domain $\{0,1\}$ which is known to be PSpace-complete \cite{BBCJK}.


Case (4). $\Pol(\Gamma)$ has the EGP property and $\Pol(\Gamma)$ does not contain $f$ such that 
$f(x,a)=x$ and $f(x,c) = c$, where $a,c\in\{0,1,2\}$, 
and $\QCSP(\Gamma)$ is PSpace-complete.
Unlike case (3), $\Gamma$ may have a WNU polymorphism.
Let $\tau$ be the ternary relation on $\{0,1,2\}$
consisting of all tuples 
$(a,b,c)$ such that $\{a,b,c\}\neq \{0,1\}$.
Then the complement to $\tau$ is 
equal to $\mathrm{NAE}_{3}$, where 
$\mathrm{NAE}_{3} = \{0,1\}^{3}\setminus \{(0,0,0),(1,1,1)\}$.
Put $$\sigma(x_{1},x_{2},x_{3},y_{1},y_{2}) =
(y_{1},y_{2}\in\{0,2\})\wedge (\tau(x_{1},x_{2},x_{3})\vee (y_{1}=y_{2})).$$
We claim that $\Gamma = \{\sigma,x=0,x=1,x=2\}$ satisfies the case (4) and $\QCSP(\Gamma)$ is PSpace-complete
(see Section~\ref{HardnessSection} for the detailed explanation).
Note that $\Gamma$ is preserved by the semilattice operation 
$s_{2}$, where $s_{2}(x,y)=2$ whenever $x\neq y$.
The reduction will be from the complement of (monotone) \emph{Quantified Not-All-Equal 3-Satisfiability} (co-QNAE3SAT) which is co-PSpace-hard (see \cite{papa}) and consequently also PSpace-hard (as PSpace is closed under complement). 
 Consider the quantifier-free part of the instance of co-QNAE3SAT
 $$\neg (\mathrm{NAE}_3(z^1_1,z^2_1,z^3_1) \wedge \ldots \wedge \mathrm{NAE}_3(z^1_k,z^2_k,z^3_k)),$$
 which is equivalent to 
 $$\left(\mathrm{AE}_3(z^1_1,z^2_1,z^3_1) \vee \ldots \vee \mathrm{AE}_3(z^1_k,z^2_k,z^3_k)\right).$$
 Something very similar can be defined by 
$\Phi:=\exists y_{1}\dots\exists y_{k-1}\bigwedge_{i=1}^{k}\sigma(z_{i}^1,z_{i}^2,z_{i}^3,y_{i-1},y_{i}).$
In fact, if we put $y_{0} = 0$ and $y_{k} = 2$, then to satisfy the above formula
we need some tuple $(z_{i}^1,z_{i}^2,z_{i}^3)$ to be from $\tau$, which 
implies on $\{0,1\}$ that this tuple is from $\mathrm{AE}_{3}$.
If $y_{0}=y_{2}\in\{0,2\}$ the formula $\Phi$ always holds.
To prove PSpace-hardness it remains to show how to add quantifiers to the formula $\Phi$:
\begin{itemize}
    \item To add the universal quantifier with $x_{i}$ we just write 
    $\forall x_{i}\; \Phi$.
    \item It is more complicated with the existential quantifier because we need $x_{i}$ to be from $\{0,1\}$. 
    Nevertheless, the following trick suggested by Miroslav Ol\u{s}\'ak solves the problem 
    $$ \exists y_{0} \forall x_{i} \exists y_{k} 
    \left(\Phi \wedge \sigma(x_{i},0,0,y_{-1},y_{k}) \wedge \sigma(x_{i},1,1,y_{k+1},y_{k})\right).$$
    Thus, instead of adding the existential quantifier to $x_{i}$ 
    we add the universal quantifier to $x_{i}$, the existential quantifiers to $y_{0}$ and $y_{k}$, and two additional constraints. Note that in the new formula  
    the variables $y_{-1}$ and $y_{k+1}$ play the role of 
    $y_{0}$ and $y_{k}$ in $\Phi$.
In fact, 
if $y_{0}$ was chosen to be equal to $y_{k+1}$ then
to satisfy the formula for $x_{i}=1$ the formula
$\Phi$ should hold on $x_{i}=1$. 
Otherwise, if $y_{0}\neq y_{k+1}$ then
to satisfy the formula for $x_{i}=0$ the formula
$\Phi$ should hold on $x_{i}=0$. 
Thus,
it holds if and only if there exists $x_{i}\in\{0,1\}$
and we simulated adding the existential quantifier.
\end{itemize}


Cases (5)-(6).
Two concrete constraint languages are presented in Sections~\ref{StrangeOneSection} and 
\ref{StrangeTwoSection}.
These constraint languages 
have the EGP property but the $\QCSP$ over these languages can be solved in polynomial time. 
The polynomial algorithm is based on the following
two ideas.
\begin{itemize}
    \item The existence of the polymorphism 
    $s_{a,c}$ guarantees that 
    it is sufficient (see Lemma \ref{ReductionToQCSP2}) to find a polynomial algorithm for sentences of the 
    form 
    $\forall x_{1}\dots\forall x_{n}
    \exists y_{1} \dots \exists y_{m}\; \Phi$.
    \item 
Since $\Pol(\Gamma)$ has the EGP property, the usual reduction from 
$\QCSP$ to $\CSP$ (without looking at the formula) cannot help because 
theoretically we need to check exponentially many tuples 
$(x_{1},\dots,x_{n})$.
The key idea here is to calculate the list of tuples
$(x_{1},\dots,x_{n})$ we need to check to be sure that 
the formula holds for all the tuples. 
To calculate them we look at the formula
$\Phi$, substitute necessary values to some variables, 
and solve polynomially many tractable CSP instances (we have the semilattice polymorphism).
See the algorithms in Sections~\ref{StrangeOneSection} and \ref{StrangeTwoSection}
for more details.
\end{itemize}

Case (7). The first and probably easiest example of
a constraint language $\Gamma$ such that 
$\QCSP(\Gamma)$ is co-NP-complete is as follows. 
Let $R_{AND}=\begin{pmatrix}
0&0&1&1&2&\cdot\\
0&1&0&1&\cdot&2\\
0&0&0&1&\cdot&\cdot
\end{pmatrix}$ 
and $R_{OR}=\begin{pmatrix}
0&0&1&1&2&\cdot\\
0&1&0&1&\cdot&2\\
0&1&1&1&\cdot&\cdot
\end{pmatrix}$ where columns are tuples of the relations and $\cdot$ means any element of $\{0,1,2\}$, that is $R_{AND}$
and $R_{OR}$ are row-wise the truth table of AND
and OR respectively. 
Put $\Gamma = \{R_{AND}, R_{OR}\}$. The proof 
of co-NP-completeness can be divided into two steps
(see Section~\ref{HardnessSection} for the details):
\begin{itemize}
\item We can compose these relations 
in the same way as we compose the operations 
$AND$ and $OR$ on $\{0,1\}$.
Using this idea we efficiently  define 
(see Lemma~\ref{ANDORHardness}) 
the complement to Not-All-Equal 3-Satisfability.
Hence, adding universal quantifiers make the 
problem co-NP-hard.
\item To show that the problem is in co-NP we need to explain a polynomial strategy for the Existential player. It turns out that to calculate the best move Existential
can assume that all the later choices of the Universal
player are 0. It is also important that the Existential player
should play 2 if several moves are possible. Since the CSP over this language is tractable, after fixing the choice of the Universal player this can be done in polynomial time.

\end{itemize}



--------------------------------------------------------










Assume that 
$a_{i} = 2$, $a_{j} =2$ for some 



Suppose 
$(a_{1},\ldots,a_{n}), (b_{1},\ldots,b_{n})\in \rho$, 
$c_{i} = a_{i}\wedge b_{i}$ for every $i$.
It is not hard to see that 
$(a_{i},b_{i},c_{i})\in AND$.
Since $f$ preserves $AND$,
$(c_{1},\ldots,c_{n})\in\rho$, which means that
$\rho$ is preserved by conjunction.
It remains to show that 
$f(1,a_{1},\ldots,a_{n})=2$ if 
$a_{i} = 2$ for some $i$.
WLOG, we assume that $i=1$.
Since the second variable of $f$ is not dummy, 
there exist $b_{0},b_{1},\ldots,b_{n},b_{1}'$ 
such that 
$$b_{0} = f(b_{0},b_{1},b_{2}\ldots,b_{n})\neq f(b_{0},b_{1}',b_{2},\ldots,b_{n})=2.$$
Assume that 
$b_{0} = 0$. Then by the first property,
$1\in B$, $b_{1}=0$, and $f(0,1,0,\ldots,0) = 2$.
Since $f$ preserves $AND$, 
$$f\begin{pmatrix}
1& 2 &a_2&\dots&a_{n}\\
0 & 0 &0&\dots & 0\\
0 & 1 &0 &\dots & 0
\end{pmatrix} = 
\begin{pmatrix}
f(1,2,a_{2},\ldots,a_{n})\\0\\2
\end{pmatrix}\in AND,
$$ which means that $f(1,a_{1},\ldots,a_{n})=2$.

Assume that 
$b_{0} = 1$. Then by the first property,
$1\in B$, $b_{1}=0$, and $f(0,1,0,\ldots,0) = 2$.
Since $f$ preserves $AND$, 
$$f\begin{pmatrix}
1& 2 &a_2&\dots&a_{n}\\
0 & 0 &0&\dots & 0\\
0 & 1 &0 &\dots & 0
\end{pmatrix} = 
\begin{pmatrix}
f(1,2,a_{2},\ldots,a_{n})\\0\\2
\end{pmatrix}\in AND,
$$ which means that $f(1,a_{1},\ldots,a_{n})=2$.




%Then for every tuple
%$(a_{0},a_{1},\ldots,a_{n})$ such that 
%$f(a_{0},\ldots,a_{n}) = 0$ we have 
%$f(h(a_{0}),\ldots,h_{n}(a_{n})) = 0$.
%Since $f$ preserves $AND$, for any three tuples 
%$(a_{0},a_{1},\ldots,a_{n})$,
%$(b_{0},b_{1},\ldots,b_{n})$,
%$(c_{0},c_{1},\ldots,c_{n})$
%such that $(h(a_{i}),h(b_{i}),c_{i})\in AND$ for every $i$
%and 
%$f(a_{0},\ldots,a_{n}) = (b_{0},\ldots,b_{n}) = 0$
%we have 
%$f(c_{0},c_{1},\ldots,c_{n})=0$.
%Note that $c_{i}$ can be arbitrary if $a_{i}\neq 0$ or $b_{i}\neq 0$.
%Let $\mathbf a^{0},\mathbf a^{1},\ldots,\mathbf a^{s}$
%be all the tuples such that $f(\mathbf a) = 0$.

\end{proof}

\begin{lem}
$\Pol(\Gamma) \supseteq  \mathcal C$.
\end{lem}

\begin{proof}
Suppose we have an operation 
$f_{B,\rho}(x_{0},\ldots,x_{n})$ for 
appropriate $B$ and $\rho$.
Let us show that 
$f_{B,\rho}$ preserves $AND$. Assume that we apply $f_{B,\rho}$ to a matrix whose columns are from $AND$.
Let $\alpha_{1},\alpha_{2},\alpha_{3}$ be the rows of the matrix.

If $f(\alpha_{1}) =f(\alpha_{2}) =0$, then $\alpha_{1}(1) = \alpha_{2}(1) = \alpha_{1}(i+1) =\alpha_{2}(i+1) = 0$ for every $i\in B$.
This implies $\alpha_{3}(1) = \alpha_{3}(i+1)=0$ for every $i\in B$.
Therefore $f(\alpha_{3}) = 0$.
If $f(\alpha_{1}) =2$ or $f(\alpha_{2}) =2$ then the result is in $AND$.
If $f(\alpha_{1}) =f(\alpha_{2}) =1$, then $\alpha_{1}(1) = \alpha_{2}(1) = 1$
and if we remove the first elements of $\alpha_{1}$ and $\alpha_{2}$ we get tuples from $\rho$.
Since $\rho$ is preserved by conjunction, $f(\alpha_{3}) = 1$.
It remains to consider the case when $f(\alpha_{1}) =0$ and $f(\alpha_{2}) = 1$.
By the definition of $f_{B,\rho}$, $\alpha_{1}(1) = \alpha_{1}(i+1)$ for every $i\in B$, 
$\alpha_{2}\in\{0,1\}^{n}$.
This implies $\alpha_{3}(1) = \alpha_{3}(i+1)=0$ for every $i\in B$.
Therefore $f(\alpha_{3}) = 0$.

Let us show that 
$f_{B,\rho}$ preserves $\delta$. Assume that we apply $f_{B,\rho}$ to a matrix whose columns are from $\delta$.
Let $\alpha_{1},\alpha_{2}$ be the rows of the matrix.
If $f(\alpha_{1}) \neq 0$ then it is obvious.
Suppose $f(\alpha_{1})=0$, then  
$\alpha_{1}(1) = \alpha_{1}(i+1)=0$ for every $i\in B$.
By the definition of $\delta$ we have  
$\alpha_{3}(1) = \alpha_{3}(i+1)=0$ for every $i\in B$.
Therefore $f(\alpha_{3}) = 0$.





%\begin{lem}
%Suppose 
%$R_{1}$ is an AND-type relation, 
%$R_{2}=\begin{pmatrix}
%0&1&1&1&2&2&2\\
%1&0&1&2&0&1&2
%\end{pmatrix}
%$.
Then $\xi_{n}$ can be pp-defined 
over $\{R_{1},R_{2}\}$ by a polynomial size formula.
\end{lem}

\begin{proof}
Put 
$\rho_{0}(x,y) = 
\exists R_{1}(x,x,z) \wedge R_{2}(z,y)$
For a tuple $(c_{1},c_{2},c_{3})\in\{0,1\}^{3}$
we define 
Let $\delta_{1}(x,y) = R_{1}(x,x,y)$, 
$\delta_{0} = R_{2}$.
$$\rho_{c_{1},c_{2},c_{3}}(x,y,z,u) = 
\exists x' \exists y' \exists z'\exists t
R_{1}(x',y',t)
\wedge 
R_{1}(z',t,u)
\wedge
\delta_{c_{1}}(x,x')
\wedge
\delta_{c_{2}}(y,y')
\wedge
\delta_{c_{3}}(z,z')
$$
It is not hard to see that 
$\rho_{c_{1},c_{2},c_{3}}(c_{1},c_{2},c_{3},e)$
is true if and only if $e=1$.
If $(d_{1},d_{2},d_{3})\neq (c_{1},c_{2},c_{3})$, 
then $(d_{1},d_{2},d_{3},0)\in\rho_{c_{1},c_{2},c_{3}}$.



$t$ can be equal to 0 unless 
$\{x,y,z\} = \{0,1\}$.

$\rho 
=\bigwedge_{i} R_{2}(x_{i},x_{i}')\wedge \bigwedge_{i} R_{2}(y_{i},y_{i}')\wedge
\bigwedge_{i} R_{2}(z_{i},z_{i}')\wedge
R_{1}(x_{1},y_{1}',z_{1})
\wedge 
R_{1}(y_{1},x_{1}',z_{1})
\wedge 
R_{1}(x_{1},z_{1}',z_{1})
\wedge 
R_{1}(z_{1},x_{1}',z_{1})
\wedge 
R_{1}(z_{1},y_{1}',z_{1})
\wedge 
R_{1}(y_{1},z_{1}',z_{1})
$



\end{proof}


Similarly, put 
$\gamma_{i} = nu_{B,C}^{2k}(\alpha_{1},\ldots,\alpha_{i-1},\alpha_{2k},
\alpha_{i+1},\ldots,\alpha_{2k})$ for $i\in\{1,\ldots,s\}$.
In the same way we can show that 
$\gamma_{i}\in\rho$ and $\gamma_{i}(N)\neq 2$ for every $i\in\{1,\ldots,s\}$.

Since $\gamma_{i}(N)\neq \beta(N)$,
we have $\alpha_{i}(N)\neq \alpha_{2k}(N)$ for every 
$i\in\{1,\ldots,s\}$.
The function $nu_{B,C}^{2k}$ can return $0$ or $1$
only if all elements of the input but one are equal. 
Since $\gamma_{i}(N)\neq 2$ for every $i\in\{1,\ldots,s\}$, 
we should have one of the following two cases:
\begin{enumerate}
    \item $s = 1$.
    \item $s = 2$, $\alpha_{1}(N),\alpha_{2}(N)\in C$.
\end{enumerate}

If $s=1$ then $\alpha_{1}(i)\neq \alpha_{2}(i)$










First, let us show that 
for any 
$(a_{1},\ldots,a_{n})$ such that $a_{i}=2$
there exists $a_{n+1}\in\{0,2\}$
such that $(a_{1},\ldots,a_{n},a_{n+1})\in R_{and,n}$.
For $i\in\{1,2,\dots,n\}$ put 
$b_{i}= c_{i} = a_{i}$ if $a_{i}\in\{0,1}$;
put $b_{i} = 0$ and $c_{i} = 1$ if $a_{i}=2$.
Let 
$b_{n+1} = 0$, $c_{n+1} = c_{1}\wedge \dots\wedge c_{n}$.
Note that 
$(b_{1},\dots,b_{n+1}),(c_{1},\dots,c_{n+1})\in R_{and,n}$.
We apply the semilattice $s$ to these tuples and obtain 
a tuple $(a_{1},\ldots,a_{n},a_{n+1})$, 
where $a_{n+1} = s(0,c_{n+1})\in\{0,2\}$.
In the same way we can show that 
for any 
$(a_{1},\ldots,a_{n})$ such that $a_{i}=2$
there exists $a_{n+1}\in\{1,2\}$
such that $(a_{1},\ldots,a_{n},a_{n+1})\in R_{or,n}$.




In this subsection we prove the classification for 
the special case we consider in this section.
\begin{lem}\label{ANDORIMPLIESAUX}
$\begin{pmatrix}
0 & 1 & 2 & 0 & 2\\
0 & 0 & 0 & 2 & 2 
\end{pmatrix}$ can be pp-defined from 
an AND-type relation and OR-type relation.
\end{lem}

\begin{proof}
By $R_{and,2}$ and 
$R_{or,2}$ we 
denote an AND-type and an OR-type relation, respectively.
Since 
$R_{and,2}$ is preserved by the semilatice $s$, 
$s$ applied to the tuples 
$(0,1,0),(1,0,0)\in R_{and,2}$ gives 
$(2,2,0)\in R_{and,2}$.
Similarly,
$(0,1,1),(1,0,1)\in R_{or,2}$ implies
$(2,2,1)\in R_{or,2}$.
Also, $s$ applied to $(0,0,0),(1,1,1)$ 
gives $(2,2,2)$, which should be in both relations 
$R_{and,2}$ and $R_{or,2}$.

Then the required 
relation can be defined by the following formula:
$$\delta(x,y) = \exists z\; R_{and,2}(x,x,z)\wedge R_{or,2}(z,z,y).$$
\end{proof}





\subsection{Remove}


\begin{lem}\label{ANDAlmostAlways}
Suppose $\Gamma$ is preserved by a 0-stable operation.
Then $\Gamma$ contains an 
AND-type relation or 
the relation $\begin{pmatrix}
0& 1& 2\\
1& 0& 2
\end{pmatrix}$.
\end{lem}

\begin{proof}
%Let us define a $(2k+1)$-ary operation $f$.
%It returns $1$ on the tuples 
%$01^i01^{2k-i-1}$,  for $i=0,1,\dots,2k-1,$
%and $0 1^{2k}$. It returns $2$ otherwise.
%This operation is not $\{0,2\}\{1,2\}$-projective, 
%therefore there should be a relation $\rho$ in $\Gamma$ that is not preserved by $f$.

Since $f_{\{1\},\{0\}}^{2k}$ is not $\{0,2\}\{1,2\}$-projective,
$\Gamma$ is not preserved by $f_{\{1\},\{0\}}^{2k}$.
By Lemma \ref{almostf} there exists a relation $\rho\in\Gamma$
satisfying one of the two cases (see notations in Lemma~\ref{almostf}).

%We are going to argue in the same way as in the proof of Lemma~\ref{almostNU}.
%We assume that $\rho$ is a relation of the minimal arity that is not preserved by $f$.
%Let $N$ be the arity of $\rho$. 
Consider tuples 
$\alpha_{0},\alpha_{1},\ldots,\alpha_{2k}\in\rho$ such that 
$f(\alpha_{0},\alpha_{1},\ldots,\alpha_{2k})=\beta\notin \rho$.
Put $\alpha_{i}' = \proj_{1,\ldots,N-1}(\alpha_{i})$ 
for every $i$, $\beta' = \proj_{1,\ldots,N-1}(\beta)$.
Since $\rho$ is a relation of the minimal arity 
for every $i$ there exists $\beta_{i}\in\rho$ that differs 
from $\rho$ only in the $i$-th coordinate.

We consider a matrix $M$ whose columns 
are $\alpha_{0},\dots,\alpha_{2k}$.
As in the proof of Lemma~\ref{almostNU} we
can show that 
every row of this matrix contains different elements, and 
all rows should be different.

Assume that $\beta$ has at least two elements equal to $2$ and they appear at the $i$-th and $j$-th positions.
Then $s(\beta_{i},\beta_{j}) = \beta$, which contradicts the fact that 
$s$ preserves $\rho$.
Assume that $\beta$ has no $2$. 
Every row of the matrix must have exactly one element different from all other elements,
and the result of applying $f$ to every row is the popular element of the row. Since we have $N\le k$ rows and $2k$ columns, there should be a column among $\alpha_{1},\ldots,\alpha_{2k}$ equal to $\beta$, which contradicts our assumptions.
W.l.o.g., we assume that $\beta(N) = 2$ 
(otherwise we just permute variables of $\rho$).


Put $\alpha_{i}' = \proj_{1,\ldots,N-1}(\alpha_{i})$ 
for every $i$, $\beta' = \proj_{1,\ldots,N-1}(\beta)$.
We know that for every $i\in\{1,\dots,N-1\}$ the $i$-th row contains exactly one element different from the others.
Since $N\le k$, at least $k+1$ of the tuples 
$\alpha_{1}',\ldots,\alpha_{2k}'$ are equal to $\beta'$.
W.l.o.g., we assume that 
$\alpha_{s+1}' = \ldots = \alpha_{2k}' = \beta'$, $\alpha_{i}'\neq\beta'$ 
for every $i\in\{1,\ldots,s\}$, where $s< N$.  
Since not all elements of the first row of the matrix are equal, 
we have $s\ge 1$.

Replace the first column of the matrix $M$ by $\alpha_{2k}$
and consider 
$nu_{B,C}^{2k}(\alpha_{2k},\alpha_{2},\alpha_{3},\ldots,\alpha_{2k}) 
= \gamma_{1}$.
Since $\alpha_{1}'\neq \beta'$, there should be a row
in the new matrix whose elements are equal.
Therefore, $\gamma_{1}\in\rho$, otherwise 
we consider $\alpha_{2k},\alpha_{2},\alpha_{3},\ldots,\alpha_{2k}$
instead of the original sequence, and get a contradiction 
with the fact that every row should contain at least two different elements.
By the definition $\proj_{1,\ldots,N-1}(\gamma_{1}) = \beta'$, 
therefore $\gamma_{1}(N)\neq 2$.
This means that 
at least $2k-2$ among the elements
$\alpha_{2}(N),\ldots,\alpha_{2k}(N)$ are equal 
to $\alpha_{2k}(N)$.
In the same way we can substitute $\alpha_{j}$ instead of $\alpha_{i}$ 
for any $i\in\{1,\dots,s\}$ and $j\in\{s+1,\dots,2k\}$ to conclude that 
$2k-2$ elements among the elements 
$\alpha_{1}(N),\dots,\alpha_{i-1}(N),\alpha_{i+1}(N),\dots,\alpha_{2k}(N)$ 
are equal to $\alpha_{j}(N)$.
Since $\beta(N) = 2$, we also have
$\alpha_{i}(N)\neq\alpha_{j}(N)$.
This implies that 
$\alpha_{s+1}(N) = \dots = \alpha_{2k}(N)\in B$, 
and one of the following cases holds:
\begin{enumerate}
    \item $s = 1$, $\alpha_{2} = \dots = \alpha_{2k}$;
    \item $s = 2$, $\alpha_{1}(N),\alpha_{2}(N)\in C$,
    $\alpha_{3} = \dots = \alpha_{2k}$.
\end{enumerate}
If $s=1$ then $\alpha_{1}(i)\neq \alpha_{2}(i)$ since there should be different elements in every row.


From the proof of Lemma~\ref{almostNU} we know that 
\begin{enumerate}
    \item $\beta$ is an essential tuple and $\rho$ is an essential relation.
    \item In any row of the matrix there should be elements that are not equal.
    \item $\beta(N) = 2$, $\beta_{i}\neq 2$ for $i\neq N$.
    \item $\alpha_{s+1}' = \ldots = \alpha_{2k}' = \beta'$, 
    $\alpha_{i}'\neq\beta'$ for every $i\in\{1,\ldots,s\}$.      
    \item $s=1$ and $N=2$ and $\beta = 12$, or 
    $s=2$, $N=3$ and $\alpha_{0}(3)=0$, $\alpha_{1}(3) =\alpha_{2}(3) = 0$, $\alpha_{3}(3) = \dots=\alpha_{2k}(3)=1$
    and $\beta = 112$.
\end{enumerate}
(I believe we need to make Lemma~\ref{almostNU} stronger to be able to apply it here).

We consider two cases from the last item.
Suppose the relation $\rho$ is binary.
Then it has tuples
$(0,c),(1,d)$ for some $c$ and $d$ but it doesn't have a tuple 
$(1,2)$. 
Since a $0$-stable operation applied to 
$(1,d)$ and $(0,2)$ gives $(1,2)$, we have $(0,2)\notin\rho$.
Since the semilattice preserves $\rho$ 
We cannot have both $(0,1)$ and $(0,0)$ in $\rho$.
Also we cannot have both $(1,1)$ and $(1,0)$ in $\rho$.

Assume that $c=d$. Then $\beta(2) = c$, which contradicts our assumptions.
Assume that $c=0$ and $d=1$, then $\beta(2) = d$, which also contradicts our assumptions.
Therefore, $c=1$ and $d=0$.
Put $\rho'(x,y) = \rho(x,y)\wedge \rho(y,x)$. 
It is not hard to see that 
$\rho'=\begin{pmatrix}
0& 1& 2\\
1& 0& 2
\end{pmatrix}$, which completes this case.

Suppose the relation $\rho$ is ternary.
Then $\rho$ contains the following tuples
$(0,0,0),(1,1,1),(0,1,0),(1,0,0)$, but doesn't contain the tuple
$(1,1,2)$.
Since $\rho$ is preserved by a 0-stable operation, 
$(c,d,2)\notin\rho$ for all $c,d\in\{0,1\}$ (otherwise we apply the 0-stable operation to 
$(1,1,1)$ and $(c,d,2)$ to get a contradiction).
Thus $\rho$ is an AND-type relation.
\end{proof}

\begin{lem}\label{ANDInTheRemaining}
Suppose 
$\delta=\begin{pmatrix}
0& 1& 2\\
1& 0& 2
\end{pmatrix}\in\Gamma$,
then there exists an AND-type relation and an OR-type relation 
in $\Gamma$.
\end{lem}

\begin{proof}
Let us consider an operation 
$f$ of arity $2k+1$ such that 
$f(01^{i}01^{2k-i-1}) = 1$,
$f(10^{i}10^{2k-i-1}) = 0$,
$f(01^{2k}) = 1$,
$f(10^{2k}) = 0$,
and $f$ returns 2 on all other tuples.

Since $f$ is not $\{0,2\}\{1,2\}$- projective, there should be a relation in $\Gamma$ 
that is not preserved by $f$.
Then we do the same as in Lemma~\ref{almostNU}.
%As a result we get a relation $\rho$ which is either binary or ternary.
To consider less cases, we may assume that $\beta$ consists of $1$ and $2$.
If $\beta(i) =0$ then instead of $\rho$ 
we consider the relation
$$\rho'(x_{1},\ldots,x_{N}) = \exists z
\rho(x_{1},\ldots,x_{i-1},z,x_{i+1},\ldots,x_{N})
\wedge \delta(z,x_{i}).$$
It is not hard to see that $\rho'$ satisfies all the properties we required from $\rho$.

Arguing as in Lemma~\ref{almostNU} we can show that 
$\rho$ is either binary or ternary.

Assume that $\rho$ is binary. Then it contains 
$(0,c)$, $(1,d)$ for some $c$ and $d$, but it 
doesn't contain $(1,2)$. 
Arguing as in the previous lemma we obtain $c=1$ and $d=0$. 
But then we get a contradiction with the fact that 
$\beta(2) = 2$ (since $f$ preserves the permutation $\delta$).

Thus $\rho$ should be a ternary relation containing 
$(0,0,0),(1,1,1),(0,1,0),(1,0,0)$. 
Arguing as in the previous lemma we show that 
$\rho$ is an AND-type relation.
\end{proof}




Similar to $nu_{B,c}^{n}$ we define an operation 
$f_{B,C}^{n}$.
By $f_{B,C}^{n}$ we denote 
the operation of arity $n+1$ defined on a tuple 
$(a_{0},a_1,\ldots,a_n)$ as follows. 
If $a_{0}=a_{1} = \dots = a_n$ then return $a_0$.
If $a_{0}\in C$, $a_{1} = \dots = a_{i-1} = a_{i+1} =\dots = a_n\in B$,
$a_{i}\in B\cup C$ for some $i$, then return $a_{j}$, where $j\neq i$.
Otherwise, it return $2$.

Similar to Lemma~\ref{almostNU} we will prove the following lemma.

\begin{lem}\label{almostf}
Suppose $\Gamma$ is not preserved by $f_{B,C}^{2k}$.
Then there exists a relation $\rho\in \Gamma\setminus \Inv(f_{B,C}^{2k})$ of arity $N$ 
such that 
one of the following conditions holds:
\begin{enumerate}
    \item There exist $\alpha_{0},\alpha_{1},\alpha_{2},\alpha_{3}\in\rho$ 
    such that 
    $f_{B,C}^{2k}(\alpha_{0},\alpha_{1},\alpha_{2},\alpha_{3},\alpha_{3},\ldots,\alpha_{3}) = \beta\notin\rho$, 
    $\beta(i) = \alpha_{3}(i)\neq 2$ for $i\in\{1,\ldots,N-1\}$, 
    $\beta(N) = 2$, $\alpha_{0}(N),\alpha_{1}(N),\alpha_{2}(N)\in C$, 
    $\alpha_{3}(N) \in B$.
    \item 
    There exist $\alpha_{0},\alpha_{1},\alpha_{2}\in\rho$ 
    such that 
    $f_{B,C}^{2k}(\alpha_{0},\alpha_{1},\alpha_{2},\alpha_{2},\ldots,\alpha_{2}) = \beta\notin\rho$,
    $\beta(i) = \alpha_{2}(i)\neq 2$ for every $i\in\{1,\ldots,N-1\}$, 
    $\beta(N) = 2$. 
\end{enumerate}
Additionally, $\rho$ is a relation of the minimal arity in $\Gamma$ that is not preserved by $f_{B,C}^{2k}$.
\end{lem}

\begin{proof}
We assume that $\rho$ is a relation of the minimal arity that is not preserved by $f_{B,C}^{2k}$.
Let $N$ be the arity of $\rho$. 
Consider tuples 
$\alpha_{0},\alpha_{1},\ldots,\alpha_{2k}\in\rho$ such that 
$f_{B,C}^{2k}(\alpha_{1},\ldots,\alpha_{2k})=\beta\notin \rho$.
Arguing as in Lemma~\ref{almostNU} we can show that 
for every $i$
there exists a tuple $\beta_{i}\in\rho$ that differs from $\beta$ only in the $i$-th coordinate. 

We consider the matrix $M$ 
whose columns are $\alpha_{0},\alpha_{1},\ldots,\alpha_{2k}$. 
Since $\rho$ is a relation of the minimal arity, every row should contain different elements and 
all rows of the matrix should be different.

Assume that $\beta$ has at least two elements equal to $2$ and they appear at the $i$-th and $j$-th positions.
Then $s(\beta_{i},\beta_{j}) = \beta$, which contradicts the fact that 
$s$ preserves $\rho$.
Assume that $\beta$ has no $2$. 
If we remove the first column of the matrix, then 
each row in the obtained matrix contains at most one element different from all other elements.
Since we have $N\le k$ rows and $2k+1$ columns, there should be a column among $\alpha_{1},\ldots,\alpha_{2k}$ equal to $\beta$, which contradicts our assumptions.
W.l.o.g., we assume that $\beta(N) = 2$.

Put $\alpha_{i}' = \proj_{1,\ldots,N-1}(\alpha_{i})$ 
for every $i$, $\beta' = \proj_{1,\ldots,N-1}(\beta)$.
If we remove the first column from the matrix, then for every $i\in\{1,\dots,N-1\}$ the $i$-th row contains at most one element different from the others.
Since $N\le k$, at least $k+1$ of the tuples 
$\alpha_{1}',\ldots,\alpha_{2k}'$ are equal to $\beta'$.
W.l.o.g., we assume that 
$\alpha_{s+1}' = \dots = \alpha_{2k}' = \beta'$, $\alpha_{i}'\neq\beta'$ 
for every $i\in\{1,\ldots,s\}$, where $s< N$.  
Since $\beta(N)=2$ and $s$ preserves $\rho$, we also obtain 
$\alpha_{s+1} = \dots = \alpha_{2k}$.

If $s=0$, then the second condition of this lemma holds.

Suppose $s\ge 1$.
In the same way as in the proof of Lemma~\ref{almostNU} 
we substitute $\alpha_{j}$ instead of $\alpha_{i}$ 
for any $i\in\{1,\dots,s\}$ and $j\in\{s+1,\dots,2k\}$.
We assume 
$f_{B,C}^{n}(\alpha_{0},\dots,\alpha_{i-1},\alpha_{j},\alpha_{i+1},\dots,\alpha_{2k})\in\rho$, since otherwise we may replace $\alpha_{i}$ by $\alpha_{j}$ 
and reduce $s$.
We therefore conclude that 
$2k-2$ elements among the elements 
$\alpha_{1}(N),\dots,\alpha_{i-1}(N),\alpha_{i+1}(N),\dots,\alpha_{2k}(N)$ 
are equal to $\alpha_{j}(N)$.
Since $\beta(N) = 2$, we also have
$\alpha_{i}(N)\neq\alpha_{j}(N)$.
This implies that 
$\alpha_{s+1}(N) = \dots = \alpha_{2k}(N)\in B$, 
and one of the following cases holds, which completes the proof:
\begin{enumerate}
    \item $s = 1$, $\alpha_{2} = \dots = \alpha_{2k}$;
    \item $s = 2$, $\alpha_{1}(N),\alpha_{2}(N)\in C$,
    $\alpha_{3} = \dots = \alpha_{2k}$.
\end{enumerate}
\end{proof}


==> old/rebuttal.tex <==
Response: We thank the reviewers for their careful reading of the paper and strong (insightful) comments. Where we made a substantial change to the paper we have made this with blue text. In some cases we have totally rewritten proofs for reasons of clarity. For example, this is the case for Lemma 18.

***************************************************

Summary of major decisions for editor (which appear also in the appropriate places in the rebuttal below):

a) We followed most of the recommendations, below we comment on each of them individually, justifying if we did not follow them.

b) We decided not to exclude the clone theory part. We thought excluding it was a good idea until we tried to implement it. Dima collected all the clone theory claims together but the new imaginary paper still seemed like an appendix to the QCSP paper. The ideas there are nice, but the facts proved there, are too specific. So, now we don't see a nice clone theory paper. Also, we still have some clone theory proofs in the Strange Structure parts, which should stay there. Therefore, we decided to keep this in the main paper after all.

c) There was an error in Lemma 17. Shortly before the reviews were sent to us, Dima noticed this error, which was noted by one of the reviewers also. The proof was faulty. One of the PSpace-complete cases has moved to co-NP-complete. 

**************************************************

Reviewer #1

Comments:
The presentation is impeccable, and the paper even features a "Section dependency diagram" to help the reader focus on the parts they are most interested in efficiently. I only have a few comments.

p1,l38-40: I don't think this is accurate: where PCSPs have indeed appeared more recently, I believe that finitely-bounded, homogeneous infinite-domain CSPs have been studied since the beginning of the 2000s just like QCSPs (although the reference [1] you give seems to be the first printed appearance of an algebraic conjecture).

Response: This is true, but we still claim QCSP is older. We write: "The exact dates of these classification questions are not exactly cast in stone but the question for QCSPs dates at least to the announcement of the classification for the 2-element case in \cite{Schaefer}". There exist infinite-domain finitely bounded homogeneous CSPs that were studied before this, but not a recognisable program of classification. For QCSPs, the program is already apparent in Schaefer (we claim). I am not sure of the first example of what we now call a promise CSP arose, but again it is a long time ago. However, the systematic program is more recent. If the reviewer knows better please let us know, we are happy to give a better account here!

p2,l23: The theorem is true without the "with all constants" assumption, by (Barto, Oprsal, Pinsker, The wonderland of reflections). You do mention afterwards that the assumption can be made complexity-wise, but the reader could be mislead to believe the WNU criterion only holds in that case. The comment on the core afterwards is probably not helpful since adding the constants is arguably more the sophisticated move.

Response: This has now been noted and a citation attached.

p3l40: "maximal class": in what sense?

Response: Indeed, this was never precise. We have changed the claim to "among the larger natural classes".

p4l12: again, the core could simply be avoided.

Response: Core is now omitted.

p6l36: I found the cases of the theorem a bit confusing, in particular, i found it hard to match them with Figure 2. Perhaps it would be easier if one could see explicitly the conditions for (7). Why don't you define a set F of functions as in item (4) already before the theorem together with the other functions; then EGP and no f in F is (4), EGP + WNU + F puts us into co-NP, ... At the moment the diagram seems to suggest EGP + WNU + F is equivalent to s_a,b?

Response: Done.

p6l47 Some readers might appreciate just a few words about the meaning of this example.

Response: We explain that, since $x-y+z\bmod 3$ preserves $\Gamma$, $\Pol(\Gamma)$ has the PGP and can be reduced to CSP which is tractable by Gaussian elimination.

p10l36: A full stop is missing.

Response: Done.

p12l16: "containing x=a": At first I was not sure how to read it, in particular since a is not quantified or specified in any way, and then moreover in l 20 an element a in A is chosen.

Response: Indeed, x=a is a unary relation. There is no need to then re-choose a, as a is chosen. This is corrected.

p20l33: Why is tau_n this relation? Definition 1 seems to allow more possibilities.

Response: We believe the two are the same. Note that that it is "{0,1} not subseteq {xi,yi,zi}" and not "{0,1} not equal {xi,yi,zi}".

p21l50: A full stop is missing.

Response: Done.

p39l10: Why can assumption (2) be made? Why assumption (4)? (The latter is particularly confusing since on p10 it is claimed that the interesting cases have alpha\cap beta=\emptyset.)

Response: We added something before the assumption list. For all EGP to be \alpha\beta-projective, we now reference the Zhuk JCTA paper. The alpha\cap beta=\emptyset was a typo; it should have been, and now is, \neq \emptyset.

Reviewer #2

The only caveat I have, which I raise for the authors and editors to consider, is that a significant fraction of the manuscript (pages 30-38) is essentially devoted to proving the following partial classification of idempotent {0; 2}{1; 2}-projective clones on {0; 1; 2} which are determined by a finite set of relations:
If the clone contains neither a 0-stable or 1-stable operation, then it has one of three pairs of invariant relations; if the clone contains both 0-stable and 1-stable operations, then it has invariant AND-like and OR-like relations; and if the clone has a 0-stable operation but no 1-stable operation, then it either contains f_0,2 or {g_0;2; s_0;2} or has x \neq 0 \/ y = z as an invariant relation.
This partial classification is needed to complete the classification of QCSPs on a 3-element domain. But is its proof appropriate in JACM? In my opinion, the paper would be improved by replacing this proof with a statement of the partial classification and relegating its proof elsewhere.

Response: We thought this was a good idea until we tried to implement it. Dima collected all the clone theory claims together but the new imaginary paper still seems like an appendix to the QCSP paper. The ideas there are nice, but the facts we prove there, are too specific. 
Thus, now we don't see a nice clone theory paper. Also, we still have some clone theory proofs in the Strange Structure parts, which should stay there. Therefore, we decided to keep this in the main paper after all.

1. Page 5, first two paragraphs of S1.2: you say that in S2 you will show how we can combine two constraint languages in one constraint language." Then you say that in Ss3-6 you will explain how to combine two constraint languages in one constraint language." How are these different? What are you trying to say here?

Response: The presentation in S2 gives a forward pointer to S5 for a proof. "Show" and "explain" are used interchangeably here, but actually the "explain" would much better be "prove". Then the difference is apparent. We made this change.

2. Page 10, 3rd paragraph: a factor should be a homomorphic image of a subalgebra (not what you have written).

Response: We have switched round the order of these two.

3. Page 10, last paragraph: here you define the phrase "is \alpha\beta-projective to coordinate i." But later in the paper you use the phrase "is an \alpha\beta-projection onto the i-th coordinate." I suggest that you decide which phrase you want to use and stick with it; or introduce both here.

Response: We now use "to" in this regard always (and never "onto").

4a. Page 12, proof of Lemma 13:
* Your proof requires |A| > 1 (in the 3rd paragraph, where you argue that you can assume that no variable appearing in an NAE3 relation is universally quantified). Why not say at the start that WLOG you can assume |A| > 1.

Response: We have added to the statement of the lemma that |A|>1 and explicitly commented where this is needed.

4b. In the first sentence of the proof, you write "choose an element a in A." That's not quite right; you need to choose a with the property that x = a is in Gamma (which is possible by hypothesis).

Response: Yes, done.

5. Lemma 14: this is a beautiful reduction, but I found the explanation to be sloppy in places and hard to follow.

(a) Page 13, 2nd paragraph: I assume that the variables yi mentioned here, in \sigma_1(xi, yi), are new variables - rather than the existentially quantified variables in the generic representation of a QCSP instance mentioned at the top of page 10. Perhaps you could state this.

Response: Yes, they are new. We now say this. As well, we say I1 and I2 have disjoint variables.

(b) Page 13, 3rd paragraph: More detail and perhaps an example will help here. 

Response: An example has been added and more explanation given in terms of a game-theoretic strategy.

(c) Page 13, 6th paragraph: you state that there is a reduction to connected components, but you never explain this. Please explain it. In particular, does this reduction need to wait until after the "typing" of variables and other simplifications? If yes, then doesn't that complicate these simplifications?

Response: We now explain this reduction to connected components which can be done before typing and other simplifications.

(d) Page 14, line 4: your claim that "adding the constraint x1 = x2 doesn't change the result" is not at all obvious. Please add more detail, including:
(i) how to modify a winning strategy for Existential on K to a strategy for Existential on K with x1 = x2 adjoined; (ii) why the modified strategy is winning (is this one place where connectivity of the Gaifmann graph is required?).

Response: An explanation is now added.

(e) Page 14, lines 6-7: sloppy and not obvious. I think you mean the hypothesis to be "Suppose we have in K some sigma1(x1, y1) ^ sigma2(x2; y2) and y is quantified before x1 and x2" similar to the previous paragraph. Also, why not help the reader by justifying your claim, e.g. by telling how to modify a winning strategy for Existential for the "before" formula to get a winning strategy for Existential for the "after" formula.

Response: Done. These are the only instances of the variable y, this is why it is working.

6. Lemma 15, statement (page 14, last line): reduce by 1 the subscripts in |A2|.|A3| + |A2| + |A3|.

Response: Done.

7. Page 15, S6: Until now, despite your statement on page 3, "We will henceforth assume Gamma contains all constants," you have been careful to acknowledge requiring constants in your constraint languages when you need them (cf. the statements of Theorems 1{3, Conjecture 1, Theorem 5, Lemma 11). I think that is good; please don't change that! But here in S6 you stop that practice. The proof of Lemma 18 needs h0 to be idempotent; the proof of Lemma 19 needs Gamma to contain all constants. Please either repeat your statement from page 3 here; or specify in the statements of Lemmas 18 and 19 (and any others that need it) that Gamma contains all constants.

Response: In the new write-up this comment applies to the following results where I add what we did about it.
Lemma 17: Two constants are explicit.
Lemma 18: 01-stable is now defined idempotent.
Lemma 19: Constants are not needed as CSP(Gamma,0,2) is in P due to the semilattice polymorphism. We added clarification here.
Lemma 20: Constants not needed.
Lemma 21: At present the constant 0 is needed. I added that it is needed.
Lemma 22: Two constants are explicit.
Section 9 assumes all constants and the statements in Section 10 assume all constants.

8. Lemma 17, statement: here you need to explicitly include the constants: QCSP({sigma,sigma_1,sigma_2} \cup { constants}) etc. are PSpace-hard.

Response: Done. (This lemma was completely rewritten.)

9. Page 15, line -: in the \bigwedge_s+1 \leq i \leq 2s conjuncts, change the sub-subscripts in x^1_ai,x^1_bi,x^1_ci to i-s.

Response: Done, though the subscripts have been changed to s+i not s-i. (This lemma was completely rewritten.)

10. Page 15, line -7: anticipating the argument that follows, it would be helpful here to note that, conversely, if y0 and y2s are assigned the same value in {0, 2}, then Existential can choose all other yj to have that same value and this will satisfy Phi for all choices of x^0_i,x^1_i in {0,1}.

Response: This proof has been rewritten as a formal induction. (This lemma was completely rewritten.)

11. Page 16, 1st paragraph of (I in co-QNAE3SAT implies Psi in QCSP(sigma, sigma_0, sigma_1)): I don't follow the argument here, and I wonder if the reduction is incorrect.

Response: Shortly before the reviews were sent to us, Dima noticed this error also. This proof is faulty. One of the PSpace-complete cases has moved to co-NP-complete. (This lemma was completely rewritten.)

12. Page 16, line -10: change "Recall" to "Assume".

Response: There are no longer any instances of "recall" in this proof. (This lemma was completely rewritten.)

13. Page 17, line 16: change i \leq N to i < N.

Response: This seems to be page 18. The proof of this lemma has been rewritten as a formal induction. This comment no longer applies.

14. Page 20, 2nd paragraph of S7: in "recalling" the definition of tau_n, note that it is with respect to alpha = {0; 2} and beta = {1; 2}.

Response: Done.

15. Page 21, 1st line: by "such relations" you mean rho (or copies of rho), so why not just say that?

Response: Done.

16. Page 21, statement of Lemma 22: before stating this Lemma, I urge you to remind the reader of your (nonstandard) convention stated on page 10: when you write Phi(x1,...,xn) you mean the projection of the relation defined by Phi onto the variables (x1,...,xn). (I had forgotten, and this confused me.)

Response: Done.

Also, do you require the variables (x1,...,xn) to be distinct, or allow repeated
variables? I am guessing the latter in the definition of R'.

Response: We allow the repetitive variables. We added a comment to preliminaries.

17. Page 21, line 5: your proof of Lemmas 22 and 23 requires < to be the coordinatewise order on {0; 1}^n, not the lexicographic order.

Response: This is now noted.

18. Page 21, statement of Lemma 22: some hypotheses are missing, I think; at least you will need to add some hypotheses if you want to keep your current proof. For example, let Phi be
Rand,2(x1; x1; x3) /\ Rand,2(x3; x3; x1) /\ Rand,2(x2; x2; x2)
and let R = Phi(x1; x2; x3) = {(a; b; c) in A^3 : a = c}. If alpha = 011, then alpha(3) = 1 and you state that this implies v(x3) = 1. But the only elements of R coordinatewise less than alpha are 000 and 010, so C_x3 = {0} and thus v(x3) = 0.

Response: It should be fine now. In the example the required variable is $x_3$. Thus C_{x_{3}} = {0}, D_{x_{3}} = {1}.

19. Page 21 line -5: your proof of Lemma 22 needs h_0,2 to be a polymorphism of
Gamma but the function you have defined is not a polymorphism. It also fails to
satisfy the equation h_0;2(x; y; z) = g_0;2(s_0;2(x1; x3); s_2(x2; x3)) claimed on line -4. I think you want the second case of the definition to be x, if x = 1 and y = z 2 {0; 1}.

Response: Yes! Done.

20. Page 21, line -4: I assume that the reason you note these two equations here is to prove that h0;2 is a polymorphism of Gamma (which you use in the proof of Lemma 23). But this follows only if s0;2 and g0;2 are polymorphisms of Gamma which you don't mention until the last line of the proof of Theorem 28 on page 25. For clarity, you should make that observation here (or earlier), and explicitly note here that the equations imply that h0;2 is a polymorphism.

Response: Done.

Also for clarity, I suggest that you explicitly note in the proof of Lemma 23 where you use the fact that h0;2 is a polymorphism.

Response: We added something here.

Also, in the second equation, change x1; x2; x3 on the right side to x; y; z

Response: Done.

21. Page 24, line -2: the formula you give for f_B,psi(B) isn't valid when B = emptyset.

Response: Done.

22. Page 25, description of the algorithm Solve1: there is none, except for the pseudocode. Please explain in words. Suggestion: replace Di in the pseudocode with Dij . Before giving the pseudocode, define the tuples alpha_1,...,alpha_n (for fixed n)
and explain that on input forall x1 ...  forall xn exists y1 ... exists ys Phi, Solve1 checks x = (0, ..., 0) and x = (1, ..., 1), then calculates for each pair (i; j) the set Dij of possible values for yj when x = alpha_i (they must be nonempty), and lastly checks another s values of x determined by the Dij.

Response: Done.

23. Page 25, -7: in the context of showing alpha_i in R for all i, you mention Di \neq emptyset. To which pass through the loop "for j := 1, ..., s do" are you referring?

Response: This is now clarified.

24. Page 25, line -5: before assuming that "D1 calculated for the variable y is equal to 1," you need to establish that y in {y1, ..., ys} (i.e., y notin {x1, ..., xn}).

Response: Done.

25. Page 26, proof of Corollary 30: it would be a kindness to the reader to point out that s0;2 is 0-stable (justifying the application of Lemma 18).

Response: Done.

26. Page 26, definition of Fy(x1, ..., xn): you say that this is a partial operation "on {0; 1}," which suggests to me that dom(Fy) subseteq {0; 1}^n. But in Lemma 35 you allow 2^{i-1}02^{n-i} in dom(Fy). Make the wording more clear.

Response: Done.

27. Page 27, line -2: the wording suggests that you are defining sigma2n for the first time, when really you are recalling the definition.

Response: Right. We changed denote to recall.

28. Page 28, lines 1-2: these two sentences already appeared on page 20.

Response: We removed the definitions 
of $\tau_n$ and $\sigma_n}$ and refer to the previous section.

29. Page 28, proof of Lemma 37: maybe it's worth pointing out that if V is the set of variables in Phi, then your same argument gives an injection from a set A^2n not sigma_n of size 2^n to the set of all subsets of V of size at most k. Hence if N = |V| then N \geq 2^{n/k}.

Response: Done.

30. Page 28, Solve2: before proving Lemma 39, please explain in words what the pseudocode for Solve2 is doing.

Response: Done.

31. Page 28, line -3: in addition to explaining that lines 7-17 correctly find the minimal 1-set for each yj if it exists, it would be helpful to note that (obviously) the minimal 1-set for xi is 0^{i-1}0^{n-i}.

Response: Done.

32. Page 30, First paragraph of S9: perhaps state that this list of assumptions remains in effect up to but not including the statement of Theorem 58.

Response: Done. (Theorem 58 became Theorem 60.)

33. Page 30, statement of Lemma 41: in your applications of this Lemma you use additional consequences of the statement which you nowhere explain. To help the reader, I suggest adding these additional consequences here, and explain
them in the proof. These consequences are:
(a) In part (1): alpha_3(i) in B for all i < N.
(b) In part (2): alpha_2(i) in  B for all i < N. Moreover, if C = A then N = 2, alpha_2(N) notin B, and [without loss of generality] alpha_1 = (2; 2).

Response: Done.

34. Page 30, proof of Lemma 41: perhaps mention at the start of the proof that the hypotheses imply N \geq 2.

Response: Done.

35. Page 31, line 11: the deduction alpha_s+1(N) = ... = alpha_2k(N) is correct, but you cannot assume that the common value is in B when s = 1.

Response: Done.

36. Page 31, line -15 change nu^2k_B,C to nu^2k_A,A.

Response: Ok.

37. Page 32, last paragraph of the proof of Lemma 43: if you adopted my suggestion in item 33(b), then here you will already have sigma1 = (2, 2).

Response: Done.


38. Page 33,
(a) lines 2-4: the formula for rho1 works only if a = b = 1; if a = b = 0 then you need to reverse the arguments of delta in the definition of rho1.
(b) lines 5-7: similarly, the formulas for rho2, rho3 only work when (a, b) = (0, 1).

Response: Done.

39. Page 33, statement of Lemma 46: I suggest changing it to "The set of all Boolean functions represented by Gamma is a clone generated by one of the following sets: {0; 1}, {+; 0; 1}, {\/; 0; 1}, {/\; 0; 1}, {/\;\/; 0; 1}, or {/\;\neg; 0; 1}."
You would just need to add one more sentence to the proof, pointing to Post's lattice for example. I think that this tightening of Lemma 46 would be a big help to the reader not intimately familiar with clones on {0,1}.

Response: Done.


40. Page 33, remark following the statement of Lemma 46: change "0 and 1" to "{0}, {1} and =." (Or delete the sentence.)

Response: Done.

41. Page 34, line 5: it wasn't clear to me until Lemma 48 that you intend the domain of f_Gamma to be A^N. (I had guessed that it was {0,1}^N.) Why not tell the reader this when you define f_Gamma.


Response: Done.

42. Page 36, line 7: in addition to noting f1(2; x) = f2(2; x) = 2 (as a consequence of f1 and f2 being {0; 2}{1; 2}-projecting on coordinate 1), could you also note
f2(0; 2) in {0; 2}? That will make it easier for the reader to see why f(0; 2) = 2.

Response: Done.

43. Page 38, line 6: I think the logic will be clearer if you replace "Assume that (0; 1; 2) notin rho" with "Therefore (0; 1; 2) notin rho."

Response: Done (and some words added).

44. Page 38, Theorem 58, statement: you seem to need to add the hypothesis "Gamma is preserved by s2." Otherwise in the proof, after the reduction in the first paragraph, you don't have all of the assumptions at the beginning of S6.

Response: Done.

45. Page 39, proof of Lemma 59, first sentence of 2nd case: change "subset B" to "subuniverse B".

Response: Added subalgebra of Pol(Gamma).

46. Page 39, line -18: change "because of Pol(Gamma)" to "because Pol(Gamma)".

Response: Done.

47. Finally, the manuscript has several occurrences of the following two English
grammatical errors, especially in S9:
* Series of two or more assertions separated by commas, where the intent is to assert their conjunction. You should include the word "and" before the last item in the series. Good examples are
(a) Statement of Lemma 11 (first sentence).
(b) Statements of Lemmas 41 and 56, and Theorem 58.
* Run-on sentences of the form "Suppose A, then B" or "Assume A, then
B." Either change the comma to a semicolon ("Suppose A; then B") or split into two sentences ("Suppose A. Then B."). Good examples are:
(a) Page 15, lines -8 and -7.
(b) Statements of Lemmas 48 and 54, Theorems 50 and 51, and Corollary 55.
(c) Page 38, line 1.
Please find and fix all such errors.

Response: We have dealt with issues of the first type, also searching the document for them ourselves. For the second type, we don't think this is a significant grammatical error. (English is widely known to be a language without a grammar.)

==> old/reductionsNewCopy.tex <==
\section{Reductions and hardness results for the 3-element domain}\label{HardnessSection}


In this section we consider the domain $A= \{0,1,2\}$
and prove all the hardness results we need for the 3-element domain.
{\color{red}An operation $f$ is called \emph{$0$-stable}
if $f(x,0) = x$ and $f(x,2) = 2$.
An operation $f$ is called \emph{$1$-stable}
if $f(x,1) = x$ and $f(x,2) = 2$.
Recall that 
$s_2$ is the semilattice operation such that
$s_2(a,b) = 2$ whenever $a\neq b$.
}

{\color{blue}
We will show how 
$\QCSP(\Gamma)$ can be reduced to a $\Pi_{2}$ formula 
if $\Gamma$ is preserved 
by a 01-stable operation.
}
%Let us define the following relations:
%\[
%\begin{array}{c}
%\sigma = \{0,2\}^2 \cup \{1,2\}^2 \\
%\sigma_0 = \{ (a,b,c) : a \in A, b,c \in \{1,2\}, (a \in \{0,2\} \vee b=c) \} \\
%\sigma'_0 = \{ (a,b,c) : a \in A, b,c \in \{0,2\}, (a \in \{0,2\} \vee b=c) \} \\
%\sigma_1 = \{ (a,b,c) : a \in A, b,c \in \{0,2\}, (a \in \{1,2\} \vee b=c) \} \\
%\sigma'_1 = \{ (a,b,c) : a \in A, b,c \in \{1,2\}, (a \in \{1,2\} \vee b=c) \}
%\end{array}
%\]
\begin{lem}
{\color{blue}
Suppose $b\in\{0,1\}$,  
$$\begin{array}{c}
\sigma_0 = \{ (a_1,a_2,a_3) : a_1 \in A, a_2,a_3 \in \{b,2\}, (a_1 \in \{0,2\} \vee a_2=a_3) \},\\
\sigma_1 = \{ (a_1,a_2,a_3) : a_1 \in A, a_2,a_3 \in \{b,2\}, (a_1 \in \{1,2\} \vee a_2=a_3) \}. 
\end{array}$$
Then $\QCSP(\{\sigma_0,\sigma_1,\{b\},\{2\}\})$ 
is PSpace-hard.}
\label{PSpaceHardness}
\end{lem}


\begin{proof}
{\color{red}
NEED TO BE DONE!
Let us begin with QCSP$(\{\sigma,\sigma_0,\sigma_1\})$. The reduction will be from the complement of (monotone) \emph{Quantified Not-All-Equal 3-Satisfiability} (co-QNAE3SAT) which is co-PSpace-hard (see \cite{papa}) and consequently also PSpace-hard (as PSpace is closed under complement). Consider an instance $I$ of co-QNAE3SAT of the form $(x_{a_1},x_{b_1},x_{c_1}), \ldots, (x_{a_s},x_{b_s},x_{c_s})$ which is a yes-instance precisely when, for all truth assignments to the variables, one among these triples $(x_{a_i},x_{b_i},x_{c_i})$ is either $(0,0,0)$ or $(1,1,1)$. We will use two variables $x^0_i$ and $x^1_i$ to encode each variable $x_{i}$ from the original problem (among the $x_{a_i},x_{b_i},x_{c_i}$). $x_i=0$ will be encoded as $(x^0_i,x^1_i)=(1,0)$ and $x_i=1$ will be encoded as $(x^0_i,x^1_i)=(0,1)$. We start with the formula

\[
\begin{array}{ll}
\Phi= & \bigwedge_{1 \le i \le s} (\sigma_1(x_{a_i}^0,y_{i-1},y_i) \wedge \sigma_1(x_{b_i}^0,y_{i-1},y_i) \wedge \sigma_1(x_{c_i}^0,y_{i-1},y_i)) \wedge \\
& \bigwedge_{s+1 \le i \le 2s} (\sigma_1(x_{a_i}^1,y_{i-1},y_i) \wedge \sigma_1(x_{b_i}^1,y_{i-1},y_i) \wedge \sigma_1(x_{c_i}^1,y_{i-1},y_i))
\end{array}
\]
with the quantifier prefix $\exists y_1 \ldots \exists y_{2s-1}$.  Suppose we imagine our $x$ variables restricted to $\{0,1\}$, then $\Phi$ captures the quantifier-free part of $I$ when either $y_0=0$ and $y_{2s}=2$; or $y_0=2$ and $y_{2s}=0$.

Let the quantifier prefix of $I$ be $Q_nx_n\ldots Q_1x_1$. Starting with $Q_1x_1$, we modify $\Phi$ iteratively in the following way. Let $k$ and $l$ be the minimal and maximal indices appearing in the $y$ variables of $\Phi$, respectively. Note that $k \le 0$ and $l>0$, and that typically $k$ decreases and $l$ increases during our construction. 

If $Q_i$ is a universal quantifier then we add outermost quantification to $\Phi$ of $\forall x^0_i \forall x^1_i$ and do not modify the quantifier-free part.

If $Q_i$ is an existential quantifier then we add outermost quantification to $\Phi$ of $\exists y_k \forall x^0_i \forall x^1_i \exists y_l$ and conjoin $\sigma_1(x^0_i,y_{k-1},y_l) \wedge \sigma_1(x^1_i,y_{l},y_{l+1})$ to the quantifier-free part. The idea is that $y_k$ ``chooses'' $(x^0_i,x^1_i)=(0,1)$ or $(x^0_i,x^1_i)=(1,0)$ in the following fashion.
%
Let us assume that $y_{k-1},y_k,y_l,y_{l+1} \in \{0,2\}$, $y_{k-1} \neq y_{l+1}$, $x^0_i,x^1_i \in \{0,1\}$, $x^0_i \neq x^1_i$, which we shall subsequently see will be the case. At the point Existential plays $y_k$, she knows the values of $y_{k-1}$ and $y_{l+1}$. Let us start with the case $(y_{k-1},y_{l+1})=(0,2)$. If $y_k=0$, then Universal must play $(x^0_i,x^1_i)=(1,0)$ in order to force $y_k \neq y_{l} = 2$. If Universal played $(x^0_i,x^1_i)=(0,1)$, then Existential could get away with $y_k = y_{l} = 0$. If $y_k=2$, then it is the other way around, with Universal having to play $(x^0_i,x^1_i)=(0,1)$ in order to force $y_k \neq y_{l} = 0$. Thus, $y_k=0$ chooses $(x^0_i,x^1_i)=(1,0)$ and $y_k=2$ chooses $(x^0_i,x^1_i)=(0,1)$. The second case of $(y_{k-1},y_{l+1})=(0,2)$ similarly splits into two subcases.

We call the quantifiers of $\Phi$ associated with those from the instance $I$ the \emph{simulation} quantifiers. Let us now ensure that Universal never tries to play some $(x^0_i,x^1_i)$ with $x^0_i=x^1_i$. We will conjoin the following.
\[
\begin{array}{c}
\Delta_0 = \bigwedge_{1 \le i \le n} \left( \sigma_0(x^0_i,z_{i-1},z_i) \wedge \sigma_0(x^1_i,z_{i-1},z_i) \right) \\
\Delta_1 = \bigwedge_{1 \le i \le n} \left( \sigma_1(x^0_i,t_{i-1},t_i) \wedge \sigma_1(x^1_i,t_{i-1},t_i) \right) \\
\end{array}
\]
The idea here is that, if (for any $i$) $x^0_i=x^1_i=0$, then $\Delta_0$ holds on a tuple with $(z_0,z_n)=(1,2)$; while if  (for any $i$) $x^0_i=x^1_i=1$, then $\Delta_1$ holds on a tuple with $(t_0,t_n)=(0,2)$.

Let $k$ and $l$ be, respectively, minimal and maximal indices appearing in the final formula $\Phi$. We claim that the original instance $I$ is equivalent to the following instance $\Psi$ of $\QCSP(\{\sigma,\sigma_0,\sigma_1\})$.
\[ y_k=0 \wedge \Phi \wedge y_l=t_0 \wedge \Delta_1 \wedge \sigma(t_n,z_n) \wedge \Delta_0 \wedge z_0=1 \]
where we make this prenex and add quantifiers $\exists t_0 \ldots \exists t_n \exists z_0 \ldots \exists z_n \exists y_k \exists y_l$ innermost. For pedagogical reasons we prefer to imagine the quantifiers $\exists y_1 \ldots \exists y_{2s-1}$ to be truly innermost, but since existential quantifiers commute with one another, this is no problem.


%## BARNY Below, it is probably not clear that by 
% x_{i}^{0},x_{i}^{1}=2 you mean that just one of them is equal to 2.
% fixed
($I\in \mathrm{co\mbox{-}QNAE3SAT}$ implies $\Psi \in \QCSP(\{\sigma,\sigma_0,\sigma_1\})$.) Let us begin by arguing that if Universal at any point plays some $x^0_i=x^1_i$ or $x^0_i,x^1_i =2$ then Existential will surely win. Suppose some $x^0_i=x^1_i=0$, then we know $\Delta_0$ holds on a tuple with $(z_0,z_n)=(1,2)$. It doesn't matter how the simulation quantifiers have been evaluated, we just set $t_n,\ldots,t_0=0$ and $y_k,\ldots,y_l=0$ (and evaluate the $z_i$ in between $z_0$ and $z_n$ as in the tuples that satisfies $\Delta_0$). Suppose some $x^0_i=x^1_i=1$, then we know $\Delta_1$ holds on a tuple with $(t_0,t_n)=(0,2)$. Set $z_n,\ldots,z_0=1$ and $y_k,\ldots,y_l=0$. Suppose now some $x^0_j=2$ or $x^1_j=2$, we find  again that $\Delta_0$ holds on a tuple with $(z_0,z_n)=(1,2)$
or 
$\Delta_1$ holds on a tuple with $(t_0,t_n)=(0,2)$.
%## BARNY. The case below was already considered.
% fixed
%while if  (for any $i$) $x^0_i=x^1_i=1$, then $\Delta_1$ holds on a tuple with $(t_0,t_n)=(0,2)$
Thus, we reduce to previous cases.

We now know that Universal must play each $(x^0_j,x^1_j)$ as either $(0,1)$ or $(1,0)$ if he is to have any chance of winning on $\Psi$. We have assumed Existential has a winning strategy in $I$ and this can be copied in $\Psi$ according to how we described the rules for how each $\exists y_k \forall x^0_i \forall x^1_i \exists y_l$ selects either  $(x^0_i,x^1_i)=(0,1)$ or $(x^0_i,x^1_i)=(1,0)$.  After the quantifiers are played in $I$, we will have in $\Psi$ that either $(y_0,y_{2s})=(0,2)$ or $(y_0,y_{2s})=(2,0)$. 
%## Barny. It is not really symmetric since we send y_k to 0.
% Thus it should be always (0,2)
% fixed
Recall $(y_0,y_{2s})=(0,2)$. After Existential has played a winning strategy in $I$, suppose that it is the triple $(x_{a_j},x_{b_j},x_{c_j})$ that is either $(0,0,0)$ or $(1,1,1)$. 
%## BARNY. The sentence below should be different for 
% (0,0,0) and (1,1,1).
% fixed
If it is $(0,0,0)$, then we evaluate $y_i$ as $0$ for $0 \le i \le j$ and $2$ for $j < i \le 2s$. If it is $(1,1,1)$, then we evaluate $y_{i}$ as $0$ for $0 \le i \le s+j$ and $2$ for $s+j < i \le 2s$ 
Then set $t_n,\ldots,t_0=2$ and $z_n,\ldots,z_0=1$. Finally, $y_k=0$ and $y_l=2$.

($\Psi \in \QCSP(\{\sigma,\sigma_0,\sigma_1\})$ implies $I\in \mathrm{co\mbox{-}QNAE3SAT}$.) Let us consider only evaluations of $\Psi$ in which each $(x^0_i,x^1_i)$ is either $(0,1)$ or $(1,0)$.  We play through the simulation quantifiers of $\Psi$ copying what is chosen in $I$.  We must have $z_n,\ldots,z_0=1$, $t_n,\ldots,t_0=2$, $y_l=2$ due to the constraints $y_k=0\wedge y_l=t_0 \wedge \sigma(t_n,z_n) \wedge z_0=1$. Furthermore, let us assume Universal plays $(x^0_i,x^1_i)$ that came from existential variables of $I$ according to their selecting $y_k$. It follows that $y_0\neq y_{2s}$ and there must be a $0 \le i \le 2s$ so that $y_i\neq y_{i+1}$. This then selects some triple of $I$ that is either $(0,0,0)$ (if $i<s$) or $(1,1,1)$ (if $i\ge s$).

Now let us show what adjustments need to be made for the problem $\QCSP(\{\sigma'_0,\sigma_1\})$ (the case $\QCSP(\{\sigma_0,\sigma'_1\})$ is symmetric). We replace $\Delta_0$ with 
\[ \Delta'_0 = \bigwedge_{1 \le i \le n} \left( \sigma'_0(x^0_i,z_{i-1},z_i) \wedge \sigma'_0(x^1_i,z_{i-1},z_i) \right) \]
and build the final instance of $\Psi$ according to
\[ y_k=0 \wedge \Phi \wedge y_l=t_0 \wedge \Delta_1 \wedge t_n=z_n \wedge \Delta'_0 \wedge z_0=2 \]
where we make this prenex and add quantifiers $\exists t_0 \ldots \exists t_n \exists z_0 \ldots \exists z_n \exists y_k \exists y_l$ innermost. 

($I\in \mathrm{co\mbox{-}QNAE3SAT}$ implies $\Psi \in \QCSP(\{\sigma'_0,\sigma_1\})$.) Let us begin by arguing that if Universal at any point plays some $x^0_i=x^1_i$ or $x^0_i,x^1_i =2$ then Existential will surely win. Suppose some $x^0_i=x^1_i=0$, then we know $\Delta'_0$ holds on a tuple with $(z_0,z_n)=(0,2)$. It doesn't matter how the simulation quantifiers have been evaluated, we just set $t_n,\ldots,t_0=0$ and $y_k,\ldots,y_l=0$ (and evaluate the $z_i$ in between $z_0$ and $z_n$ as in the tuples that satisfies $\Delta'_0$). Suppose some $x^0_i=x^1_i=1$, then we know $\Delta_1$ holds on a tuple with $(t_0,t_n)=(0,2)$. Set $z_n,\ldots,z_0=2$ and $y_k,\ldots,y_l=0$. 
%## BARNY Below, it is probably not clear that by 
% x_{j}^{0},x_{j}^{1}=2 you mean that just one of them is equal to 2.
% fixed
Suppose now some $x^0_j=2$ or $x^1_j=2$, we find  again that $\Delta'_0$ holds on a tuple with $(z_0,z_n)=(0,2)$
or $\Delta_1$ holds on a tuple with $(t_0,t_n)=(0,2)$.
%## BARNY. The case below was already considered.
% fixed
%while if  (for any $i$) $x^0_i=x^1_i=1$, then $\Delta_1$ holds on a tuple with $(t_0,t_n)=(0,2)$. 
Thus, we reduce to previous cases.

We now know that Universal must play each $(x^0_j,x^1_j)$ as either $(0,1)$ or $(1,0)$ if he is to have any chance of winning on $\Psi$. We have assumed Existential has a winning strategy in $I$ and this can be copied in $\Psi$ according to how we described the rules for how each $\exists y_k \forall x^0_i \forall x^1_i \exists y_l$ selects either  $(x^0_i,x^1_i)=(0,1)$ or $(x^0_i,x^1_i)=(1,0)$.  After the quantifiers are played in $I$, we will have in $\Psi$ that either $(y_0,y_{2s})=(0,2)$ or $(y_0,y_{2s})=(2,0)$. 
%## Barny. It is not really symmetric since we send y_k to 0.
% Thus it should be always (0,2)
Recall $(y_0,y_{2s})=(0,2)$. After Existential has played a winning strategy in $I$, suppose that it is the triple $(x_{a_j},x_{b_j},x_{c_j})$ that is either $(0,0,0)$ or $(1,1,1)$. 
%## BARNY. The sentence below should be different for 
% (0,0,0) and (1,1,1).
% fixed
If it is $(0,0,0)$, then we evaluate $y_i$ as $0$ for $0 \le i \le j$ and $2$ for $j < i \le 2s$. If it is $(1,1,1)$, then we evaluate $y_{i}$ as $0$ for $0 \le i \le s+j$ and $2$ for $s+j < i \le 2s$ 
Then set $t_n,\ldots,t_0=2$ and $z_n,\ldots,z_0=2$. Finally, $y_k=0$ and $y_l=2$.

($\Psi \in \QCSP(\{\sigma'_0,\sigma_1\})$ implies $I\in \mathrm{co\mbox{-}QNAE3SAT}$.) Let us consider only evaluations of $\Psi$ in which each $(x^0_i,x^1_i)$ is either $(0,1)$ or $(1,0)$.  We play through the simulation quantifiers of $\Psi$ copying what is chosen in $I$.  We must have $z_n,\ldots,z_0=2$, $t_n,\ldots,t_0=2$, $y_l=2$ due to the constraints $y_k=0\wedge y_l=t_0 \wedge t_n=z_0 \wedge z_n=2$. Furthermore, let us assume Universal plays $(x^0_i,x^1_i)$ that came from existential variables of $I$ according to their selecting $y_k$. It follows that $y_0\neq y_{2s}$ and there must be a $0 \le i \le 2s$ so that $y_i\neq y_{i+1}$. This then selects some triple of $I$ that is either $(0,0,0)$ (if $i<s$) or $(1,1,1)$ (if $i\ge s$).
}\end{proof}


By $\QCSP^{2}(\Gamma)$ recall we denote the decision problem 
where the input in a $\QCSP(\Gamma)$ instance
is a $\Pi_{2}$ formula, that is a formula of the form $\forall x_1 \dots\forall x_{n} \exists y_1\dots\exists y_s \Phi.$


%By $h_{0}$ we denote the operation such that $h_{0}(0,1) %= 0$, $h_{0}(a,a) = a$ and it returns 2 otherwise.
%Similarly, by $h_{1}$ we denote the operation such that %$h_{1}(1,0) = 1$, $h_{1}(a,a) = a$ and it returns 2 %otherwise.




The following lemma shows that using 
a 01-stable operation we can reduce 
$\QCSP(\Gamma)$ to $\QCSP^{2}(\Gamma)$.


\begin{lem}\label{ReductionToQCSP2}
{\color{blue}
Suppose $\Gamma$ is preserved by $s_2$ and a 01-stable operation $h_{01}$.
Then an instance 
$$\forall x_1\exists y_1 \forall x_2 \exists y_2 \dots \forall x_{n} \exists y_{n} \Phi$$
of $\QCSP(\Gamma)$ is equivalent to 
$$\forall x_1\forall x_2 \dots \forall x_{n}
\exists \exists  
((\exists' \exists' \Phi_{1}^0\wedge \Phi_{1}^1)\wedge 
(\exists' \exists' \Phi_2^0 \wedge \Phi_2^1) \wedge \dots \wedge (\exists' \exists' \Phi_n^0\wedge \Phi_n^1)
),$$
where 
$$
\Phi_{i}^0 = \Phi^{x_{i+1},\ldots,x_{n}, y_{i+1},\ldots,y_{n}}_{x_{i+1}^0,\ldots,x_{n}^0,y_{i+1}^0,\ldots,y_{n}^0} \wedge x_{i+1}^0 = 0 \wedge \dots\wedge x_{n}^0 = 0,
$$
$$
\Phi_{i}^1 = \Phi^{x_{i+1},\ldots,x_{n}, y_{i+1},\ldots,y_{n}}_{x_{i+1}^1,\ldots,x_{n}^1,y_{i+1}^1,\ldots,y_{n}^1} \wedge x_{i+1}^1 = 1 \wedge \dots\wedge x_{n}' = 1,
$$
(note that $\Phi_{n}^0 =\Phi_{n}^1 = \Phi$) and by 
$\exists \exists$ and $\exists' \exists'$ we mean that we add all necessary existential quantifiers for $y$-variables without a superscript and with a superscript, respectively.
}
\end{lem}




\begin{proof}

(Forwards/ downwards.)
If we have a solution $(f_1,\ldots,f_{n})$ of the original instance then it is 
also a solution of the new instance with the additional assignments $x_{j}^0 = 0$, $x_{j}^1 = 1$, $y_{j}^0 = f_{j}(x_{1},\ldots,x_{i},0,\ldots,0)$,
and 
$y_{j}^1 = f_{j}(x_{1},\ldots,x_{i},1,\ldots,1)$
in the definition of $\Phi_{i}^0\wedge \Phi_{i}^1$ for every $j> i$.
%To get $\Phi_{i}$ form the original instance 
%we just assign $x_{j} = 0$ for every $j>i$, 
%which is obviously weaker than the original instance.


(Backwards/ upwards.)
{\color{green!45!black}
First, introduce some notations. 
By $\vee$ denote $s_{2}$, 
by $\le$ denote the partial order such that 
$0<2$ and $1<2$ but $0$ and $1$ are
incomparable.
For an operation 
$f(x_1,\dots,x_s)$ 
by $f(x_1,\dots,x_t)$, where $t<s$ we denote 
$\bigvee\limits_{(a_{t+1},\dots,a_{s})}
f(x_1,\dots,x_t,a_{t+1},\dots,a_{s})$.


Let us show how to build a solution to the original instance from 
a solution of the new instance. 
Let a solution of the new instance be defined by 
$y_{i} = f_{i}(x_{1},\ldots,x_{n})$, 
$y_{i}^{0} = g_{j,i}^{0}(x_{1},\ldots,x_{n})$
and 
$y_{i}^{1} = g_{j,i}^{1}(x_{1},\ldots,x_{n})$
for 
the variables $y_{i}^{0}$ and $y_{i}^{1}$
from $\Phi_{j}^{0}\wedge \Phi_{j}^{1}$.

First, let us show that 
$$(x_1,\dots,x_{j}, c,\dots,c,
f_{1}(x_1,\dots,x_{j}),\dots,
f_{j}(x_1,\dots,x_{j}),
g_{j,j+1}^{c}(x_1,\dots,x_{j}),
\dots,
g_{j,n}^{c}(x_1,\dots,x_{j}))$$
is a solution of $\Phi$ 
for every $j\in[n]$ and $c\in\{0,1\}$.
In fact, from $\Phi_{j}^{c}$ 
the tuple 
$$(x_1,\dots,x_{j}, c,\dots,c,
f_{1}(x_1,\dots,x_{n}),\dots,
f_{j}(x_1,\dots,x_{n}),
g_{j,j+1}^{c}(x_1,\dots,x_{n}),
\dots,
g_{j,n}^{c}(x_1,\dots,x_{n}))$$
is a solution of $\Phi$. 
Consider all the evaluations of the variables 
$x_{j+1},\ldots,x_{n}$ to obtain $3^{n-j}$ solutions of $\Phi$, 
and apply the semilattice $s_2$ to them. 
As a result we obtain the required tuple, which implies that this 
tuple satisfies $\Phi$.

We prove by induction on $N=0,\dots,n$ that 
there exists operations $s_{1},\dots,s_{n}$

Second, consider the maximal $N$ 
such that there exist operations 
$s_{1},\dots,s_{n}$,
%$s_{N+1}^0,\dots,s_{n}^0$,
%$s_{N+1}^1,\dots,s_{n}^1$
satisfying 
\begin{enumerate}
    \item 
    $(x_1,\dots,x_{n},
s_{1}(x_1),s_{2}(x_1,x_2),\dots,
s_{N}(x_1,x_2,\dots,x_{N}),
s_{N+1}(x_1,x_2,\dots,x_{n}),
\dots,
s_{n}(x_1,x_2,\dots,x_{n}))$ is a solution of $\Phi$ for all 
$x_1,\dots,x_{N}$, and
%    \item 
%    $(x_1,\dots,x_{N}, 1,\dots,1,
%s_{1}(x_1),s_{2}(x_1,x_2),\dots,
%s_{N}(x_1,x_2,\dots,x_{N}),
%s_{N+1}^1(x_1,x_2,\dots,x_{n}),
%\dots,
%s_{n}^1(x_1,x_2,\dots,x_{n}))$ is a solution of $\Phi$ for all 
%$x_1,\dots,x_{N}$, and
\item 
$s_{i}(x_{1},\dots,x_{i})\ge f_{i}(x_{1},\dots,x_{i})$
for every $i\in[N]$.
\item 
$s_{i}(x_{1},\dots,x_{n})\ge f_{i}(x_{1},\dots,x_{n})$
for every $i\in\{N+1,\dots,n\}$.

\item 
$s_{i}(x_{1},\dots,x_{n})$ is uniquely determined 
by 
$x_1,\dots,x_{i}$ and $f_{i}(x_{1},\dots,x_{n})$
for every $i\in[n]$.
\end{enumerate}

Such $N$ exists because the above conditions 
hold 
for $N=0$ and $s_{i}(x_1,\dots,x_{n}) = f_{i}(x_1,\dots,x_{n})$ for every $i\in[n]$.
If $N = n$ 
then 
$(x_1,\dots,x_{n},s_{1}(x_1),s_{2}(x_1,x_{2}),\dots,
s_{n}(x_1,\dots,x_{n}))$ gives a solution to the original instance, 
which completes this case.

Assume that $N<n$.
Apply the 01-stable operation $h_{01}$ to 
the three solutions of $\Phi$
$$(x_1,\dots,x_{n},
s_{1}(x_1),s_{2}(x_1,x_2),\dots,
s_{N}(x_1,x_2,\dots,x_{N}),
s_{N+1}(x_1,x_2,\dots,x_{n}),
\dots,
s_{n}(x_1,x_2,\dots,x_{n}))$$
$$(x_1,\dots,x_{N+1}, 0,\dots,0,
f_{1}(x_1,\dots,x_{N+1}),\dots,
f_{N+1}(x_1,\dots,x_{N+1}),
g_{N+1,N+2}^{0}(x_1,\dots,x_{N+1}),
\dots,
g_{N+1,n}^{0}(x_1,\dots,x_{N+1}))$$
$$(x_1,\dots,x_{N+1}, 1,\dots,1,
f_{1}(x_1,\dots,x_{N+1}),\dots,
f_{N+1}(x_1,\dots,x_{N+1}),
g_{N+1,N+2}^{1}(x_1,\dots,x_{N+1}),
\dots,
g_{N+1,n}^{1}(x_1,\dots,x_{N+1}))$$

The first 
$n$ coordinates of the obtained tuple are
$(x_1,\dots,x_n)$.

Let us calculate the next $N$ coordinates.
For $i\in [N]$ put  
$$s_{i}'(x_1,\dots,x_{N+1}) = h_{0,1}(
s_{i}(x_1,\dots,x_{i}),
f_{i}(x_1,\dots,x_{N+1}),
f_{i}(x_1,\dots,x_{N+1})).$$
Let us show that 
$s_{i}'$
 depends only on 
$x_1,\dots,x_{i}$.
If 
$f_{i}(x_1,\dots,x_{i})=2$ then 
$s_{i}(x_1,\dots,x_{i})=2$ 
and 
$s_{i}'(x_1,\dots,x_{N+1})=2$.
If $f_{i}(x_1,\dots,x_{i})=d\neq 2$, then 
$f_{i}(x_1,\dots,x_{N+1})=d$ and 
$s_{i}'(x_1,\dots,x_{N+1}) = s_{i}(x_1,\dots,x_{i})$.
Additionally we can check that 
$s_{i}'(x_1,\dots,x_{N+1})\ge s_{i}(x_1,\dots,x_{i})\ge 
f_{i}(x_1,\dots,x_{i})$.


Let us calculate the $(n+N+1)$-th coordinate.
Put $$s_{N+1}'(x_1,\dots,x_{n}) = h_{0,1}(
s_{N+1}(x_1,\dots,x_{n}),
f_{N+1}(x_1,\dots,x_{N+1}),
f_{N+1}(x_1,\dots,x_{N+1})).$$
If 
$f_{N+1}(x_1,\dots,x_{N+1})=2$ then  
it returns 2, otherwise it is uniquely determined by $x_{1},\dots,x_{N+1}$, and 
$f_{N+1}(x_1,\dots,x_{n})= f_{N+1}(x_1,\dots,x_{N+1})$. 
That is, in all the cases $s_{N+1}'$ is uniquely determined by 
$x_1,\dots,x_{N+1}$.

For $i>{N+1}$ put $s_{i}'(x_1,\dots,x_{n}) = h_{0,1}(
s_{i}(x_1,\dots,x_{n}),
g_{N+1,i}^0(x_1,\dots,x_{N+1}),
g_{N+1,i}^0(x_1,\dots,x_{N+1}))$.
Since $s_{i}$ is uniquely determined 
by $x_1,\dots,x_{i}$ and $f_{i}(x_1,\dots,x_{n})$, 
the same is true for $s_{i}'$.
Thus we defined operations
$s_{1}',\dots,s_{n}'$ satisfying conditions (1) and (2), 
which contradicts the maximality of $N$.

}


Consider solutions of the new instance
such that 
$y_{i} = f_{i}(x_{1},\ldots,x_{n})$
for every $i$. \textcolor{red}{A solution for the new instance will also have Skolem functions for each of $y^0_i$ and $y^1_i$ making it of size $4n$ including the $x_i$. However we will repress the additional $2n$ terms in our tuple representation for reasons of space. For a certain such solution,} let $N$ be the minimal number such that 
$f_{N}$ depends on $x_{j}$ for some $j>N$. In fact, we would like that there is some solution such that this number does not exist as then this is also a solution of the old instance. But for now assume for contradiction that such an $N$ does exist and we choose it to be \textcolor{red}{maximal} among all the solutions.
{\color{blue}Since 
$(f_{1},\ldots,f_{n})$ gives us a solution of $\Phi_{N}^0$, 
the following tuple is a solution of $\Phi$
%\begin{align*}
$$(x_{1},\ldots,x_{N},0,\ldots,0,
f_{1}(x_{1},\ldots,x_{n}),\ldots,
f_{N}(x_{1},\ldots,x_{n}),f_{N+1}^0(x_{1},\ldots,x_{n}),
\ldots,f_{n}^0(x_{1},\ldots,x_{n}))$$
%(x_{1},\ldots,x_{N},1,\ldots,1&,
%f_{1}(x_{1},\ldots,x_{n}),\ldots,
%f_{N}(x_{1},\ldots,x_{n}),f_{N+1}^1(x_{1},\ldots,x_{n}),
%\ldots,f_{n}^1(x_{1},\ldots,x_{n}))
%\end{align*}
for every $x_{1},\ldots,x_{n}$ and some functions $f_{N+1}^0,\ldots, f_{n}^0$.
%\textcolor{red}{This solution to $\Phi$ has a canonical extension to an enlarged tuple which was the assumed solution to the whole quantifier-free part of the new instance, however we will not write this extra part of the enlarged tuple for reasons of space.} 
Note that we could see this tuple (with an additional term written and another omitted) rather as
$$(x_{1},\ldots,x_{N},0,\ldots,0,
f_{1}(x_{1}),\ldots,f_{N-1}(x_{1},\ldots,x_{N-1}),
f_{N}(x_{1},\ldots{n}),f_{N+1}^0(x_{1},\ldots,x_{n})
\ldots)$$
as we assume $f_i$ depends only on $x_1,\ldots,x_i$ for $i< N$.
Consider all the evaluations of the variables 
$x_{N+1},\ldots,x_{n}$ to obtain $3^{n-N}$ solutions of $\Phi$, 
then apply the semilattice operation to them to obtain
one solution $\alpha^0(x_{1},\ldots,x_{N})$ of the form
$$(x_{1},\ldots,x_{N},0,\ldots,0,
f_{1}(x_{1}),\ldots,
f_{N-1}(x_{1},\ldots,x_{N-1}),
e_{N}^0(x_{1},\ldots,x_{N}),
%g_{N+1}(x_{1},\ldots,x_{N}),
\ldots,e_{n}^0(x_{1},\ldots,x_{N})).$$
Note that $e_{N}^0(x_{1},\ldots,x_{N})$ is equal to $c$ if 
$f_{N}(x_{1},\ldots,x_{N},a_{N+1},\ldots,a_{n})=c$ for every $a_{N+1},\ldots,a_{n}$, 
and 
$e_{N}^0(x_{1},\ldots,x_{N})=2$ otherwise.
}

{\color{blue}
Doing the same with the solution of $\Phi_{N}^1$ we get 
a solution $\alpha^1(x_{1},\ldots,x_{N})$ of $\Phi$ of the form
$$(x_{1},\ldots,x_{N},1,\ldots,1,
f_{1}(x_{1}),\ldots,
f_{N-1}(x_{1},\ldots,x_{N-1}),
e_{N}^1(x_{1},\ldots,x_{N}),
%g_{N+1}(x_{1},\ldots,x_{N}),
\ldots,e_{n}^1(x_{1},\ldots,x_{N})).$$
Note that $e_{N}^0=e_{N}^1$.
}

%Let us build a solution of the new instance.
%Denote the quantifier free part of the new instance by $\Psi$.
%We need to find an assignment to all the $y$-variables 
%Put 
%$y_{i} = f_{i}(x_1,\dots,x_{n})$ for $i<n$, 
%$y_{i} = 
{\color{blue}
It remains to 
apply the 01-stable operation $g$ to
$(x_{1},\ldots,x_{n},f_{1}(x_{1},\ldots,x_{n}),\ldots,f_{n}(x_{1},\ldots,x_{n}))$, 
$\alpha^0(x_{1},\ldots,x_{N})$, and 
$\alpha^1(x_{1},\ldots,x_{N})$ 
to obtain a solution of the instance 
such that $f_{N}$ doesn't depend on $x_{N+1},\ldots,x_{n}$. \textcolor{red}{Recalling that we should have been applying always our polymorphisms to the $4n$-tuples involving Skolem functions for each of the $y^0_i$ and $y^1_i$, this gives also a new solution to the new instance,
%Also, applying $g$ to a solution of $\Phi_{j}^{c}$ and 
which gives us a contradiction to the maximality} of $N$ over all solutions.
}

Now let us define the evaluations $f'_1,\ldots,f'_n$ for the existential variables in the original instance by $f'_i(x_1,\ldots,x_i)=f_i(x_1,\ldots,x_i, x_{i+1},\ldots,x_n)$ where $x_{i+1},\ldots,x_n$ are chosen arbitrarily (as we proved $f$ does not depend on them).
%WE NEED TO DEFINE THE EVALUATIONS TO $y_{i}^{0}$ in each $\Phi_{i}$.

\end{proof}

The next lemma follows from Lemma~\ref{ReductionToQCSP2} and the fact 
that if $\Gamma$ is preserved by a semilattice then $\CSP(\Gamma)$ can be solved in polynomial time.
Nevertheless, to explain how a $01$-stable operation can be used 
in an algorithm we give an alternative proof.

\begin{lem}\label{InCONPForStable}
Suppose $\Gamma$ is preserved by $s_2$ and a 01-stable operation $g$.
Then 
$\QCSP(\Gamma)$ is in co-NP.
\end{lem}

\begin{proof}
Suppose we have an instance 
$\forall x_1\exists y_1 \forall x_2 \exists y_2 \dots \forall x_{n} \exists y_{n} \Phi$.
We can use an oracle to choose an appropriate value for $x_{1}$ (let this value be $a_{1}$).
Then we need to find an appropriate value for $y_{1}$, such that we can use an oracle for $x_2$ and continue.
We want to be sure that if the instance holds then it holds after fixing $y_{1}$. 

To find out how to fix $y_{1}$ we check the satisfability of the two instances 
%\exists y_1 \exists x_2 \exists y_2 \dots \exists x_{n} \exists y_{n} 
$$\Phi\wedge x_{1} = a_{1} \wedge x_{2} = x_{3}=\dots=x_{n} = 0,$$
%\exists y_1 \exists x_2 \exists y_2 \dots \exists x_{n} \exists y_{n} 
$$\Phi\wedge x_{1} = a_{1} \wedge x_{2} = x_{3}=\dots=x_{n} = 1.$$
These are CSP instances, which can be solved in polynomial time 
because the semilattice preserves $\Gamma$.
We check whether both have a solution with $y_{1}=0$, $y_{1} =1$, $y_{1}=2$ (we solve six instances).
Let $Y$ be the set of possible values for $y_{1}$ such that both instances have solutions.
If $Y$ is empty, then the QCSP instance does not hold and we are done.
If $|Y|=1$, then we fix $y_{1}$ with the only value in $Y$. Obviously, 
the fixing of $y_{1}$ cannot transform  
the QCSP instance that holds into an instance that does not hold.
If $|Y|>1$ then $2\in Y$ due to the semilattice polymorphism. 
Let the solutions of the CSP instances with $y_{1} = 2$ be 
$(x_{1},y_{1},x_{2},y_{2},\dots,x_{n},y_{n}) = 
(a_{1},2, 0, c_{2},\dots,0, c_{n})$
and $(x_{1},y_{1},x_{2},y_{2},\dots,x_{n},y_{n}) = 
(a_{1},2, 1, d_{2},\dots,1, d_{n})$.
Assume that the QCSP instance has a solution 
$(a_{1},f_{1} (a_{1}), x_{2},f_{2}(x_{1},x_{2}), \ldots,x_{n},f_{n}(
x_{1},\ldots,x_n))$.
Then by applying the operation $g$ to this solution,
$(a_{1},2, 0, c_{2},\dots,0, c_{n})$, and 
$(a_{1},2, 1, d_{2},\dots,1, d_{n})$,
we get a (partial) solution of the $\QCSP(\Gamma)$
with $y_{1}=2$.

We proceed this way through the quantifier prefix, using an oracle to choose values for  $x_{2}, \ldots,x_{n}$,
while we solve CSP instances to 
choose appropriate values for 
$y_{2},y_{3},\ldots,y_{n}$.
\end{proof}


We say that a ternary relation $R$ is \emph{an AND-type} relation if 
$R\cap (\{0,1\}\times\{0,1\}\times\{0,1,2\})
=\begin{pmatrix}
0&0&1&1\\
0&1&0&1\\
0&0&0&1
\end{pmatrix}$, that is, it is row-wise the truth table of AND.
If $s_2$ preserves $R$, 
then it also contains $(2,2,0)$ and $(2,2,2)$.
We say that a ternary relation $R$ is \emph{an OR-type} relation if 
$R\cap (\{0,1\}\times\{0,1\}\times\{0,1,2\})
=\begin{pmatrix}
0&0&1&1\\
0&1&0&1\\
0&1&1&1
\end{pmatrix}$, that is, it is row-wise the truth table of OR.
Again, if $s_2$ preserves $R$, 
then it also contains $(2,2,1)$ and $(2,2,2)$. One can readily imagine AND/OR-type relations of arity $k+1$ higher than three built from AND/OR operations of arity $k$. 

\begin{lem}\label{ANDORHardness}
Suppose $\Gamma$ contains an AND-type relation and an OR-type relation,
and $\Gamma$ is preserved by $s_2$.
Then $\QCSP(\Gamma)$ is co-NP-hard.
\end{lem}
\begin{proof}

By $R_{and,2}$ and 
$R_{or,2}$ we 
denote an AND-type and an OR-type relation, respectively.
For $n=2,3,4,\dots$ put 
$$R_{and,n+1}(x_{1},\ldots,x_{n},x_{n+1},y) = 
\exists z \;R_{and,n}(x_{1},\ldots,x_{n},z)
\wedge R_{and,2}(x_{n+1},z,y),$$
$$R_{or,n+1}(x_{1},\ldots,x_{n},x_{n+1},y) = 
\exists z \; R_{or,n}(x_{1},\ldots,x_{n},z)
\wedge R_{or,2}(x_{n+1},z,y).$$

Let us define a relation $\xi_{n}$ for every $n$ by
\begin{align*}
\xi_{n}(x_{1},y_{1},z_{1},\dots,
x_{n},y_{n},z_{n})&=
\exists u\exists u_{1}\dots\exists u_{n}
\exists v\exists v_{1}\dots\exists v_{n}\;
R_{and,2}(u,v,v) \wedge \\
R_{and,3}(x_{1},y_{1},z_{1},u_{1})&\wedge
\dots\wedge
R_{and,3}(x_{n},y_{n},z_{n},u_{n})\wedge
R_{or,n}(u_1,\dots,u_{n},u)\wedge\\
R_{or,3}(x_{1},y_{1},z_{1},v_{1})&\wedge
\dots\wedge
R_{or,3}(x_{n},y_{n},z_{n},v_{n})\wedge
R_{and,n}(v_1,\dots,v_{n},v).
\end{align*}

It follows from the definition 
that 
$\xi_{n}\cap \{0,1\}^{3n}$ is defined by
$\mathrm{AE}_3(x_{1},y_{1},z_{1})\vee
\mathrm{AE}_3(x_{2},y_{2},z_{2})\vee
\dots
\vee
\mathrm{AE}_3(x_{n},y_{n},z_{n})$,
where 
$\mathrm{AE}_3 = \{(0,0,0),(1,1,1)\}$.

Suppose 
$R(y_1,\dots,y_{t}) = 
\xi_{n}(y_{i_1},y_{i_{2}},\dots,y_{i_{3n}})$, 
where 
$i_{1},\dots,i_{3n}\in\{1,2,\dots,t\}$.
Let us show that 
$\forall y_{1}\dots\forall y_{t}\;
\xi_{n}(y_{i_1},y_{i_{2}},\dots,y_{i_3n})$
holds if 
$\xi_{n}(y_{i_1},y_{i_{2}},\dots,y_{i_3n})$
holds for all $y_{1},\ldots,y_{t}\in\{0,1\}$.
%Suppose $\xi_{n}(y_{i_1},y_{i_{2}},\dots,y_{i_3n})$
%defines a relation $R$.
We need to prove that if $\{0,1\}^{t}\subseteq R$ then 
$A^{t}\subseteq R$, which follows from the fact that the semilattice $s_2$ preserves $R$.

Now we may encode the complement of \emph{Not-All-Equal 3-Satisfiability} using $\Gamma$.
This complement can be expressed by
a formula of the following form:
$$\forall y_{1}\dots\forall y_{t} \ 
\mathrm{AE}_3(y_{i_1},y_{i_{2}},y_{i_3})\vee
\dots
\vee
\mathrm{AE}_3(y_{i_{3n-2}},y_{i_{3n-1}},y_{i_{3n}}),$$
which is equivalent to 
$$\forall y_{1}\dots\forall y_{t}\;
\xi_{n}(y_{i_1},y_{i_{2}},\dots,y_{i_{3n}}).$$
Thus, we reduced a co-NP-complete problem to $\QCSP(\Gamma)$, which completes the proof.
\end{proof}


\begin{lem}\label{NoStrange2Hardness}
Suppose $\Gamma\subseteq\Inv(s_2)$, 
$\Gamma$
contains 
$\delta(x,y,z) = (x\neq 0)\vee (y=z)$ 
and an AND-type relation $R_{2}$. 
Then $\QCSP(\Gamma)$ is co-NP-hard.
\end{lem}
\begin{proof}
Here we will define a reduction from the complement of 
$\CSP(\{1\mathrm{IN}3\})$, which is known  to be NP-complete \cite{Schaefer},
where 
$1\mathrm{IN}3 = \begin{pmatrix}
1&0&0\\
0&1&0\\
0&0&1
\end{pmatrix}$.
First, 
put 
$$\delta_1(x_1,x_2,x_3,x_4) = \exists t\;\delta(x_1,x_{3},t) \wedge \delta(x_{2},t,x_4).$$
It is not hard to see that 
$\delta_1(x_1,x_2,x_3,x_{4}) = 
(x_{1}\neq 0)\vee 
(x_{2}\neq 0)\vee
(x_{3}=x_{4}).$
Put 
$$\delta_{2}(x_{1},x_{2},x_{3},x_{4}) = 
\delta_{1}(x_{1},x_{2},x_{3},x_{4})
\wedge 
\delta_{1}(x_{1},x_{3},x_{2},x_{4})
\wedge 
\delta_{1}(x_{2},x_{3},x_{1},x_{4}).
$$
By the definition, the first three variables of
$\delta_{2}$ are symmetric.
Suppose $(a,b,c,d)\in\delta_{2}$. 
It is not hard to see that
$a=b=c=0$ implies $d=0$.
Also 
$a=1, b=c=0$ implies $d=1$.
If there are at least two 1s in $(a,b,c)$ then 
$d$ can be arbitrary.
Put $R'(x,y) = R_{2}(x,x,y)$.
By the definition of an AND-type relation, 
$R'$ contains $(0,0),(1,1),(2,2),(2,0)$
but doesn't contain $(0,1),(0,2),(1,0),(1,2)$.
Put
$$\delta_{3}(x_{1},x_{2},x_{3},x_{4}) = 
\exists x_{1}'\exists x_{2}'\exists x_{3}'\;
\delta_{2}(x_{1}',x_{2}',x_{3}',x_{4})
\wedge 
R'(x_{1},x_1')
\wedge 
R'(x_{2},x_2')
\wedge 
R'(x_{3},x_3').$$
Then 
$(a,b,c,0)\in\delta_{3}$
for all tuples $(a,b,c)$ but the tuples from $1\mathrm{IN}3$.

%Let $R_2$ be the AND-type relation.
Again, we apply the recursive 
formula to build an $n$-ary ``and''
$$R_{n+1}(x_{1},\ldots,x_{n+1},z) = 
\exists t\; R_{n}(x_{1},\ldots,x_{n},t)\wedge
R_{2}(t,x_{n+1},z).$$


Define 
$\zeta_{n}(x_{1},\ldots,x_{3n})$ by
$$\exists z_{1}\dots\exists z_{n}\exists t\;
R_{n}(z_{1},\ldots,z_{n},t)
\wedge 
\delta_{3}(x_{1},x_{2},x_{3},z_{1})\wedge
\dots\wedge \delta_{3}(x_{3n-2},x_{3n-1},x_{3n},z_{n})
\wedge (t=0).
$$

Now we may encode the complement of $\CSP(\{1\mathrm{IN}3\})$ using $\Gamma$. If $\overline{1\mathrm{IN}3}$ is the complement of $1\mathrm{IN}3$ with respect to $\{0,1\}^3$, then we use
a formula of the following form:
$$\forall y_{1}\dots\forall y_{t} \ 
\overline
{1\mathrm{IN}3}(y_{i_1},y_{i_{2}},y_{i_3})\vee
\dots
\vee
\overline{1\mathrm{IN}3}(y_{i_{3n-2}},y_{i_{3n-1}},y_{i_{3n}}),$$
which is equivalent to 
$$\forall y_{1}\dots\forall y_{t}\;
\xi_{n}(y_{i_1},y_{i_{2}},\dots,y_{i_{3n}}).$$
Thus, we reduced a co-NP-complete problem to $\QCSP(\Gamma)$, which completes the proof.
\end{proof}


\begin{lem}
Suppose 
$$\begin{array}{c}
\sigma_0 = \{ (a_1,a_2,a_3) : a_1 \in A, a_2,a_3 \in \{1,2\}, (a_1 \in \{0,2\} \vee a_2=a_3) \},\\
\sigma_1 = \{ (a_1,a_2,a_3) : a_1 \in A, a_2,a_3 \in \{0,2\}, (a_1 \in \{1,2\} \vee a_2=a_3) \}. 
\end{array}$$
Then $\QCSP(\{\sigma, \sigma_0,\sigma_2,\{0\},\{1\}\})$ 
is coNP-hard.
\label{lem:coNP-hardness-oldPSpace}
\end{lem}

\begin{proof}
Let us encode the complement of \emph{Not-All-Equal 3-Satisfiability} using $\{\sigma, \sigma_0,\sigma_2,\{0\},\{1\}\}$.
An instance $\mathcal I$ of this complement can be expressed by
a formula of the following form:
$$\forall x_{1}\dots\forall x_{t} \ 
\mathrm{AE}_3(x_{a_1},x_{b_{1}},x_{c_1})\vee
\dots
\vee
\mathrm{AE}_3(x_{a_s},x_{b_s},x_{c_s}),$$
where $\mathrm{AE}_3 = \{(0,0,0),(1,1,1)\}$.
{\color{red}
Let
\begin{align*}
    \Phi_0= & \bigwedge_{1 \le i \le s} (\sigma_0(x_{a_i},y_{i-1},y_i)\wedge
    \sigma_1(x_{b_i},y_{i-1},y_i) \wedge \sigma_0(x_{c_i},y_{i-1},y_i))\\
    \Phi_1= & \bigwedge_{1 \le i \le s} (\sigma_1(x_{a_i},z_{i-1},z_i)\wedge
    \sigma_1(x_{b_i},z_{i-1},z_i) \wedge \sigma_1(x_{c_i},z_{i-1},z_i))\\
\Psi =& \forall x_{1}\dots\forall x_{t}\;
\exists y_{0}\exists y_1\dots\exists y_{s}\;
\exists z_{0}\exists y_1\dots\exists z_{s}\;
(y_{0} = 1\wedge \Phi_{0}\wedge z_{0} = 0\wedge \Phi_1 \wedge \sigma(y_{s},z_{s})).
\end{align*}
Let us show that $\mathcal I$ is equivalent to $\Psi$.

($I\in \mathrm{co\mbox{-}NAE3SAT}$ implies $\Psi \in \QCSP(\{\sigma,\sigma_0,\sigma_1\})$.) Suppose in $\Psi$ Universal plays some sequence of $0$s and $1$s for the $x_i$s. Let this be duplicated by Universal in $I$ and we may assume that the resulting instance of $\mathrm{QNAE3SAT}$ has a clause $j$ that is falsified. Without loss of generality, let us assume it is falsified by $(x_{a_j},x_{b_j},x_{c_j})=(1,1,1)$, since the other case is dual (and may be inferred from the proof of the reverse implication below). Existential plays in $\Psi$ as follows. $y_0,\ldots,y_{j-1},y_j,\ldots,y_s$ are set to $1$. $z_0,\ldots,z_{j-1}$ are set to $0$ and $z_j,\ldots,z_s$ are set to $2$. Let us look at the interesting conjunction in $\Phi_1$, which is $\sigma_1(x_{a_j},z_{j-1},z_j)\wedge
    \sigma_1(x_{b_j},z_{j-1},z_j) \wedge \sigma_1(x_{c_j},z_{j-1},z_j)$, and note that this is satisfied trivially as $(x_{a_j},x_{b_j},x_{c_j})=(1,1,1)$. The fact that the other parts are satisfied is straightforward since $y_{i}=y_{i-1}$ and $z_{i}=z_{i-1}$.

($\Psi \in \QCSP(\{\sigma,\sigma_0,\sigma_1\})$ implies $I\in \mathrm{co\mbox{-}NAE3SAT}$.) We cannot have $y_0,\ldots,y_s=1$ and $z_0,\ldots,z_s=0$ because we violate $\sigma(y_s,z_s)$. Thus, at least at some point in one of these sequences, we make a transition to $2$. Let us assume, without loss of generality, since the other case is dual (and may be inferred from the proof of the reverse implication above), that it is in the $y_i$ at the point $y_{j-1}=1$ and $y_j=2$. Then the conjunction $\sigma_0(x_{a_j},y_{j-1},y_j)\wedge
    \sigma_0(x_{b_j},y_{j-1},y_j) \wedge \sigma_0(x_{c_j},y_{j-1},y_j)$ enforces that $(x_{a_j},x_{b_j},x_{c_j})=(0,0,0)$.

Thus, we reduced a co-NP-complete problem to $\QCSP(\{\sigma, \sigma_0,\sigma_2,\{0\},\{1\}\})$, which completes the proof.
}
\end{proof}

==> old/reviews.tex <==
Review #10A
===========================================================================

Paper summary
-------------
For a fixed finite relational language $\Gamma$ on a domain $D$, the Quantified Constraint Satisfaction Problem QCSP($\Gamma$) is to decide whether a given sentence $\forall x_1 \exists y_1 \dots \forall x_n \exists y_n\ \Phi$ holds, where $\Phi$ is a conjunction of relations from $\Gamma$. Hence QCSP is a generalization of the Constraint Satisfaction Problem CSP by allowing universal quantification of variables and a generalization of Quantified SAT (or QBF) by allowing  arbitrary constraints on not necessarily Boolean domains.

Prior to this paper only $\Gamma$ with QCSP($\Gamma$) in P, NP-complete or PSPACE-complete were observed. Chen's Conjecture, which has been around for about 10 years, is that these are indeed the only cases that occur for $\Gamma$ containing all constants. The authors verify it under the stronger assumption that $\Gamma$ contains all unary relations (Theorem 4). However, for $\Gamma$ containing all constants on a 3-element set they show that complexity of QCSP($\Gamma$) is either P, NP-complete, coNP-complete or PSPACE-complete (Theorem 3). Additionally on a domain of size 4 they exhibit some $\Gamma$ with DP-complete QCSP (Corollary 8). On a 10-element set they construct $\Gamma$ with $\Theta_2^p$-complete QCSP (Corollary 10).

These are major result with quite ingenious proofs which certainly need to be published. The paper breaks new ground on the complexity description of QCSP and should be of interest for anyone in complexity theory and general algebra. The only thing that could be improved is the presentation. Proofs are quite technical and could maybe be better motivated. Some suggestions on the presentation are below. I strongly recommend acceptance subject to minor revisions.

Comments for authors
--------------------
\begin{enumerate}
\item
 page 1, line -3 of abstract: clone of such $\Gamma$

Yes.
BM: Done.
DZ: the reviewer said about line -3 and you corrected line -2. BM: Oh, you are right... I will fix it.

\item  page 4, line -7 of Section 1.1: When noting $s=s_c$ make reference to Section 7.1 for the definition of $s_c$.
 
Yes.
BM: Done.

\item
 page 5, line 2 of Section 2: on a $3$-element domain (Careful with articles throughout!) 
 
Yes. Although I got used to the Russian English!
BM: Done.

 \item  page 5, title of Section 2.1: on $3$-element domains 
 
Yes.
BM: Done.
DZ: I don't see the correction. 
BM: Ah you are right, I added it.

 \item
  page 5, line 1 of Section 2.1: Specify $a,c$, e.g: For $a,c\in\{0,1,2\}$ define the following operations
  on $\{0,1,2\}$.

Yes.
BM: Done.

\item
  page 7: on A 3-element domain (5x)

Yes.
BM: Done.
DZ: I added few more articles like this.

\item
 page 11, line 7: Gaifman

Yes.
BM: Done.

\item
 page 12, title of Section 6: the 3-element domain 
 
Yes (though this is not really necessary). 
BM: I did it.

 \item  page 12, line -4: the domain $\{0,1,2\}$ 
 
Yes.
BM: Done.

 \item  page 13, line -4-(-1) above Lemma 17: Definitions of the relations are ambiguous to parse. E.g. is $\sigma_1$ just
 $\{1,2\}\times\{0,2\}^2 \cup \{ (0,0,0),(0,2,2) \}$? Better rephrase. 

Yes (add brackets).
BM: Done.
DZ: I tried two variants (below) and I think our original is better. 
\sigma_0 = (A\times \{1,2\}\times\{1,2\})\setminus \{(1,1,2),(1,2,1)\} \\
\sigma_0 = \{0,2\}\times \{1,2\}\times\{1,2\}\cup \{(1,1,1),(1,2,2)\} \\
BM: Right but with the brackets we now have I don't think there is a problem.

\item
 page 13, paragraph -3: What do you mean by `k and l \dots the minimal and maximal indices appearing in $y$ variables  of $\Phi$'? Is not $k=0, l = 2s$ from the definition of $\Phi$ in the previous paragraph? How should $k\leq 0$?

The reviewer doesn't follow that k decreases and l increases in the construction. We should make this explicit.
BM: Done.

\item
 page 13, line -9: From the definition of $\Phi$ $y_1,\dots,y_{2k-1}$ are already existentially quantified.
 How do you set $\exists y_k$ etc again?

This follows from previous misunderstanding.

\item
 page 16, Lemma 19: co-NP

Yes.
BM: Done.

\item  
 page 18, line 5 of Section 7: $\tau_n$ is the   

Yes.
BM: Done.

\item
 page 19, Lemma 22: In line 1 $\Phi$ is $n$-ary, in line 3 $n+1$-ary. What are $R$ and $R'$ really?
 
*** Dima ***
Yes, we need to emphasise y is bound in R but free in R'. We say Phi is conjunctive but surely y is existentially quantified in R?
*** Dima ***
Here I got confused... Is Phi quantifier free?

DZ: Phi is quantifier free conjunctive formula, and we gave a definition in preliminaries saying that $\Phi(z_{1},\dots,z_{n})$ is the projection of the solution set of $\Phi$ onto $z_{1},\dots,z_{n}$. 
I suggest recalling the definition here.
BM: Right, so there is an implicit existential quantification on the y. We should definitely recall the definition.

\item
  page 20, line 1: Display the definition of $h_{0,2}$ to make it easier to read.

We could try but it will take more space.
BM: Done.

\item
 page 21, line 1 of Lemma 25: $(m+1)\times n$-matrix 

Yes.
BM: Done.

 \item  page 28, line 1 of Lemma 41: minimal arity $N$ 
 
Yes.
BM: Done.

\item  page 32, title of Section 9.2: Boolean 

Fine.
BM: Done. Hm... Dima: can we always use operation instead of function? Maybe it doesn't matter.

DZ: in my head they are synonyms, so I don't really care. Nevertheless, I suggest using the word function in section 9.2 to emphasize that these are operations generated from relations, so they are different, on 2-element domain and not related to operations on 3-element domain. In all other places I suggest using the word operation. But I don't insist. What do you think?
BM: Sounds fine.

\item  page 32, Lemma 46: Note that this holds for arbitrary $\Gamma$ containing $0,1$.

*** Dima ***
Yes, I suppose it is true Dima?
BM: Done.

DZ: I returned everything back. Gamma in section 9 cannot be used for any constraint language.
But yes, it is true that any constraint language containing the equality relation and constants 0 and 1.
I added note. Please check.
I also worry again about the equality relation. 
The only place we mention that we always have it is preliminaries. 
And here we actually use this in a claim. Probably we should write this precisely.
BM: I think the equality thing is not a problem. I will remove the indent.

\item
 page 33, line -1 above Lemma 48: operation 
 
Yes.
BM: Done.

 \item
  page 33, line 2 in the proof of Lemma 49: $v_0$ is a $\{0,2\}\{1,2\}$-projection

Yes.
BM: Done.

  \item
  page 34, line -2: Why is $f(0,2)=2$?

Well, it \alpha\beta projects to second coordinate so must return 2 here. Actually, it was noted we didn't define \alpha\beta projects to a coordinate, so we will put this earlier explicitly.

DZ: I added a comment, please check.
BM: It is fine.

\item
 page 36, line 3 of Lemma 56: Then the relation ...

It is fine as it is, actually.

\item
 page 36, line 7 of proof of Lemma 58: (the 1-stable case ...) 
Yes.
BM: Done.

 \item
  page 38, line 2 of proof of Lemma 59: ..., then 
  
Yes.
BM: Done.

DZ: you added a comment and I corrected what they wanted.

 \item  page 39, line -2 of Acknowledgments: for fruitful 
 
Yes.
BM: Done.

\item  page 40, references [3] and [17]: QCSP and CSPs 

Yes.
DZ: Done

\item  page 41, references [27]: Don't capitalize title to be consistent with the other references.

Yes.
DZ: You did this already!
BM: Ah yes, I did it in passing and then forgot about it!
\end{enumerate}


* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #10B
===========================================================================

Paper summary
-------------
QCSP Monsters and the Demise of the Chen Conjecture
---------------------------------------------------

The Feder-Vardi dichotomy conjecture is a famous and influential statement on the complexity of CSPs over different constraint languages.
Namely: it states that *no* CSP problem is NP-Intermediate; it is either in P or NP-Complete.
After many years of work, the dichotomy conjecture was recently resolved independently in two celebrated papers --- one by Bulatov and one by Zhuk.

With that being said, there are still many classification questions about variants of CSPs that remain open.
This paper considers one such fundamental class: the *quantified* CSPs.
Quantified CSPs are simply the CSP generalizations of TQBF, and so they clearly can have complexity ranging all the way up to PSPACE.
Indeed, there is even an analogous "dichotomy" conjecture for QCSPs, on which there has been significantly less progress:

Chen Conjecture. If L is a finite constraint language then L is either in NP or is PSPACE-Complete.

The present paper presents a family of results which refute (!) this widely-known conjecture:

(1) The paper gives several examples of QCSP languages with *widely varying* complexities between PSPACE and NP: from their techniques, one can show the existence of CSPs with complexity in coNP, and even stranger classes (e.g. DP, which is the class of languages L of the form L1 intersect L2, where L1 is in NP and L2 is in coNP, and Theta_2^P, corresponding to P^NP where you only allow O(log n) calls to the oracle).
Accompanying these examples is a general toolbox to produce QCSP languages of varying complexities.
(For instance, one can easily generalize their techniques to obtain a language at *any* level of the Boolean hierarchy; albeit, the size of the domain will increase with the levels of the hierarchy).

*** Dima ***
>> Well, we're not sure we can reach all levels of the Boolean Hierarchy. Should perhaps discuss in conclusion.

DZ: I am pretty sure it is not possible using the presented technique. I also believe it is not possible at all because conjunction is always given to us for free. 
BM: Should we mention this in the conclusion? Maybe it should be for the journal version of sequel.

(2) A complete complexity classification of the conservative QCSP (i.e. QCSPs with all unit constraints) that agrees with the Chen Conjecture.

(3) A complete complexity classification of the QCSP on domains with three elements, provided constants are allowed --- in particular, they seperate the complexity into P, NP-Complete, co-NP-Complete, and PSPACE-Complete.

Thus, the authors show that unlike the standard CSP problem, the complexity of the QCSP problem is much more sensitive to the underlying domain size.
Furthermore, they resoundly *shatter* any hopes of getting a "simple" complexity classification of all QCSP problems into a small number of classes.
Furthermore, they show that even the prior algebraic conditions which were at least partially believed to classify the complexity of QCSP (the polynomial and exponential generated powers properties) strongly do *not* separate such CSPs in general, although they do in the conservative case.
Thus, the paper gives shows an amazing richness of the family of QCSPs, and suggests a re-evaluation of the work in this area.

All in all, I found this paper to be fascinating. Anyone interested in the complexity of CSPs is bound to find it interesting. 
I have verified the proofs of (1) and (2), as well as the proof of the existence of a QCSP language that is coNP-complete; however, I did not fully verify the proof of the 3-element classification as it is extremely technical.
Modulo this, I believe that this paper is a perfect fit for STOC.

Comments for authors
--------------------
Comments for Authors
--------------------

I only have one major comment for the authors. 
I believe it would be very helpful for the readers if you extracted from your argument a standalone proof of a constraint-language G such that QCSP(G) is coNP-Hard.
It could be of independent interest beyond the CSP community, and currently the proof is embedded in some small lemma (with no fanfare) in your general 3-element characterization.
This is especially true as your construction is relatively simple and understandable, and so it also serves as a good warm-up to convince the reader that such alternative complexities are obtainable (especially since all the other wild complexities you generate rely on having a coNP-Complete QCSP).

*** Dima ***
>> Could be a good idea for long and journal version, what do you think, Dima?

DZ: I totally agree, it is a good idea! Probably even for the STOC version.

* * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * * *


Review #10C
===========================================================================

Paper summary
-------------
QCSP (Quantified Constraint Satisfaction Problem) over a finite set of relations Gamma on a finite domain D (a.k.a. constraint language) is the computational problem of deciding whether a given first-order sentence, whose quantifier-free part uses only conjunction and atomic formulae over Gamma, is true. The paper studies how the computational complexity of QCSPs depends on the fixed constraint language. This version of the QCSP is a member of a larger class of problems when one fixes a finite constraint language together with allowed connectives and quantifiers (e.g., for QCSP both quantifiers are allowed and the only allowed connective is the conjunction). In fact, after the celebrated resolution of the dichotomy conjecture for CSPs (where we allow only universal quantification and conjunction) by Bulatov (FOCS'17) and Zhuk (FOCS'17), the QCSP is the last member of this class for which a complexity classification is open. The paper's main results are the following.

- a full complexity classification of the complexity for constraint languages on a three-element set which contain the singleton unary relations (namely, 4 nontrivial complexity classes modulo P-time reductions occur: P, NP-complete, coNP-complete, PSpace-complete)
- a full complexity classification of the complexity for constraint languages which contain all unary relations
- a theorem that enables us to combine constraint languages to get more exotic complexities; in particular, the authors construct two constraint languages whose QCSP is DP-complete and \Phi^P_2-complete

Another interesting result is obtained as a byproduct: there is an (explicitly given) constraint language Gamma and a family of relations that are primitively-positively (pp-) definable from Gamma, but every pp-definition uses exponentially many quantifiers.


The results are excellent and interesting for several reasons.

- In CSP and all the other variants but QCSP, only the expected complexity classes show up (eg. P and NP-complete in CSP). The expected complexity classes for QCSP were P, NP-complete, and PSpace-complete. The presented result, that coNP-complete QCSPs exist even on a 3-element domain and even more complexity classes are present on larger domains, are very surprising. 
- The classification results (3-element QCSPs with singletons, conservative QCSPs) form a major step toward the full classification. Note that similar special cases for CSPs were indeed among the most important results before the full classification. 
- The proofs contain novel algorithmic and mathematical techniques (eg. dealing with universal quantifiers without the PGP property, new information about clones on a 3-element set, lower bounds on the size of pp-definitions)
- The results encourage further investigation: What other complexities show up? Can one formulate elegant criterions for membership in some complexity class or hardness?



The paper is well organized, the background is well explained, and the contributions clearly stated. However, significant improvements can be made in the technical parts (mostly proofs, also some statements and explanatory text) and I suggest to give the paper a thorough revision before the publication in the proceedings. 


In summary, the contribution is excellent and interesting for people in computational complexity and surrounding areas. 
I strongly support the acceptance of the paper.

Comments for authors
--------------------
- There are numerous language issues that can be easily corrected when thoroughly read by a native speaker, such as the second author. Here are some of them (not a comprehensive list):

  -- p13, l3, "we assume every instance of QCSP....". It is not a nice formulation and also, stricly speaking, not true: there are instances of QCSP constructed later on (e.g. right after, in Lemma 17) which are not be of this form. Question: shouldn't the players Existential and Universal be always capitalized?
  
Will discuss prenex form earlier. Universal and Existential should always be capitalised when naming players.
BM: Done.

  -- The words "correspondingly" and "respectively" are sometimes used incorrectly, I believe (see the statement of Lemma 18, page 31 last paragraph). Also "for example" and "in particular" (2nd line of proof of Lemma 41)
  
I will change some correspondingly to respectively. The latter criticism is not so fair.
BM: Done.

  -- "This complement is a formula..." on page 17 does not make sense
  
Will rephrase.
BM: Done.

  -- The remark between Lemma 22 and its proof is not well formulated. (The proof of this Lemma can be improved as well.)

*** Dima ***
Actually, this remark is not so helpful in its current position. It should appear after the proof if anywhere, but I wonder if it can't just be removed.
BM: I hid it.
DZ: Agree. We don't need this remark since it is 
essentially about Lemma 23. We need to go through the proof again to make it better.
BM: Well, this remark came back. But I am reconciled with it.

  -- page 20, "In fact, for the first two elements of the left part...": It is not clear what is meant

Right, this needs to be rephrased. It is the first two coordinates of the \betas.
BM: Done.

  -- The description of the clone C above Lemma 25 does not read nicely.
  
I will make a small adjustment.
DZ: Please do.
  
  -- page 24, "we assume that ... is not defined": it is not an assumption, rather a definition
  
Yes.
BM: Done.

  -- "and" is missing in the statement of Lemma 25, definition of minimal 1-set, Lemma 34

Yes.
BM: Done.

  -- proofs of eg. Lemma 41, Theorem 50 contain formulations like "row whose elements are equal" to mean a constant row

Yes, but this is fine.

  -- the first paragraph of Lemma 43 is not well formulated
  
Yes.

  -- proof of Theorem 50: formulation "(see the proof of Lemma 41 for the detailed explanation)" is not nice, since Lemma 41 proves something else; formulation "By Lemma 49, we consider two cases:" is not nice either.
  
*** Dima ***
Yes. Yes: the "By Lemma 49..." is not wholly accurate.   

DZ: I corrected this, but we will need to go through the proofs again while preparing the full version.
BM: Yes.

  -- there are several strange formulations in the proof of Lemma 52

I thought this was alright.
  
  -- line 2-3 on page 37, the formulation "It remains to check that.... It follows from the fact...." is not nice
  
We should flesh these out in the journal version.

DZ: to be honest I don't see a problem =)

  -- Quite often no distinction is made between relation and clause/conjunct/constraint/atomic formula. This can be confusing. E.g. lines 4-5 in the introduction or the proof of Lemma 14

I will fix this.
BM: Done.

- Suggestion to improve the organization of the paper:

  -- I suggest to add some more detailed discussion about the cases in Theorem 6. In particular, specify what "otherwise" is in the co-NP-complete case. Also, some discussion about \alpha\beta-projectivity and relation to the cases would be helpful here (see also the next comment).

*** Dima ***
Hm... Dima, isn't this non-trivial? We left this for the otherwise because it occurs once the cases are exhausted.
BM: \alpha\beta-projectivity is now discussed in more detail in prelims. Dima: you should read the new prelims.

DZ: We could notice after the statement that otherwise means EGP+WNU+\alpha\beta-projective with $\alpha\cap\beta\neq\varnothing$ and omitting cases 5 and 6. But I wouldn't put it into the statement.

  -- I suggest to add somewhere earlier some discussion about \alpha\beta-projectivity because the reader needs to wait until Section 9.3 and Section 10 when the role of projectivity becomes somewhat clearer. E.g., Corrollary 55 implicitely uses that \rho is pp-definable.
  
Yes, will do this.
BM: Done.

  -- The discussion about a solution of a QCSP instance and the game theoretic viewpoint should come earlier, preferably before Section 4 but certainly before Section 5, where it is implicitely used. 
  
Yes.
BM: Done.

  -- Lemma 46 was already proved (in a particular case) in Lemma 20. I suggest to move the initial part of this subsection to come before Lemma 20

*** Dima ***
This I don't follow.
DZ: there should be a mistake. It is stupid to move parts of Section 9.2 earlier. Let's ignore this.
BM: Ok.

- The text is sometimes very formal, some informal explanations and/or less symbol-heavy definitions would help. Also, too much work is left for the reader (especially given the lack of informal explanations). Here are several more concrete remarks (again, not a comprehensive list). 

  -- In Lemma 14, 
    --- the reader will likely start to understand the role of the relations \sigma_? only after reading a big portion of the whole proof. Without any preliminary understanding, even the easier reduction is hard to read
	
We can add something here.

    --- the sentence J is sloppily defined. 
	
Yes.

    --- what is "disjoint union" of reductions? (page 11, 3rd line)

This "disjoint union" is even wrong, rather it is a conjunction. This is my mistake.
BM: Done.

    --- 2nd paragraph on page 11 is not nicely phrased.
	
Not sure about this.
DZ: It seems fine to me.
BM: Yes, I thought it was fine.

    --- 3rd paragraph is not well phrased either, in "...either takes on values in ..., or ..., or A" the last option is always true, something else was meant. Also what "fixed element constant appears in a position where it is forbidden" should mean?
	
I will improve the readability here, the reviewer has become confused.

    --- It is not clear how K_1 and K_2 are defined. 

We can elaborate.

    --- There are various assumptions derived in the proof, but they are never explicitely applied. The authors assume that the reader will do a lot of pieces of the proof himself/herself, but do not give any hints. 

Perhaps.
DZ: In my opinion, adding much mare details will not make the proof easier. But let's go through the proof knowing what was confusing for the reviewers.

  -- Add some explanation of an AND-type relation and an OR-type relation and also the n-ary versions in the proofs (..org.). The remarks about other tuples in these relations should be put somewhere else (where they are used)
  
We can elaborate here but the remarks about the other tuples should be put here.
BM: Done.

  -- Some discussion about the strategy in Section 7 will be helpful, eg.
    --- better explain the role of the special element in Lemma 22 (will be used both in the algorithm as well as for Lemma 23)

*** Dima ***	
Which is the special element? This is one for you, Dima.

DZ: I believe special element is a variable y. I added an informal description of Lemma 22. Please check.
BM: Looks good. I will take out the indent.

    --- say that Lemma 23 and Corollary 24 are independent from the rest


Yes, that makes sense.
BM: Done. Also this applies to Lemma 37 and Corollary 38. Does Lemma 36 play a role in the main proof?
DZ: I would probably say more than "sanity check" explaining why this is cool. Lemma 36 (as well as 37 and 38) does not play any role in the main proof, but it is important for the example we give before Lemma 36 showing that finite Strange Structure of type 2 exists! 
BM: I added that it was cool, slightly rephrased.

    --- say before Lemma 25 that the aim is to prove Theorem 28
	
Yes.
DZ: Agree. Could you do this?
BM: Done.

  -- "we can check" is excessively used. Sometimes it is meant as "it is easy to see", in which case it would be better to omit the phrase or say from what the claim follows; sometimes my only suitable interpretation is "the authors can prove" (such as in the last line of the proof of Lemma 13, or in the proof of Theorem 50), in which case some argument is needed. Similarly, "contradicts our assumptions" etc. should be made specific.
  -- Special care should be taken about the proof of Theorem 6. It is the main result, so the proof should be given especially clearly.

These reasonable criticisms. We should at least add proofs to the places (Lemma 13, Theorem 50) mentioned.

DZ: Agree!
Ad Lemma 13, I tried to tighten the proof. It is easy to assume no universal variables are allowed in NAE constraints in I'. But one would also like to assume the instance I' is equality-free. Then I got in a pickle, as I couldn't remember whether we allowed equalities in our instances anyway? It is not so clear reading the paper and I know you raised this question in another context. What is our policy here and should we be clear about it at some point? Anyway, have a look at what I did in Lemma 13's proof.

- There are several notions that were not defined, please define or rephrase:
  -- the order used in Section 7 (e.g. Lemma 22)
  
Yes.
BM: Done.

  -- clone, composition f(g_1,...,g_n), linear in Subsection 9.2
  -- \alpha\beta-projection to a coordinate in Sections 9 and 10. (the paper only provides the definition for a \alpha\beta-projective function)
  -- factor, subuniverse, subalgebra in the proof of Lemma 59

Yes, these should go into prelims. 
BM: Done. Except I define linear only in the section in which it is used.
DZ: I changed your definition of linear. Should we also define monotonic or it is fine?
BM: Hm... probably we should. I will add a definition.

- I suggest to expand the conclusion: Does the classification suggest some general criteria for membership in some complexity classes? Hardness criteria? What about the non-idempotent 3-element case?

*** Dima ***
What do you think, Dima?

DZ: To be honest, I like our conclusions. Anyway, I tried to add few sentences. Have a look.
BM: Looks good to me.

- Few other minor comments
 -- Lemma 17, typos in the displayed formula
 
*** Dima ***
I don't see these.
DZ: Me neither. It is too many of them in the proof.

 -- Make the formulation of Lemma 18 more precise (also there is a typo in the definition of \Phi_i - the superscripts and subscripts are swapped). I suggest to define the formula in the proof, rather than in the formulation.

Yes. Michal noticed the subscripts and superscripts also.

DZ: Probably it is more natural to replace bottom by the top =) What do you think about hiding the formula inside the proof? I wouldn't because now reader doesn't need to go into the proof to get an idea. What do you think?
BM: I think it is fine as it is.

 -- Lemma 21: Inv(s) -> Inv(s_2)
BM: Switched superscripts and subscripts.
 
Yes.

 -- Lemma 41: specify what N is in the formulation
 
Yes, also picked up by another reviewer.
BM: Done.

 -- "grateful" in acknowledgements, the Czech names are typed "Ol\v s\'ak", "Je\v r\'abek"

Yes. (Can't see the problem with "grateful", perhaps we fixed it after submission?)
BM: Done.
